Effective Random Test Generation for Deep Learning Compilers

Deep learning compilers help address the difficulties of deploying deep learning models on diverse types of hardware. Testing deep learning compilers is highly crucial, because they are impacting countless AI applications that use them for model optimization and deployment. To test deep learning compilers, random testing, the testing method popularly used for compiler testing practices, faces the challenge of generating semantically valid test inputs, i.e., deep learning models that satisfy the semantic model specifications (in short as semantic specifications). To tackle this challenge, in this paper, we propose a novel approach named Isra, including a domain-specific constraint solver that resolves the constraints from the semantic specifications without backtracking. We implement and apply our approach to three popular real-world deep learning compilers including TVM, Glow, and a commercial compiler named SophGo. The evaluation results show that Isra is more effective than the state-of-the-art approaches and the baseline approaches on constructing valid test inputs for compiler-bug detection, and Isra successfully finds 24 previously unknown bugs in released versions of the three compilers. These results indicate Isra's effectiveness and practical value.

==> arXiv-2302.00842v2/macros.tex <==
\newcommand{\pre}[1]{}

% \newcommand{\rev}[1]{{\color{blue}{#1}}}
\newcommand{\rev}[1]{#1}

\newcommand{\CodeIn}[1]{{\small\texttt{#1}}}
\newcommand{\TODO}[1]{{\color{red} \bf \{TODO: {#1}\}}}
\newcommand{\toolname}{Isra}
\newcommand{\Luyao}[1]{{\color{blue} \bf \{Luyao: {#1}\}}}
\newcommand{\Ziheng}[1]{{\color{cyan} \bf \{Ziheng: {#1}\}}}
\newcommand{\bugnumber}{33}
\newcommand{\unknownbug}{24}

\newcommand{\opnumber}{65}
\newcommand{\metricsnumber}{XX}
\newcommand{\tone}{graph-level constraint resolving}
\newcommand{\ttwo}{operation-level constraint resolving}
\newcommand{\toneandtwo}{graph-level and operation-level constraint resolving}

\newcommand{\firstp}{graph-level directional consistency}

\newcommand{\bone}{declarative-style generation}
\newcommand{\boneshort}{DeclGen}
\newcommand{\btwo}{Randoop-like generation}
\newcommand{\btwoshort}{Randoop-Gen}


\newcommand{\mhy}[1]{{\color{orange} \bf \{Haiyue: {#1}\}}}
\newcommand{\zhengkai}[1]{{\footnotesize{\color{green} [Zhengkai: #1]}}}
\newcommand{\yx}[1]{{\footnotesize{\color{red} [Xiong: #1]}}}

\newcommand{\lcx}[1]{{\color{orange} \bf \{chenxi: {#1}\}}}

\newcommand{\tao}[1]{{\color{purple} \bf \{Tao's comments: {#1}\}}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}} 
\renewcommand{\algorithmicensure}{\textbf{Output:}} 



\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{1,1,1}
 
\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}
 
\lstset{style=mystyle}

==> arXiv-2302.00842v2/pkgs.tex <==
\usepackage{booktabs} % For formal tables
\usepackage{color}
\usepackage{listings}
\usepackage{enumitem}
\usepackage{threeparttable}
\usepackage{multirow}% http://ctan.org/pkg/multirow
\usepackage{hhline}% http://ctan.org/pkg/hhline
\usepackage{subfigure}
\usepackage{array}
\usepackage{pifont}
\usepackage{booktabs}
\usepackage{xcolor}
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage[noend]{algpseudocode}
\usepackage{graphics}
\usepackage{epsfig}

\usepackage{amsmath}

\usepackage{hyperref}
% \usepackage{amsmath,amssymb,amsfonts}
\usepackage{bbding}
\usepackage{caption}

%\usepackage[ruled,linesnumbered]{algorithm2e}

%\usepackage{algorithmic}
%\usepackage{graphicx}
%\usepackage{textcomp}


==> arXiv-2302.00842v2/sections/approach.tex <==
\section{Detailed Approach Description}\label{sec:approach}

%In order to better conduct random testing for deep learning compilers, we propose an approach named \toolname{} to effectively and efficiently generate random, diverse and valid deep learning models. We use a top-down way to illustrate our approach in details. The graph-level construction (as Section~\ref{sec:s3.2}) is the main process for our approach. Within the graph-level construction, the approach contains a main compound called operation-level construction (as Section~\ref{sec:s3.3}).

% Based on our insights on the properties of deep learning models, we illustrate our approaches on graph-level and operation-level separately, with discussing the soundness and completeness of them.

%As a suitable representation level of for the deep learning model, the computation graph is chosen as our generation target. In the computation graph, the nodes denotes mathematical operations and edges denotes input/output tensor(s).

\subsection{Notations and Definitions}\label{sec:s3.1}
% To better model the problem and describe our approach, we formalize following concepts with some notations.

%A tensor placeholder $T$ is an instance that we will assign the specific tensor value later in the computation of deep learning. It allows us to create our operations and build our computation graph, without needing the specific data. A edge is defined as a tuple with two tensor placeholders $(T_x, T_y)$, denoting a dataflow of computation graph, i.e., a value of placeholder (i.e. a specific tensor) that gets transferred between the $T_x$ and $T_y$. 
\subsubsection{Concepts in the Computation Graph}

A tensor $t$ is a generalized vector, like N-D array (N is a positive integer). The structure of tensor $t$ is defined as a set $Str_t$, denoting the structural information of the tensor. $Str_t$ includes (1) a numerical value $dim_t$ that denotes $t$'s dimension size and (2) a variable-length array that denotes each dimension's length of tensor $t$ (i.e., $t[i]$ as the i-st dimension's length).  

An operation $n$ is defined as a function with tensor(s) as input and output. It has some parameters: we denote $Op_{n}$ as its type ($Op_n \in AllOps$, $AllOps$ is a unverisal set which contains all types of operations), $Attr_{n}$ as a set which contains attributes of the operation (such as \emph{strides} in \CodeIn{Conv} operation, and \emph{axis} in \CodeIn{SoftMax} operation). 
Also, $Input_n=\{in_1, in_2, ...\}$ is a set which contains one or more tensors as the input of $n$, and $Output_n=\{out_1, out_2, ...\}$ as the output of $n$. 
Specially, $Attr_n$ contains a special attribute $Indegree_n$ as the number of tensors in $Input_n$, i.e., $Indegree_n = |Input_n|$. 

A tensor placeholder $tp$ is simply a variable, denoting a tensor to which the specific data will be assigned later. A tensor placeholder that denotes tensor $p$ could be created with merely $Str_p$, without need of specific data. 

%tuple $(Op_n, Attr_n, Input_n, Output_n)$, where $Op_n$ is an enumerated type data denoting the type of the operation ( is a universal set of the types of operations), $Attr_n$ is a set denoting the attributes of the operation (such as \emph{strides} in \CodeIn{Conv} operation, and \emph{axis} in \CodeIn{SoftMax} operation), both of $Input_n$ and $Output_n$ is a set of tensor placeholders denoting the input/output tensor(s) of the operation. 

A computation graph $G$ is defined as an ordered triple $(V_G, E_G, \psi_G)$, where the set $V_G$ denotes the nodes, the set $E_G$ denotes the edges. An element in $V_G$ is either an operation or a tensor placeholder. An element in $E_G$ is a tensor. $\psi_G$ is called an incidence function which maps an edge into a pair of nodes (i.e., a mapping from $E(G) \rightarrow V(G) \times V(G)$), denoting the structure of the graph.


%Each operation in a computation graph is naturally accompanied by the semantic specification, which specifies conditions that mathematical computations must satisfy. Specifically, for operations in a computation graph, the specification of the operation $N$, i.e., $Spec_{N}$, is defined as a set of constraints, which is related to the operation's attributes, i.e., $Spec_{N}: Spec_{Op_{N}}(Attr_N, Input_{N}, Output_{N})$.

% A variable $x$ is a symbol for a quantity that may change. In particular, a variable may represent a numerical number, a tensor, or an operation. 

\subsubsection{Constraint Satisfaction Problem}

A constraint $C$ is a limitation placed on the values of variables. Consider a finite sequence of variables $S:=\{x_1,x_2,...,x_k\}$, with respective domains $D(x_1)$, . . ., $D(x_k)$ associated with them. So each variable $x_i$ ranges over the domain $D(x_i)$. By a constraint $C$ on $S$ we mean a subset of $D(x_1) \times D(x_2)... \times D(x_k)$.

% We denote the set of all tensors in graph $G$ as $AllT_G$, i.e.,  $AllT_G = \bigcup \limits_{\forall N \in G} Input_N \cup \bigcup \limits_{\forall N \in G} Output_N$.

An instantiation $Q$ is defined as a set of tuples, written as $\left \langle x_1 = v_1, x_2 = v_2, ..., x_m = v_m \right \rangle$, denoting that a specific value $v_i$ that has been assigned to the variable $x_i$. 
%We denote $Var_Q$ as the union of the first element in each tuple, i.e., $Var(Q) = \bigcup \limits_{\forall (s:v) \in Q} s$.

%A evaluation $e: eval(Q, SC)$ means checking whether instantiation $Q$ satisfies all of constraints in $SC$.

%We call an instantiation $Q$ is satisfied on a constraint $C$ if \Luyao{todo}. we substitute the variable with its assigned value in $Q$, then $C$
%\Luyao{We call an instantiation $Q$ is satisfied on a constraint $C$ if ...}



%Note, the instantiation could be partial, that is, not all of the variables in the set $X$ are assigned by $Q$, i.e., $Q[X]$ is a partial instantiation if $\{s\ |\ \forall(s:v)\in Q\} \subset X$.

%For example, we have four variables: $x, y, z, w$, and we have an instantiation $Q: \{x: 1, y: 3, w: 4\}$. If we consider set $X=\{x,y,z\}$, then $Q[X]=\{x: 1, y: 3\}$, which is a partial instantiation because the variable $z$ is not assigned in instantiation $Q$.

%A instantiation $Q$ is defined as a set of tuples. Each tuple in $Q$ denotes a value instantiation for a variable, written as $(v, p)$. So $Q$ is written as $\{(v_1, p_1), (v_2, p_2) ...\}$.

%\Luyao{list all of possible forms of constraint}
%Our problem only contains the following two type of constraints: the equation with primitive operations between variables (i.e. $C1: c[axis]=a[axis]+b[axis]$) and 2) the inequation between two variables like $C2: strides<=a[1]$.


%Similar to Kleene logic~\cite{kleene1938notation}, there are only three kinds of results of evaluation: true, false or unknown.
% \Luyao{improve: improve the concept of evaluation, maybe satisfied, unsatisfied, unknown? check again.}
%For example, $eval(x \geq 2, \{(x: 3)\}) = true$, and $eval(x \geq 2, \{(y: 3)\}) = unknown$.

% $S$ is a universe set of all variables.
% $\overline{x}$ means the variable x is assigned with the value.
% $Y \subset S$

A constraint satisfaction problem (CSP) $P:(V, D, C)$, where $V$ is a set of variables, $D$ is the set of domains of values for each variable, $C$ is a set of constraints.
%where $Con_P$ as the set of the constraints in $P$, and $Var_P$ as the set of the variables in $P$.
A solution to a problem $P$ is an instantiation $Q$, containing the assignment of all variables in $V$, which satisfies all of constraints in $SC$. Namely, an instantiation $Q$ is a solution of $P: (V, D, C)$ only if it satisfies with all of constraints in $C$.

\subsubsection{Local Consistency and Global Consistency}
Let $X = (X_1, X_2, ..., X_n) $ be a set of variables in a CSP, and let $X^{'} = (X^{'}_1, X^{'}_2, ..., X^{'}_m)$ be a subset of variables from $X$.  A partial instantiation of variables $\left \langle X^{'}_1 = x_1, X^{'}_2 = x_2, ..., X^{'}_m = x_m \right \rangle$ is locally consistent if it satisfies all the constraints in $X^{'}$.
A globally consistent CSP is one in which any locally consistent partial instantiation of variables can be extended to a consistent full instantiation. Globally consistent CSPs have the property that a solution can be found without backtracking ~\cite{dechter1992local}.

% We call a problem $P$ is 1-consistent among variables if for every variable $x$ that every unary constraint of $x$ equals to $D(x)$. An extension of an instantiation is to assign a value to a variable which is not in current instantiation. And we call $P$ is k-consistent for $k \ge 1$, every (k-1)-consistent instantiation can be extended no matter which new variable is chosen. We call $P$ is strong n-consistent if it is i-consistent for every $i \in [1..n]$~\cite{dechter1992local}.


% Consider a problem with $k$ variables, where $k \geq 1$, such that (1) at least one domain is non-empty, (2) it is strongly k-consistent. Then this problem could be solved without backtracking \cite{} with ensuring the consistency.

%\subsubsection{Others}
%Besides above definitions, we define $D_{P, Q}(x)$ as the domain of $x$ under problem $P$'s constraints together with a partial instantiation $Q$. 


%For example, $Cor(R,T)[\{R[1]: \overline{R[1]}\}]=\{T[1] : \overline{R[1]}\}$ means the image of the instantiation of variables of $(R[1] : \overline{R[1]})$ in $T$ is $(T[1] : \overline{R[1]})$ (i.e. assign the corresponding variables of $T$ with same values in $R$). 
%Note that if the dimension size of one or both tensors has not been assigned (i.e. for a tenor $T$, $dim_T \notin Var_Q$), we can still build the mapping between this tensor and another one.

% We call a node $N$ in graph $G$ is valid if $Assign(G) \in Solution(P_N)$. We call a graph $G$ is valid if all of its node is valid. 

% In a problem $P$, We define the set of variables in $P$ which are related to a given tensor $T$ as the project of variables $PV(P, T)$. 

%A partial instantiation $I$ is globally consistent if it can be extented to a solution, i.e. there exists $s \in sol(P)$ with $I = s[Y]$.


% For tensors in $input(N)$ and $output(N)$, we only care about their shape since the semantic specification on the operation are all related to their shapes. We denotes the shape of tensor as a list where every element in dimension list is an integer value denoting the length of corresponding dimension of the tensor, the number of tensor's dimension as a numerical value.

\iffalse
\subsubsection{Our goal}

$P_G$ is defined as the CSP specified from computation graph $G$'s semantic specification. %$P_G$ contains all of constraints and variables of its nodes.

A model $M: (G, Q)$ is defined as a computation graph $G$ with an instantiation $Q$. We call a model valid if the instantiation $Q$ is a solution to the problem $P_G$. We define $M^{valid}$ as the set of all the valid models: $$M \in M^{valid} \iff Q \in Solution_{P_G} $$.

We define the function $Rand(S)$ as randomly sampling an element from set $S$. Our goal is to design a effective sampling approach for $Rand(M^{valid})$.
\fi

%For example, we have an operation $N=(MatMul, \emptyset, \{a, b\}, \{c\})$, then $Spec_{N}$ includes Equation~\ref{c1}-\ref{c5} (terms related to $c$ have not shown).

%The specification of the edge $e$, i.e., $Spec_{e}$, is defined as a constraint on the structures of two tensor place holder. Actually, assume $e=(T_x, T_y)$, then $Spec_e$ implies a constraint of equality on the structure of $T_x$ and $T_y$, i.e., $Spec_e := Str_{T_x}=Str_{T_y}$.

%Taking all of data in the operation $N$ as variables as $AllVar_N$, i.e.,  $AllVar_N = \{Op_N\} \cup Attr_N \cup (\bigcup \limits_{\forall T \in AllTPS_N} Str_T)$; $AllVar_e$ as the set of all data related to edge $e:(T_x, T_y)$, i.e., $AllVar_e = Str_{T_x} \cup Str_{T_y} $. Then, we denote the problem of an operation and a edge: $P_N$ i.e., $(Spec_{OP_N}, AllVar_N)$ is the problem of an operation $N$; $P_e$, i.e., $(Spec_{e}, AllVar_e)$ is the problem of a edge $e$.


% i.e., $Con_{P_G} = \bigcup \limits_{N \in V_G} Con_{P_N} \cup \bigcup \limits_{e \in E_G} Con_{P_e}, Var_{P_G} = \bigcup \limits_{N \in V_G} Var_{P_N}$.



\subsection{Graph-level constraint resolving}\label{sec:s3.2}

Based on the acyclic trait of the computation graph, for any computation graph, there always exists a topological order of operations, i.e., for every two operation $x$ and $y$ in computation graph, if there is a tensor that is both the output tensor of $x$ and the input of $y$, then operation $x$ comes before operation $y$ in the ordering.

Our approach works as a top-down way to incrementally instantiate a computation graph by iteratively instantiate a new operation and appending it into the computation graph, as shown in Figure~\ref{fig:p3}. % Our approach is a backtrack-free way for randomly constructing a whole computation graph. 
Specifically, we follow the topological order of operations to generate them in the computation graph. When to generate a new operation $x$, we need to instantiate $OP_x$, $Attr_x$ and $Input_x$, with ensuring the satisfaction $Spec_{OP_x}(Attr_x, Input_x)$ (the same with the definition in Section~\ref{sec:nutshell}). We leave the instantiation of edges in $Output_x$ later (when we instantiate another operation $y$ with an edge from $x$ to $y$) because the value of $Output_x$ could be determined only by $OP_x$, $Attr_x$ and $Input_x$, i.e., $Output_x = f_{OP_x}(Attr_x, Input_x)$.

%For the edges we instantiate in $Input_x$, we could create one 

%when the following nodes (nodes are behind of $x$ in topological order) are generated and be connected to $x$, because the the structure of tensors in the output could be separately determined by $OP_x$, $Attr_x$ and $Input_x$ (i.e., \begin{small} $Spec_{OP_x}(Attr_x, Input_x, Output_x) \Leftrightarrow Spec_{OP_x}(Attr_x, Input_x) \wedge Output_x = f_{OP_x}(Attr_x, Input_x)$ \end{small}).\Ziheng{Need to define fOP?}
% In other words, after $x$'s instantiation, when it turns to the instantiation of another operation $y$ (which is behind of $x$ in the topological order), we will consider the edge between $x$ and $y$, i.e., set the tensor $v$ from $Output_x$ as one of tensors in $Input_y$ with the condition that they are the same tensor ($v \in Output_x \wedge w \in Input_{y} \wedge v=w$).
% In this way, to ensure the consistency of instantiation, when instantiating $Input_x$, we need to consider the nodes before $x$. Because tensors in the output of the nodes before $x$ in the topological order may be the incoming edge of $x$ (i.e., tensor in the input of $x$).

After finishing the instantiation for current the operation (with its attributes and incoming edges), we iterate the same process for instantiating the next operation if the number of operations in the computation graph has not exceeded to the parameter we set (named $numop_{G}$ as the number of operations in generated computation graph).

\subsubsection{Property of \firstp{}}

% With taking each node as a variable (a set variable $V_x$ containing $Op_x$, $Input_x$, $Attr_x$), then the constraints related to each operation (e.g. Equation~\ref{eqs1} and \ref{eqs2}) is an unary constraint, and each map in $\psi_G$ corresponds to a binary constraint on two variables (the output of an node equals to the input of another node), so it is a binary CSP. 

Taking each operation as a variable (a set variable $V_x$, containing $Op_x$, $Input_x$, $Attr_x$), constraints of the computation graph could be rewritten as a binary CSP, consisting of two kinds of constraints: first are unary constraints on each variable, and second are binary constraints between two variables (i.e., the output of an operation equals to the input of another operation).
According to the definition, an instantiation $Q$ is locally consistent on $V_x$ if $Q$ satisfies all the constraints in $V_x$.

Because our instantiation follows the topological order of a computation graph, with only instantiating edges which are from previous nodes (variables that are ahead of $V_x$ in the order) to current variable $V_x$, the instantiation on $V_x$ will not affect local consistency of previous variables (based on the property of topological order). Thus, for each $x$, as long as we are able to instantiate $Q$ with its local consistency on $V_x$ every time, then we could include $V_x$ in the end of topological order, and instantiation is still consistent. Also, because we instantiate edges with the direction followed by the topological order, the overall graph is loop-free. Thus, following with the topological order, ensuring local consistency on each operation leads to bracktrack-free instantiation on the graph level.

%An instantiation $Q$ on a computation graph holds global satisfaction, if all of operations in the graph are locally satisfied with $Q$.
%A computation graph with global satisfaction, as well as no loop in the graph, corresponds to a semantically valid computation graph.


%Taking the topological order as the linear ordering on the variables, this problem is directional path consistent~\cite{apt2003principles}.

%Path consistency is equivalent to 2-path consistency~\cite{montanari1974networks}.
%This property guarantees that we only need to ensure the 2-path consistency, in other words, if we assure the new appended operation's validity, then the whole graph will be valid. In this way, we reduce the generation of the whole computation graph to the generation of several local parts of computation graph. Each local part contains type, attributes and input of a single operation. \Ziheng{Just one subsection?}



%The computation graph is a directed acyclic graph, which implies that the semantic specifications have no cyclic dependencies.

%No semantic specification exists between multiple operations.

%we could know that for any valid computation graph, if we remove the last operation in the computation graph's topological order, the rest of the computation graph is still valid.

%We have following observations on the properties of computation graph: (1) ; (2) induced subgraph $I$ (induced subgraph is formed from a subset of the vertices of a graph and all of the edges from the original graph connecting pairs of vertices in that subset) of a valid computation graph $G$ is also a valid computation graph if the node set of $I$ makes up a prefix of the topological order of nodes in $G$.


% $N_1, N_2, N_3, ...$. All of these nodes comprise a computation graph. $N_i$ means a single node with its edges on computation graph. $input(N_i)$ denotes its input tensor(s), and $output(N_i)$ denotes its output tensor(s).
%Based on the above analysis, our approach works as incrementally adding the operation with its related tensors into the computation graph and ensuring the computation graph is valid all the time.
%Based on our observation of the acyclic trait of the computation graph, we can ensure that the whole computation graph will be valid if the constraints of the current operation are satisfied.

\iffalse
Our graph-level construction is both sound and complete. The reasons are as follows: (1) the ensuring of soundness is because the existence of a valid operation with a specific type always holds since at least we could let all of its input tensors be newly generated, i.e., the operation becomes an isolated part in the model. So, for any given type $o$ we could always generate an operation with $o$ type:
$$\forall M_G \in M^{valid}, \forall o \in AllOps, \exists N, (Op_N = o) \wedge (M_{G'} \in M^{valid}) $$ where $G'=G \cup \{N\}$. (2) the ensuring of completeness is because the  operation's type is uniformly selected from the universal set. With a fixed number of total operations in the graph, arbitrary structure (sequence of the types of the operations) holds equal probability in generation.

% because of validity during generation, our approach holds the soundness of random generation for deep learning models.
The overall algorithm for graph generation is straightforward as Algorithm~\ref{alg:alg3}.

\begin{algorithm}[htbp] 
\caption{The Main Process of \toolname{}} 
\label{alg:alg3} 
\begin{algorithmic}[1]
\Require $AllOps$: the set of all of the types of operations, $sizeRange$: the range of the number of operations in the generated graph.
\Ensure A valid model generated by \toolname{}.
\State $(G, Assign_G) \gets (\emptyset, \emptyset)$ \Comment{Initialization with an empty model.}
\State $numOp \gets \Call{Rand}{sizeRange}$
\While{$|G| < numOp$ }
    \State $op \gets \Call{Rand}{AllOps}$ %\Comment{Randomly pick an operation.}
    \State $(G, Assign_G) \gets \Call{OpConstruction}{(G, Assign_G), op}$ 
    %\Comment{The function will generate a valid node.}
    %\State $G \gets G \cup \{N\}$ 
    %\Comment{Append the node into the computation graph.}
\EndWhile
\State \Return $(G, Assign_G)$
\end{algorithmic} 
\end{algorithm}

\fi




\subsection{Operation-level constraint resolving}\label{sec:s3.3}
% At operation-Level instantiation, our goal becomes how to instantiate a new operation to append into the existing work-in-progress computation graph. Specifically,

To instantiate a new operation $x$ and append it in the existing computation graph, we need to instantiate (1) $OP_x$, (2) $Attr_x$, (3) $Input_x$ (i.e., incoming edges). We take the instantiation of these items into following steps.

We first determine the $OP_x$ by random sampling from $AllOps$. Thereafter, the constraints can be specified.
To model constraints as a CSP as $P_x(V, D, C)$, we define a variable set $V_{x}$ which contains all the numerical items from $Attr_x$ and $Input_x$, i.e., $V_{x} = Attr_x \cup \bigcup_{t \in Input_x} Str_{t}$, and also, specify the semantic specification of the operation $Spec_{OP_x}(Attr_x, Input_x)$ as a set of constraints $C$ on the variables. A specific example is shown in Equation~\ref{c1}-\ref{c3}.

To solve the above CSP, based on constraint propagation~\cite{apt2003principles}, our approach works as follows: iteratively extending the instantiation by picking an unassigned variable and assigning the value to the variable from its domains; after each turn's instantiation on a variable, with the help of the solver, our approach will conduct constraint propagation among unassigned variables throughout the constraints to reduce the domain of unassigned variables.

During the above process, there are three main issues as follows.

First, the existence of quantifiers and unknown functions in the constraints introduces the difficulty of conducting constraint propagation. For example, in Equation~\ref{c2}: $C_2: \forall i \in [1, 2, ..., d_x] \wedge (i \neq axis), x_i = y_i$, without instantiating the value of $axis$, we do not know whether $C_2$ implies $x_1=y_1$.

Second, how to instantiates $\psi_G$ (the structure of the graph) during the solving process. A straightforward way (in a `generate-then-match' style) works as follows: first instantiate all symbol variables in $Input_{x}$,
and then matches each tensor in $Input_{x}$ with instantiated tensors (i.e., outcoming edges of instantiated nodes) by comparing their structures.
% However, due to the large space of tensors, the chance of exactly matching with instantiated tensors will be fairly low.
However, because the  domain of the tensors under instantiation is large, the probability of exactly matching instantiated tensors is fairly small. For example, in the example of Section~\ref{sec:s2}, to instantiate tensor $x$ and $y$ (i.e., incoming edges of \CodeIn{Concat}), the number of possible solutions is exploded, which leads to fairly low probability of the equivalence between $Str_x$/$Str_y$ and structures of instantiated tensors (such as $Str_p$).
Thus, this straightforward way will lead to the result that generated computation graph tends to be simple and scattered.
%because an edge between two operations has low probability to be instantiated, except when the randomly instantiated tensor exactly matches with the existing tensors.

Third, constraint propagation might produce an empty domain, causing backtracking of the solver (i.e., inconsistence of the instantiation), which affects the effectiveness of constraint solving. For example, for the constraint $(x=y) \wedge (x=z) \wedge (y \neq z)$, if the instantiation is $\left \langle x=1 \right \rangle$, after constraint propagation, $y$ holds an empty domain.

%There is a direct way to 
%in a 



To address those issues, we tailor a well order that successfully
%(1) eliminates the quantifier and unknown functions in constraints during instantiation,
(1) simplifies the constraints to be quantifier-free and unknown-function-free, and
(2) enables to controllably select choices for instantiating unassigned tensors;
with the guarantee that our propagation-based instantiation is backtrack-free (keeps consistency during the whole process).

In the following parts, we will first describe the order, and then explain our reasons for that, finally, illustrate the property of \ttwo{} in our approach.

\subsubsection{The order of the instantiation}

%To efficient sample solutions, we order variables in a sequence for the instantiation. With the well order of instantiation, we are able to eliminate quantifier and unknown function, and also, efficiently extend the instantiation without backtracking.



% the dimension size of the tensor (i.e., $\{dim_T | \forall T \in AllT(G)\}$).


%Because the forms of the constraints related to $dim_T$ are limited in deep learning model's semantic specification such as $c1 \leq dim(T) \leq c2 $ or $dim(T) = dim(T_1)$ ($c1, c2$ is integer values).
%\Ziheng{What do these constraints mean?}.
% So those values are either determined by the values of the existing variables of dimension size, or sampled from a known integer range.

For an operation $x$, our order contains several groups, arranged as follows: $G_1, G_2, G_3, ..., G_{|Indegree_x|+2}$. First group consists of one variable: $G_1=\{Indegree_x\}$. Second group is the variables related to the first tensor in the input (first incoming edge of this operation), i.e., $G_2 = Str_{in_1} (in_1 \in Input_x$).
Third group is the attributes of operations (except for $Indegree_x$), i.e., $G_3 = Attr_x \setminus \{ Indegree_x \}$.
For the rest, each group is variables related to the next tensor in the input (next incoming edge of this operation), i.e., $G_{i+2} = Str_{in_i} (in_i \in Input_x)$.
In the groups related to each tensor (assume the tensor is $t$), the variable that denotes the dimension size of the tensor is ahead of the variables that denote the length of each dimension of the tensor, i.e., $d_t$ (denotes $dim_t$) is ahead of $t_i$ (denotes $t[i]$).


%Actually, for all of operations in deep learning model, it only contains following dependencies: $dim_T, T \in Input_N$ depends on $Attr_N$; $T[i], T \in Input_N, i \in \mathbb{N}^+$ depends on $Attr_N$; $T[i], i \in \mathbb{N}^+$ depends on $dim_T$. \Luyao{refine}



%In the original semantic specifications, the existence of some items and constraints are actually dependent on the dimension size of the tensors. Because of layered generation, the value of dimension size of the tensor (i.e., $dim_T$) is already known, which means the number\Ziheng{value?} of variables in tensor structural constriants is known and the quantifier's range of constraints could also be known. 




%Our approach will first generate $Attr_x$, then we plug the value of $OP_x$ and $Attr_x$ into constraints, then $Spec_{OP_x}[Attr_x]$ only contains constraints on $Input_x$ and its related edges.


%The semantic specification of various operations could be modeled as constraints among input tensors.
%To generate a valid operation corresponds to the generation of random solutions to constraints. Formally, given a valid model $M_G$ and an operation type $op$, we need to construct a random operation $N$ with $OP_N=op$ and return a new valid model $M_{G'} \in M^{valid}$ where $G'$ is the graph after $N$ is appended to $G$ (i.e., $G'=G \cup \{N\}$).

%Next, we introduce our strategies for operation-level construction in detail, and illustrate the overall approach at last.

%The problem can be regarded as a constraint satisfaction problem (CSP) ~\cite{apt2003principles}, which is an NP-hard problem in general.

\subsubsection{Reason I: Quantifier and unknown function elimination}\label{sec:s3.3.1}
Specifically, there are two forms which cause the existing constraint solving or sampling approaches~\cite{DBLP:conf/tacas/MouraB08, DBLP:conf/iccad/DutraBS18} hard to handle. First is the quantifier in the constraints, which hold the forms as $\forall i \in f(x), C(i) $, where $f$ is a function returns a set, $x$ is a variable, $C(i)$ is a constraint whose form is dependent on the value of $i$. Second is the unknown function. Constraints may contain terms such as $t_{f(x)}$, where $f(x)$ is a function that returns an integer number and $t_{f(x)}$ is the variable that denotes the $t[f(x)]$ (f(x)-st dimension's length of tensor $t$).
%\Ziheng{the unknown function is t, not f, right?}
%\Ziheng{The two challenges has been clarified before. Also, the word unknown hasn't been explained here.}

Our instantiation could eliminate the quantifiers and unknown functions in constraints with the following reason.
As quantifiers in form of $\forall i \in f(x), C(i)$, for all of variable $v$ whose existence in $C(i)$ depends on the domain of $f(x)$, we call that $v$ depend on $x$.
As constraints with unknown function such as $t_{f(x)}$, we call $t_i$ depends on $x$. 
For constraints on deep learning models, the above dependencies among constraints are loop-free. Our instantiation order is actually a topological order satisfying those dependencies, i.e., ensuring that for any dependencies that $x$ depends on $y$, $y$ is ahead of $x$ in the order. Thus, followed by the instantiation order, with satisfying the precondition of eliminating quantifiers and unknown functions by instantiation, we could simplify the constraints to a decidable propositional logic for constraint propagation.

%As an example, $B_{dim_B-1}$ appears in Equation~\eqref{c4}. The term $B[dim_B-1]$ could not be determined to which variable unless we know the value of $dim_B$. 

% we could observe that the existence of some variables or constraints are dependent on some of other variables,
%For example, in Equation~\eqref{c5}, $A[1]=B[1]$ exists only when the value of $dim_A$ is larger than 2.
%Generally, the domain of the quantifier may depend on other variable(s), so the existences of some relations may depend on other variables. 

% Actually, only after being aware of the specific value of $dim_A$ and $dim_B$, we could determine the variables which are at the each side of the constraint $a[dim_A] = b[dim_B-1]$. In other words, 
%The structures of tensors will appears at the constraints.


\iffalse
Inspired by the quantifier elimination technique, we could transform those terms into a fixed number of variables. \Luyao{refine}

The overall constraints could be simplified as quantifier-free constraints with no extra dependence.
%Back to our example, after first assigning the value of $dim_A$, Equation~\eqref{1c} and Equation~\eqref{1c} will be concrete.


In our design, the attributes of the operation are at the first layer in constraint simplification. As for the implementation, our approach will start with first randomly generate the attributes of the operation.

Next, we construct the input of the operation. To formalize it, taking the semantic specifications of the operation as constraints, we model the generation of the input for operation $N$ as a problem $P_N$.
%$Var_P$ contains $Para(N)$ and $\{\forall X \in input(N), Str(X)\}$. $Cons_P$ constrains the constraints in semantic specification which are related to those variables.
We need to sample a random solution for $P_N$ as an instantiation $Q$, which contains the attributes of the operation and the input tensor(s) of the operation: $Q \in sol(P_N)$ and $\forall T \in input(N), Str_T \in Var_Q$.

\fi


\subsubsection{Reason II: On-demand instantiation}
%Though strong n consistency , .... \Luyao{}

The reason why we put the variables related to the same tensor in a group, i.e., instantiate the tensor(s) one by one, is due to the consideration of instantiating $\psi_G$.

%\Luyao{remove following paragraph?}

We design an on-demand policy for instantiating the tensor, with consideration of the instantiation for $\psi_G$ in the meanwhile. For each tensor $t$ in the input of $x$ ($t \in Input_{x}$), 
our on-demand policy instantiates $Str_t$ with two choices: (1) reusing the structure $Str_s$ of an existing tensor $s$ as long as they are consistent with the instantiation, in other words, we set $t$'s structure the same as an instantiated tensor $s$, which is from the output of an instantiated node $ex$, i.e., instantiating $t = s$ with $\psi_{G}(t) = (ex, x)$ (if there are more than one satisfied tensor, we will randomly pick one of them; if no such tensor, we choose the second way); (2) creating a new tensor placeholder as a node $n$, and set its output as $t$, in other words, instantiating a tensor $t$ with $t \in Output_n$ as well as $\psi_G(t) = (n, x)$.

We select the choice of instantiating tensors according to a Bernoulli distribution, as a common way to produce random boolean decisions. Any other distributions are also allowed. The distribution is controlled by a parameter $picking\ rate$. The higher $picking\ rate$ is, the higher chance that our approach would select the first choice (i.e., reusing an existing tensor). To favor generating more complicated computation graphs, we set $picking\ rate$ relatively high in practice.
We will further explain the effect of this parameter in Section~\ref{sec:evaluation}.

\iffalse
In the implementation of our on-demand policy, there is a key process named tensor matching, aiming to find candidates from instantiated tensors that can be assigned to the tensor under instantiation without breaking the consistency of instantiation. 
%In short, we call those candidates match with the tensor under instantiation.
%\Ziheng{i.e., extending the instantiation? P.S., the terms related with instantiation are too many, e.g., ordered instantiation, on-demand instantiation, extend the instantiation...} 
% This is the way to join different nodes in computation graph. Scilicet the input/output tensors in one node could be the input tensors of another node in computation graph. Reusing the tensors builds the dataflow of tensors in computation graph which commonly happens in almost all of deep learning models in practice. In our approach, we design the tensor reuse mechanism based on tensor matching.
%We will use concepts of the mapping of tensor's attributes in the later parts in this section. 
To formalize it, we define the mapping between structures of two tensors $r$ and $t$ as follows: 
$M_{r, t}: \{dim_r \rightarrow dim_t, r[1] \rightarrow t[1], r[2] \rightarrow t[2], ...\}$.
%For $\{v1 \leftrightarrow v2\} \in Cor(r, t)$, we define a function $Cor(r,t)}(v1) = v2$ to denote the image of variables in correspondence.
We define a set denoting the correspondence between two tensors under the instantiation: $Cor_{Q}(r, t) = \{(M_{r, t}(x) : v)\ | (x \in Str_r) \wedge ((x : v) \in Q) \} $.
With above definitions, we conduct tensor matching for tensor $t$ under instantiation $Q$, named $Match(r, Q)$. To find all of such tensor $r$ that satisfies with the condition that $r$ is instantiated and the instantiation $Q$ on $Str_t$ is the subset of corresponding instantiation on $Str_r$: 
$$ Match(r, Q) = \bigcup_{t} \ Q \subset Cor_{Q}(r, t) $$
\Luyao{add t is instantiated? Strt belongs to Q}
\fi

\subsubsection{Property of operation-level global consistency}
We illustrate that our propagation-based instantiation will not lead to inconsistence due to the property we called operation-level global consistency.
For the constraints related to each single operation such as $x$, after determining the type ($OP_x$) and the number of tensors in the input ($Indegree_x$), we could take attributes as a variable and each tensor in the input of the operation as a variable. With good properties of specification on deep learning operations, this CSP is globally consistent~\cite{dechter1992local}. Thus, any order for instantiation, including our delicately-designed instantiation order in our approach, will not lead to inconsistence.

\subsection{Properties of \toolname{}}
Overall, \toolname{} in our approach is backtrack-free, sound and complete.
%guarantees soundness and completeness for generating random deep learning models.
Based on the property of \firstp{} and opertional-level global consistency, we are able to instantiate without backtracking. And also, soundness is guaranteed because the instantiation is always consistent, leading to the satisfaction of final solutions.
Completeness is due to that we do not lose probability of generation of any instantiation during the whole process, in other words, any instantiation that satisfies the constraints has the possibility to be generated.



\iffalse
\subsubsection{A running instance of operation-level instantiation}

In our example, for $a$, it could reuse existing tensor $r$ or $t$\Luyao{todo}; or it could be newly generated. This choice actually effect the density of edges in the model (measured by a metric named NOP in our evaluation). We would control\Luyao{another word maybe?} the choice with a user-defined parameter (we will discuss in detail in Section~\ref{sec:approach}).
In our example, different choices for $a$ and $b$ lead to different models as shown in Figure~\ref{fig:p2}.

As the running instance of the Section~\ref{sec:s2}, shown in right of Figure~\ref{fig:p2}, assume we already pick tensor $A$ as $X_out$. For the construction of $B$, we will match each of existing tensors with $B$. Note, some variables of $Str_B$ could have already been assigned with values. In that example, $Q=\{dim_B: 2, B[1] : 5\}$, assume the tensor to match with $B$ is tensor $X$, we will check if $Q[Str(B)] \subset I_{Cor(X, B)}(Q[Str(X)])$ . Here, the tensor $Y_{out}$ (output of operations $Y$) satisfies the condition because 
$Q[Str(B)] \subset Cor(Y_{out}, B)[Q] = \{dim_B: 2, B[1]: 5, B[2]: 4\}$.
The $X_{out}$ does not satisfy the condition because 
$Q[Str(B)] \not\subset Cor(X_{out}, B)[Q] = \{dim_B: 2, B[1]: 3, B[2]: 5\}$.
We will randomly pick any of matched tensors to update our new generated tensor with the instantiation of picked tensor (assume we pick $Y_{out}$ here then we will add $(B[2] : Y_{out}[2])$ into instantiation $Q$).
%We will also do propagation as we have mentioned previously because some variables have values assigned to. 

As for the second choice of two ways for construction, because all of variables in our under-construction tensor is newly generated. We could model this construction as follows. Given a problem $P_N$, a target tensor $T \in input(N)$ for generation and a value instantiation $Q$ (i.e., a partial instantiation including some of tensors which have already been constructed), we aim to assign values for variables in $Str_T$ into $Q$ with no conflict on constraints. Based on the layered constraint simplification as discussed in Section~\ref{sec:s3.3.1}, we assign the value for variables with the layered order. For each variable $x$, we sample a random value from its valid domain, i.e., $D_{P,Q}(x)$. The valid domain for variable $x$ under problem $P$ with the instantiation $Q$ could be calculated by the propagation technique~\cite{apt2003principles} on the constraints.
%a linear constraint solver. In our approach, we implement an effiencent .
\fi

\iffalse
\subsubsection{propagation-based solver for the valid domain}
%(i.e., $Q[Str(T)] \in D_{P, Q}(T_i) \wedge \forall C \in Cons_P, \ eval(C, Q[Var_P]) \neq false$)
%\subsubsection{Propagation in Constraint Simplification}
Layered constraint simplification transform the constraints to be quantifier-free and without tensor structural constraints for each layer. Actually, due to the traits of operations in deep learning, the constraints would be linear expressions between variables. Furthermore, it holds a loop-free property: if we build a graph with every constraint and variable both as a node (named `constraint node' and `variable node' respectively), and add undirected edges between `variable node' $x$ and `constraint node' $e$ if variable $x$ exists in expression $e$, then this graph does not contain the loop.

This property could guide a more aggressive constraint simplification process. Our approach conduct an effective and efficient propagation-based simplification process for solving the valid domains of variables.

Every time we assign a value to a variable $v$, we will conduct the propagation process. It works as follows: if there exists a constraint with only one variable whose value has not been assigned, we will update the variable's domain based on the constraint.
%and assign the value to the variable. The propagation will iterate until no such constraint exists. After the propagation process, we pick the next unassigned variable in the current layer and repeat this process until all of the variables have been assigned.

To formalize, for an instantiation $Q$, we take $U_{Q}(C)$ as the set of unassigned variables in the constraint $C$ (i.e. $U_{Q}(C) = Var_C \setminus Var_Q$).
Inspired by constraint propagation in constraint programming, in our case, if there exists a constraint $C$ that $|U_{Q}(C) = \{v\}| = 1$, then we pick the only unassigned variable $v \in U_{Q}(C)$ and calculate the domain of $v$ by plugging the values of other variables into the constraints. In our problem, because the constraints are all linear expressions with primitive mathematical operation, the rewriting is relatively easy. For example, in constraint $C: x + y \geq z, Q: \{x : \overline{x}, z: \overline{z}\}$, because $x$ and $z$ have been assigned values $\overline{x}$ and $\overline{z}$ but y has not, $y$ is the only unassigned variable in $C$. We do constraint propagation on variable $y$ : use $C[Q]: y \in [\overline{z} - \overline{x}, +\infty]$ to update $D_{P,Q}(y)$. This process works as Algorithm~\ref{alg:1}.

\begin{algorithm}[htbp] 
\caption{The Pseudocode of Propagation} 
\label{alg:1} 
\begin{algorithmic}[1]
\Function {Propagation}{$P, Q$} 
    \While{$\exists \ C\in P, |U_{Q}(C) = Var_C \setminus Var_Q| = 1$}
        \State $pv \gets the\ only\ variable\ in\ U_{Q}(C)$
        % \State $C' \gets rewrite\ C\ with\ only\ v\ on\ left\ hand\ side$
        \State $update\ D_{P,Q}(pv)\ with\ C[Q]$
        % \State $Q.add(\{pv:pvValue\})$
    \EndWhile
\EndFunction
\end{algorithmic} 
\end{algorithm}

%Back to the layered tensor constraints solving,
%\textbf{Propagation} happens when we assign a value to a variable. 
%in our approach means assigning the value to a variable from its domain randomly. At each step, we will pick an unassigned variable and sample a random value from its domain, then assign the value to it. We will also use other sampling algorithm or sample with some distributions on variable's domain.
% After picking the specific value $t$ of the variable $v$, we add the $(t, v)$ into our instantiation. Note, when adding a new instantiation on variable(s), in order to meet the constraints, we may need to assign values to some other variables because some other variables' value could be already determined. Actually, we conduct a process named propagation to achieve it. In our problem, since the constraints are all linear expressions with primitive mathematical operation, the propagation is relatively easy and we will describe it in detail later. 

The soundness of the propagation is ensured by the acyclic trait of the graph we use before (i.e. the graph with `variable node' and `constraint node').
%During propagation, the attribute-dependent constraints will be determined due to value instantiation in the well order that toposort generated. Thus the constraints in propagation process will be all quantifier-free.
%We build a graph that each node either denotes a variable or a quantifier-free constraint. And we build a edge between node $x$ and node $y$ if following conditions are satisfied: (1) $x$ denotes a constraint $C$, (2) $y$ denotes a variable $v$, (3) variable $v$ appears in constraint $C$. 
Based on the trait of constraints from deep learning specifications, we will obverse such property: the graph we used before is a tree actually, and the propagation process is like passing the value from one `variable node' (the node denotes a variable) to another `variable node' through an `constraint node' (the node denoting a constraint).

\fi


% For the third level, because the structures of the tensor (i.e., the tensor’s dimension size and each dimension’s length) are determined, which indicates the shape of the tensor, we just need to construct a specific tensor according to the known shape. For each element in the tensor, we regard it as a variable and generate a random numerical value for it. By arranging these elements as the shape of the tensor, we could finally construct the tensor that satisfies the constraints on the third level.





% \subsubsection{Linear constraint solving with Propagation}

%\textbf{Tensor matching} 
%for a given tensor $T$ that we need to generate, we will check if each existing tensor could be the same shape with $T$ without conflicting the constraints.

%Note, some attributes of $T$ could already been assigned to values.

% In the example, $dim_B: 2, b[1] : 5$. We will check if the current instantiation on the attributes of tensor $B$ is the subset of corresponding values in the tensor $t$ we would like to match with. Here, the tensor $Y_{out}$ (output input of operations $Y$) satisfies the condition because current instantiation on the attributes of tensor $B$ is the subset of corresponding values in $Y_{out}$ ($Y_{out}$'s dimension is 2, length of its 1-st and 2-st dimension is 5 and 4). The $X_{out}$ does not satisfy the condition because its 1-st dimension is 3 which is not equal to 5. We will choose any of matched tensors and copy the values of its attributes to our target tensor (here it is $B$), like assign the value for variable in a batch. We will also do propagation as we have mentioned previously because some variables have values assigned to. 


% Our approach will first randomly generate the type of the operation and construct rest of the things based on the semantic specification of the operation. We take the semantic specification as the constraints we would like to satisfy, and the variables in the constraints map to the nodes and edges in the deep learning model. Constructing the valid node which conforms to its operation's semantic specification could be taken as the random instantiation on variables with satisfying the constraints among those variables. Furthermore, to achieve randomness becomes sampling from the solutions of variable instantiation on the constraints. Each valid solution which satisfies the constraints are corresponding to a valid scheme for the operation. We would like to effectively random sample on those solution to the constraints.  Inspired by the idea of constraint propagation in constraint programming~\cite{apt2003principles}, we propose a novel technique which enables our approach to randomly generate solution with satisfying the constraints. The key step of technique is called propagation, which is to propagate value restriction from known variables to unknown variables. With the acyclic trait on variable level, we could prove that the propagation keeps up with soundness and completeness for the generation.




% \subsubsection{A quick running instance}
% Our approach for node construction mainly contains two main techniques: on-demand tensor generation and layered tensor constraint solving.
% Before describing each technique in detail, let us take a concrete example as Figure~\ref{fig:p1} and Figure~\ref{fig:p2} to illustrate how our node construction works in a nutshell.

% Based on semantic specification of the $MatMul$ operation (if the dimension of tensor is larger than 2 it is treated as a stack of matrices residing in the last two indexes and broadcast\footnote{\url{https://docs.scipy.org/doc/numpy-1.13.0/reference/generated/numpy.matmul.html}}), the value of variables need to satisfy the following constraints:
% \begin{align} 
% &a.len = b.len       \label{1a}\\
% &a_{a.len} = b_{b.len-1}   \label{1c}\\
% &a_{i} = b_{i}, i \in [1, 2, ..., a.len-2] \label{1f}\\
% \end{align}

%Our approach generates the input tensor(s) of the operation one by one. For each tensor we would like to generate, we have two choices: (1) reusing an tensor from the output tensor(s) of existing operations, (2) generating a new tensor. We randomly select the choice. The probability of selection on each choice is controlled by a predefined attributes called `picking rate'. The higher the `picking rate' is, the higher chance that our approach would select the first choice. In our implementation, we set this parameter relatively high because we would like to let the graph have more connections instead of many isolated parts. \Luyao{We also do a sensitive experiments for this parameter in evaluation.}
%For the first choice, we would conduct `Tensor Matching'. It is also possible that no existing tensors match with current targeted tensor. Under such situation, we have to generate a new one. 
%For the second choice, we would iterate run sampling process and propagation until all attributes of the target tensor have value assigned. 

% Because output is determined by input(s), we just need to generate attributes of input tensors that satisfies the constraints.

% Assume it chooses the \CodeIn{MatMul} operation (i.e. matrix multiplication) to insert into the model. We denote the input and output tensors of this operation as $A$, $B$ and $C$ with $C = MatMul(A, B)$. 

% Next, our approach constructs the input tensors via on-demand tensor generation. In the example, assume we first construct $A$ then $B$ (situation of first $B$ then $A$ is similar). For the construction of tensor $A$, we have two choices: (1) reusing an existing tensor, (2) generating a new tensor in the existing model. We randomly select the choice with a parameter named $picking\ rate$ to control the distribution (it will be discussed in detail later). We illustrate both of the cases in the left of Figure~\ref{fig:p2}. 

% %which would leads to more connections in the generated graph instead of many isolated parts. \Luyao{We also do a sensitive experiments for this parameter in evaluation.}
% If we select the first one, we will conduct tensor matching to take an existing tensor for $A$. If we select the second one, we need to construct a new tensor for $A$. In this situation, we conduct layered tensor constraint solving to generate the new tensor. Assume we construct $A$ with second choice as taking $X_{out}$ with the shape of $3 * 5$.

% Then we start to construct tensor $B$. At this point, we also have two choices for $B$:  reusing an existing one or generating a new tensor. We illustrate both of the cases in the right of Figure~\ref{fig:p2}.  For the first case (reusing existing tensors), we will also conduct tensor matching to take an existing tensor for $B$. For the second case, we also conduct the layered tensor constraint solving for generating $B$. The different choices for tensor $B$ lead to different models as shown in the rightmost of Figure~\ref{fig:p2}.

\iffalse
\subsubsection{Overall Operation-Level Construction}

The overall approach of iterative operation construction works as Algorithm~\ref{alg:alg2}. 

\begin{algorithm}[htbp] 
\caption{The Pseudocode of Operation-Level Construction} 
\label{alg:alg2} 
\begin{algorithmic}[1]
\Require $op$: the type of the operation to append. 
\Ensure A new model that from the prefix model with the appendix of the randomly generated operation.
\Function {OpConstruction}{$M,  NewOp$} 
    % \For {$p\ in\ Attr_N$} 
    %     \State $Assign_G \gets Assign_G \cup \{p : \Call{Rand}{D(p)}\} $
    % \EndFor
    \State $(G, Q) \gets M$ 
    \State $ExistingTs \gets AllT_G$ 
    \State $PRM \gets Parameters_{NewOp}$
    \For {$p\ in\ PRM$} \Comment{Generating the parameters.}
        \State $Q \gets Q \cup \{p : \Call{Rand}{D(p)}\}$ 
        % parameters of operation (as the first step in constraint simplification)
    \EndFor
    
    \State $N \gets (NewOp, Q[PRM], ..., ...)$ \Comment{Initialize the operation.}
    \State $P \gets (Spec_{NewOp}, Vars_N)$
    \For {$T\ in\ Input_N$} \Comment{Bottom-up Tensor Generation.}
        \State $matchSet \gets \{R | R \in ExistingTs \wedge Match(R,\ T)\}$  % \Comment{Get all tensors that matches $t$.}
        % \State Constraint Simplification...
        \State $IsReuse \gets Bernoulli(picking\ rate) $
        \If{$IsReuse \wedge (|matchSet|>0) $}  
        %\If{$(|matchedSet|>0)\ and\ (X \sim B(1, picking\ rate))$}
            %\State \Comment{Reusing existing one.}
            \State $matchT \gets \Call{Rand}{matchSet}$ 
            % \Comment{Randomly pick one of matched tensors.}
            \State $Q \gets Q \cup Cor(matchT, T)[Q] $
            %\For{$ (v: value)\ in\ Ass_{Q}(Str(r))$}
            %    \State $Q.add(\{I_{Cor(R,T)}(v) : value\})$
            %\EndFor
            %\State $add\ ct's\ attributes\ to\ t$ \Comment{Assign the attributes of picked existing tensor to the target generated tensor.}
            %\State \Call{Propagation}{$P, Q$}
        \Else 
            %\State $Sv \gets Str(t)$ \Comment{get all variables related to tensor t in P.}
            % RandAssign(S) \{(x : ) | \forall x \in S\}
            
            %\State \Comment{Generating new one.}
            \For{$x\ in\ \Call{Layer}{Str_T}$} 
                \State $Q \gets Q \cup \{x: \Call{Rand}{D_{P, Q}(x)}\} $
            \EndFor
        \EndIf
        % \State $\Call{Layer Simplification}{Assign_G}$
        % \For{$ level = 1\ to\ 3 $ }
        %     \For{$ v\ \in\ current\ level's\ variables $}
        %         \If{$v \in Str(T)$}
        %             \State 
        %         \EndIf
        %     \EndFor
        % \EndFor
        % \State \Call{Layered Simplication}{$Assign_G$}
    \EndFor
    \State $Output_N \gets \Call{calculate}{NewOp, Input_N} $
    \State  \Return $(G \cup \{ N \}, Q)$
\EndFunction

\end{algorithmic} 
\end{algorithm}

The function $Layer$ in Line 16 corresponds to the layered order as we discussed in Section~\ref{sec:s3.3.1}. It accepts a structure of a tensor $Str_T$, and returns a layered order of variables of $Str_T$. The function $calculate$ in Line 18 means that it directly calculates the result of operation $newOP$ with the input as $Input_N$. The return of this function is one or several tensors as the output of this operation.
\fi

% Completeness holds because that our approach does not miss any chance of generating arbitrary valid deep learning models. The detailed explanation of the soundness and completeness will be described in Section~\ref{sec:approach}. 


% following reasons: (1) on-demand tensor generation holds the satisfaction of the constraints because of strong arc consistency; (2) the layered tensor constraint solving holds the satisfaction because of the soundness of the propagation process in each layer. So the completeness and soundness of the whole algorithm for the node construction are both guaranteed.

% We could do topological sorting on the attributes: for every `index dependency' $a \xrightarrow{} b$, variable $a$ is prior to variable $b$ in sequence $S$, we call sequence $S$ as a topological order on tensor $t$'s attribute which satisfies the order relation between variables. Note, topological order for tensor $t$ is not necessarily unique, and we would like to random sample from all the topological orders. \Luyao{add how to generate a `random' topological order?}. With the topological order, we could generate variables based on the order of topological order which could avoid the unknown index of tensors' variable. 




% \subsection{Properties of our approach}
% \Luyao{TODO}

% \subsubsection{Soundness}
% The soundness of the whole algorithm could be ensured by the validity of generated deep learning model. We will show the correctness of propagation and tensor matching in our approach that achieves the satisfaction on the constraints in the problem.

% \subsubsection{Completeness}
% First, since there is no restriction between nodes in computation, any sequence of computation graph's node could be generated. So the problem comes to show the completeness of generation process for single node generation. Actually, it is equivalent to show that all the sampling have not lose the space of solution. \Luyao{need to complete}

% \subsubsection{Randomness}
% In variable sampling, all the variables are sampling from their domains. And in node construction, reused tensors are sample from the set of all matched tensors. 


%We can easily define a DL model using ONNX API, whose ecosystem supports exporting its model to run on various deep learning compilers.


%Next, we will describe each part in detail.



%However, because of the dependencies for the existence of some attributes or constraints as we have mentioned in Section \ref{sec:s2}, the order of variable generation is important to us. A well-designed order will eliminate the indetermination of the existence of some attributes or constraints, which we will discuss in toposort part later.



%Because constraints just contains primitive mathematical operation

%And the completeness

% if we treat both the variables and the quantifier-free constraints as nodes and add edge between a node of constraint and a node of variable if the variable appears at the constraint, the this graph is acyclic so we could safely conduct propagation as determining some attribute's value without backtracking.


%The reason why propagation is sound
%\Luyao{proof for \emph{propagation-level} acyclic trait}


%\subsubsection{Toposort}
%Given a set of variables and the dependencies of variables, toposort process will take the variables as nodes and dependencies as edges in the graph, and generate a sequence of nodes where each node appears before all other nodes it points to. 

% The expression of constraints would contain terms like $a[a.len-1]$ (because the existence of list) or $a[axis]$ (axis is the parameter of the operation). Only after we know the value of the variable in the index (i.e. $a.len$ or $axis$ in the examples), we could identify which variable the variable  $a[a.len-1]$ or $a[axis]$ is corresponding to. 

% Among all the specification of deep learning operation we use for construction, the dependencies only have two forms:
% 1. a numerical variable $x$ (allows with primitive arithmetical operations) appears at the index of a list variable $a$ in constraints like $a[x - 1]$.
% 2. a numerical variable $x$ appears at the range of quantifier, and the quantifier is the index of some list data like $\forall i \in [1, x], a[i] = b[i]$.

% Note, because of the peculiarity of operation's semantic specification in deep learning model,

% Both forms imply the dependencies that only given some of numerical variables could we determine the existence of attributes or constraints related to variables in the list data:
% % it also implies the following special semantic relation of the order of generation:
% $ x \xrightarrow{} a_{i} $
% The arrow is defined as the left variable will be assigned earlier than the right variable, in other words, $x$ is ahead of $a[i]$ in the sequence of variable's instantiation order. 

%For all constraints of the operations, those `index dependencies' are only within the attributes of one tensor, in other words, in the scope of all semantic specifications of deep learning model. We only have term like $a[a.len]$, $a[a.len-1]$ in the expression of constraints, term like $a[b.len + c.len]$ will not appear in the expression of the constraint. Actually, it will only happen in two situations: $parameter \xrightarrow{} a_{i}, i \in \mathbb{N+}$ and $a.len \xrightarrow{} a_{i}, i \in \mathbb{N+}$ (a is a list denotes the shape of a tensor). 

% Taking the dependencies as the edge on a direct graph whose node is each attributed, we will do topological sorting on the graph.
% %We call sequence $S$ as a topological order on tensor $t$'s attribute which satisfies the order relation between variables.
% Note, the topological order is not necessarily unique, and all of them are feasible to our sampling. With the topological order, we can generate variables based on the order and satisfy all of constraints without backtracking.

% The existing of such topological order in our cases (constraints from semantic specification of operations in deep learning models) is not difficult to prove: the numerical variable $x$ which is at the left side of dependencies can only be either operation's numerical parameters (like $axis$ in \textbf{Concat}) or the attribute that denotes tensor's number of dimension (like $a.len$). We will always put the numerical parameters of the operation at the first in the sequence, then place all of variables which denote tensor's number of dimension, and finally put all other variables at the back. It actually proves the correctness of \emph{dependency-level} acyclic trait because a directed graph is acyclic only if there exits a topological order of the graph.


\iffalse

\subsubsection{Quantifier and unknown function elimination}\label{sec:elimination}
%Based on the instantiation, we could eliminate quantifiers and unknown functions in the constraints to further ease our sampling.
Inspired by quantifier elimination~\cite{gradel2007finite, DBLP:conf/cade/MouraB07}, if we already determine the domains of quantifiers and unknown functions in constraints according to the instantiation, we could then rewrite the formula of constraints to an equivalent form that does not have quantifier and unknown functions. 
%\Luyao{do we need to add the limitation that the domain is finite?}

Specifically, if the domain of a quantifier is determined, we could transform a quantified constraint to an equivalent quantifier-free constraint.
%For example, in Equation~\ref{e1}, with the assumption that we already determine the domain of $v$ (i.e., $V(G)$) as $\{x, y\}$, then $\bigwedge_{v \in V(G)} Spec_v(...)$ could be simplified to a quantifier-free constraint $Spec_{x}(...) \wedge Spec_{y}(...)$.
% For example, for Equation~\ref{c5}, with the assumption that $dim_a = \overline{dim_a}$ ($\overline{dim_a}$ means a specific integer number), this constraint could be simplified as $\forall i \in [1, 2, ..., \overline{dim_A}-2], a[i] = b[i]$, i.e., $a[1]=b[1] \wedge a[2]=b[2] \wedge ... \wedge a[\overline{dim_a}-2] = b[\overline{dim_b}-2]$.
Also, if the domain of an unknown function is determined, we could simplify the constraint by using a set of variables to denote the return value of the function under each input within the domain of the function.
%For example, with the instantiation that $dim_a = \overline{d_a}$ ($\overline{d_a}$ means a specific integer number), then the domain of the function $a[i]$ is determined, so we could denote the values of unknown function $a[i]$ as a set of variables, i.e., $a[1]$ as a variable $a_1$, $a[2]$ as a variable $a_2$, ..., and $a[d_a]$ as a variable $a_{d_a}$. Note, for Equation~\ref{c5} that contains both quantifier and unknown functions, it could also be simplified with the determination of the domains of both quantifiers and unknown functions, i.e., with $dim_a = \overline{d_a} \wedge dim_b = \overline{d_b}$, it could be simplified as $a_1=b_1 \wedge a_2=b_2 \wedge ... \wedge a_{\overline{d_a}-2} = b_{\overline{d_b}-2}$ ($a_i$ is a variable denotes $a[i]$, same with $b[i]$).

\Ziheng{Quantifier and unknown functions are two things; should use domains?} 
To satisfy the condition of elimination, i.e., the domain of quantifiers and unknown functions is determined, we could first instantiate the variables in the domain of quantifiers and unknown functions to simplify the constraints for better solving or sampling. For example, for $Spec_{Concat}(axis, r, s, t)$ (i.e., Equation~\ref{e5}-Equation~\ref{e8}), the domain of quantifiers and unknown functions would be determined if we first instantiate $dim_r$.
However, casual\Luyao{change the word, maybe aggressive} instantiation may lead to the constraint unsatisfied, when it happens, we need to backtrack and adjust our instantiation, which hurts the overall efficiency of sampling solutions. 
In our example, if we first instantiate their values as $dim_r:2$ and $axis:3$ to conduct quantifier elimination for Equation~\ref{e6} and \ref{e7}, the instantiation would be inconsistent due to Equation~\ref{e8}.

Thus, an appropriate instantiation is critical for the efficiency of constraint sampling. Our approach defines a well order to extend the instantiation that achieves the random sampling without backtracking. The order ensures that every time we sample the value of current variable, the constraints related to the variable are able to be simplified as quantifier-free and unknown-function-free ones, because the domains of quantifiers and unknown functions of constraints are determined due to the present instantiation.


\fi


==> arXiv-2302.00842v2/sections/evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}
\pre{To evaluate the effectiveness of our approach, we compare our approach with four baselines, including two state-of-the-art approaches Muffin~\cite{DBLP:conf/icse/GuLZ022} and TVMFuzz~\cite{DBLP:conf/sigsoft/ShenM0TCC21}.}
~\rev{To evaluate the effectiveness of our approach, we compare our approach with five baselines, including three state-of-the-art approaches Muffin~\cite{DBLP:conf/icse/GuLZ022},  TVMFuzz~\cite{DBLP:conf/sigsoft/ShenM0TCC21}, and NNSmith~\cite{NNSmith}.}
Also, we evaluate them on three popular real-world deep learning compilers to investigate their bug detection capability.
We construct the computation graph based on the ONNX~\cite{onnx} standard. Our implementation is on Python 3, supporting generation of \opnumber{} operations in total ~\cite{israproject}.
We address the following three research questions with an evaluation conducted on Ubuntu 20.04 of a laptop computer with Intel® Core™ i5-1135G7 CPU @ 2.40GHz and memory of 8GB. More details are included on our project website~\cite{israproject}.

RQ1: Is \toolname{} effective for generating test inputs for testing deep learning compilers?

RQ2: How effective and practical are the generated tests in revealing bugs in popular real-world deep learning compilers?
%What is the practical value of our approach for testing deep learning compilers in the real world?

RQ3: Does our approach outperform state-of-art approaches in terms of testing deep learning compilers in terms of coverage and bug detection capability?

\subsection{Compared Work}

To assess the effectiveness of \toolname{}, we first design and implement two baselines as the representative of another two types of test generation techniques, named \boneshort{} and \btwoshort{}. In addition, we also compare \toolname{} with \pre{two} \rev{three} state-of-the-art approaches that can be applied for testing deep learning compilers.
More specifically, we include the following representative techniques in our evaluation:

\subsubsection{\boneshort{}}
Declarative-style generation constructs deep learning models only based on the syntax grammar, in short as \boneshort{}. When determining the shape of tensors, it just randomly generates from all choices.
After the construction of the input, i.e., a whole computation graph, this approach directly feeds input into the compiler under test, and relies on the compiler's running to check whether the model is satisfied with its semantic specifications.
%It assures to satisfy only the syntactic specifications of computation graphs and is less possible to satisfy the semantic specifications. Running of compilers for checking also causes some overhead.

\subsubsection{\btwo{}}
Inspired by feedback-directed random test generation~\cite{pacheco2007feedback}, this approach conducts random generation for operation construction, i.e., randomly constructs a new operation to append it into the model, and checks whether the model satisfies the semantic specifications or not. This generation way can avoid generating invalid models at early stages, leading to the improvement of overall effectiveness, while the generation for a single operation to satisfy its semantic specifications is still ineffective.

\subsubsection{Muffin}
Muffin~\cite{DBLP:conf/icse/GuLZ022} is a state-of-the-art generation-based testing approach, proposed originally to test deep learning libraries such as Keras~\cite{keras}, generating models based on two model structure templates (chain structure with skips and cell-based structure) with deep learning library APIs. To satisfy with tensor structural constraints, Muffin hardcodes additional \CodeIn{Reshaping} layers to reshape the input/output tensors for the connection between layers.
\rev{Though Muffin is not designed for testing deep learning compilers, we can retrofit it to barely achieve the goal by converting the models constructed by high-level APIs into computation graphs with existing tools~\cite{tf2onnx}.}

\subsubsection{TVMFuzz}
\pre{To our knowledge, TVMFuzz~\cite{DBLP:conf/sigsoft/ShenM0TCC21} is the only existing work specifically targeting testing deep learning compiler.}
\rev{TVMFuzz~\cite{DBLP:conf/sigsoft/ShenM0TCC21} is a fuzzer which specifically targets testing TVM~\cite{DBLP:conf/osdi/ChenMJZYSCWHCGK18}.}
It randomly generates and mutates Tensor-level IR(TIR) expressions (the intermediary language of TVM) for fuzzing test, mainly towards the type-related bug detection. 

\rev{
\subsubsection{NNSmith}
NNSmith~\cite{NNSmith} is a generation-based approach for testing deep learning compilers, as a parallel research work with ours. 
NNSmith constructs the computation graphs based on the specifications of deep learning models: it tries possible choices for types, attributes, and input/output of operations by iteratively adding constraints from specifications and leveraging existing constraint solver Z3~\cite{DBLP:conf/tacas/MouraB08} to check the satisfaction; if constraints are not satisfied, it will backtrack and try different choices to pick. 
}

%because it generates test inputs at the level of the TVM IR.

\subsection{Study Subjects and Settings}~\label{s4.2}
We choose TVM \pre{and}\rev{,} Glow (two popular open-source compilers), and SophGo (a state-of-practice commercial compiler) as our study subjects.
% TVM is currently a top-level project of the Apache Software Foundation, and has more than 6.6k stars on GitHub. It is in use at dozens of both industrial and academic organizations and institutions. 
%TVM team has also established a startup named OctoML to commercialize TVM project and scale it up.
% ONNX Runtime is another deep learning which is established at 2018 by Microsoft. It released its first official 1.0.0 version at Oct, 2019. It currently has more than 4.5k stars on GitHub. Note, these two deep learning compilers are all maintained by experts and have well-tested before release.
For TVM and Glow, we download their official released versions from GitHub: TVM as v0.7 (commit id 728b829), Glow\footnote{Glow does not have release version on GitHub. Thus we directly download its latest version.} (commit id a2036bd). For SophGo, we attain its latest released version from the company that develops it.
%All of these study subjects are downloaded from their official GitHub repositories without any extra modification. 
%

%of these two compilers as our experimental subjects: TVM as official released version (v0.7.0) published at 2020-10-03 with 400k+ lines of code, ONNX Runtime as the stable version v1.8.0 with 570k+ lines of code. The experimental subjects are all downloaded from their official GitHub repositories without any extra modification. 

%ONNX Runtime as the stable version v1.6.0 with 470k+ lines \Luyao{refine} of code. The experimental subjects are all downloaded from their official GitHub repositories without any extra modification. 
%TVM is a popular deep learning compiler which has released its first public version at July, 2017. 
% We first download the latest offical released version of these two deep learning compilers (TVM v0.7.0 and ONNX Runtime v1.8.0). We then also pick another latest experimental version of TVM (c31e338). Note that our whole random testing treats the deep learning compiler as a blackbox. The only information we need is the final output when it terminates normally or the error message when it crashes or terminates abnormally. After download, we directly runs our tool on these compilers without any extra modification.


%\textbf{System Environment.} Our experiments were conducted on VMware-workstation 15.5.0 with ubuntu 20.04.1 on Windows 10 of a laptop computer with Intel® Core™ i7-8550U CPU @ 1.80GHz and memory of 8GB. 
%macOS Catalina 10.15.7 of a laptop computer with Intel® Core™ i5 CPU@ 1.4 GHz × 4 and memory 16 GB 2133 MHz LPDDR3.
%
For test oracles, we use two types of oracles: (1) runtime failure (including error/crash behaviors) of compilers, i.e., when a computation graph causes the exception of compilers (excluding invalid inputs that violate the specifications);  (2) differential testing by feeding the same random inputs and comparing the outputs of compiled models from different compilers.
In differential testing, % in order to avoid deviation,
we set the relative error as 10\% (we set this value relatively large in order to avoid many false positives) for automatically comparing results from different compilers under the same input. 
%In the experiments on bug detection, we exclude the errors that due to the existence of unsupported operations in the computation graph. 

%For the test oracle, we use both differential testing and the crash status of the compiler under test.  %As for the strategies of differential testing, we use both cross-compiler (i.e., comparing results produced by different compilers) and cross-optimization (i.e., comparing results produced by different optimization levels on the same compiler). 

%So for all input tensors in deep learning model, we initialize them with a tensor that contains specific value as input. Because we already know the shape of each tensor, we simple randomly generate each tensor by filling with random real numbers. 
%The testing process will iterate until it reaches to the time limitation. During the process of compiler testing, many bugs may be detected.

%\input{tables/table1}

For \toolname{}, we set the upper bound on the tensor dimension as 5, and the upper bound on the length of each dimension as 5 (which is aligned with default settings of Muffin). For $picking\ rate$, we set it with $0.97$ based on our sensitivity experiments, as shown in Table~\ref{tab:pickrate}. Except for above parameters which keep the same among all of experiments, we set the lower bound and upper bound of operation number in the graphs (named $lb$ and $ub$) according to the experiments, the $numop_G$ is uniform sampling between $lb$ and $ub$. 

%For Muffin, it contains 4 generation modes in their implementation. We randomly choose the modes with the same probability. For other parameters, we obey its default settings. 
For Muffin, we obey its default settings. For alignment with comparsions on coverage metrics, we convert the Keras models generated by Muffin to ONNX format with TF2ONNX~\cite{tf2onnx}. Because Keras API is more higher level than ONNX, the converting leads to the growth of model size. For fairness, in the experiment on coverage measurement, for every model Muffin generated, we adopt \toolname{} to  generate a model with the number of operations same as Muffin, named \toolname{}*. Also, we ensure that both approaches have a same operation set (of size 36, which is the number of overlapped operations).

%Note that models generated by Muffin may contain operations of type that we have not supported, in this experiment, we first let Muffin generate a fixed number of models (same as the settings below as 10000) whose operations are all in our implemented operation set, and then restrict \toolname{}* to generate models using the same operation set as that of the generated Muffin models. 

%The number of the operations that are overlapped is 36.


For TVMFuzz, we obey its default parameters. Due to the difference on the type of generated inputs (\toolname{} generates computation graphs, while TVMFuzz generates programs in TIR, an IR for the TVM compiler), the metrics that we design for the work in this paper are not applicable for TVMFuzz. So we are unable to measure our coverage metrics on TVMFuzz. TVMFuzz is compiler-dependent, so we are unable to test TVMFuzz on compilers except for TVM.

\rev{For NNSmith, we obey its default parameters. For fairness, in the experiment on coverage measurement, we align the settings of \toolname{} with those from NNSmith, named \toolname{}**. For every model NNSmith generated, \toolname{}** generates a model with the same number of operations. Also, we ensure that both approaches have a same operation set (of size 40, which is the number of overlapped operations).}
%\rev{For NNSmith, we obey its default parameters. For fairness, in the experiment on coverage measurement, for every model NNSmith generated, we adopt \toolname{} to generate a model with the number of operations same as NNSmith, named \toolname{}**. Also, we ensure that both approaches have a same operation set (of size 40, which is the number of overlapped operations).}

For the experiment on coverage measurement, we run each approach to generate a fixed number of models, as 10000. For the parameters of operation number in the graphs, we set $lb$ as 1 and $ub$ as 200 for \toolname{} as well as \boneshort{} and \btwoshort{} in the experiment.
To eliminate randomness, We run our approach and baselines separately for five times and calculate the average number.
According to our results of the experiments, the coverage metrics of the three approaches are all saturated or converged, so it is a reasonable setting for our evaluations. %\Ziheng{except DEC}


For investigating bug detection capability, aligned with the setting in ~\cite{DBLP:conf/icse/GuLZ022}, for each method, we generate 300 computation graphs for testing compilers. Due to the difference of supported operations for each compiler, we run the generators with filtering the generated graphs that contain unsupported operations until the graph number reaches to 300. To reduce manual work on deduplication, we set the generated model relatively small with $lb$ as 1 and $ub$ as 10.

 
%For the experiment of efficiency, we run our approach and baselines separately with a fixed time limit as 1 hour for five times and calculate the average number to eliminate randomness.


To save manual effort for checking duplicated bugs, we automatically check and filter the bugs with the same error messages and stack traces as produced before. For the rest of the bugs, two authors manually check their root causes through error messages, stack traces, and generated inputs to further eliminate duplicated bugs and false positives.


%The result is shown in Table~\ref{tab:exper3}. We also compare the results with various settings of parameters. More details are included on our project website~\cite{israproject}.

\subsection{Metrics}
In order to evaluate the effectiveness and practicability of different approaches, we investigate on their bug-detection capability, by counting the number of distinct bugs they detect within a fixed number of test inputs when used to test real-world deep learning compilers.

Furthermore, to better measure various aspects of generated inputs, 
\rev{we inherit the coverage criteria from previous research work~\cite{DBLP:conf/icse/LuoCRWFC21} and expand upon them to measure the diversity of computation graphs, including types, tensor shapes, and attributes of operations as well as connections between operations.
The design of these coverage criteria is motivated by the
fact that (1) existing traditional code coverage criteria are ineffective in deep learning testing~\cite{DBLP:conf/icse/LuoCRWFC21}, and neuron coverage criteria~\cite{DBLP:conf/sosp/PeiCYJ17} are also invalid in our evaluation because compiler testing involves different input models, and (2) type and shape problems are major root
causes of deep learning compiler bugs as demonstrated in a recent study~\cite{DBLP:conf/sigsoft/ShenM0TCC21}, also, (3) a lot of high-level optimizations in deep learning compilers, which are error-prone due to continuous and frequent development and modifications~\cite{DBLP:conf/sigsoft/ShenM0TCC21, du2021empirical}, could only be triggered by different types of specific connections between operations in the computation graphs~\cite{HirGen}.
}

%\rev{To capture diversity of generated models, we inherit the metrics from previous research work~\cite{DBLP:conf/icse/LuoCRWFC21} and expand upon them.
%including data types, shapes, and operations.}

\rev{Specifically,} we design 11 types of metrics for measuring coverage among input space.
The metrics are of two major categories: graph-level metrics and operation-level metrics. 
For operation-level metrics, we mainly follow the work by ~\cite{DBLP:conf/icse/LuoCRWFC21}.
For graph-level metrics, we design them with analogy of concepts in structural code coverage and combinatorial testing. Besides the preceding metrics, we also count the frequency of occurrences for operations and calculate the distribution of operations. 

% \vspace{1cm}

\subsubsection{Graph-level metrics}
\rev{Graph-level metrics are designed for measuring various aspects of a single generated model.}
Let a \textbf{test set} be the set of models generated by an  approach. Given a test set $I$, which contains $n_I$ graphs, the graph-level metrics are defined as follows. 

%An \textbf{operation corpus} is a set of operations and their attributes including operation name, possible number of different input degrees and output degrees. %In this work, we construct the operation corpus using the \opnumber{} operations mentioned above.

%Considering that each model is a computation graph, besides the operator-level coverage metrics, we also propose the graph-level metrics to present the quality of the models generated by our approach, compared with the baselines. %
%\Ziheng{similar formulas, can they be merged?}

\textbf{Number of Operations (NOO)} of a graph $g$ is defined as the total number of operations in $g$. 
\textbf{Number of Operation Types (NOT)} of a graph $g$ is defined as the number of different types of operations in $g$. 
\textbf{Number of Operation Pairs (NOP)} of a graph $g$ is defined as the number of different edges in $g$ that connect two operations together. 
\textbf{Number of Operation Triples (NTR)} of a graph $g$ is defined as the number of different pairs of adjacent edges that connect three operations together in $g$.   
\textbf{Number of Shapes and Attributes (NSA)} of a graph $g$ is defined as the total number of different shapes of input tensors and attributes (except for its input dgrees) for each operation in graph $g$. 
These graph-level metrics for test set $I$ are defined as the average of each of them among all the graphs in $I$: $GLM(I) = \frac{\Sigma_g{GLM_g(g)}}{n_I}$, where $GLM \in \{NOO, NOT, NOP, NTR, NSA\}$.

%We put these metrics together because they all represent the diversity of a computation graph.
% The NOO  The NOT  The NOP  The NTR 
% The NSP 
% These metrics for test set $I$ are defined as the average of each of them of allthe graphs in $I$: $NXX(I) = \frac{\Sigma_g{NXX_g(g)}}{n_I}$, where $NXX \in \{NOO, NOT, NOP, NTR, NSP\}$.
%$NOO(I) = \frac{\Sigma_g{NOO_g(g)}}{n_I}$, $NOT(I) = \frac{\Sigma_g{NOT_g(g)}}{n_I}$, $NOP(I) = \frac{\Sigma_g{NOP_g(g)}}{n_I}$, $NSP(I) = \frac{\Sigma_g{NSP_g(g)}}{n_I}$.%

% \textbf{Number of Operations (NOO)}.
% This metric presents the size of a computation graph. The NOO of a graph $g$ is defined as the total number of operations in $g$. The NOO of $I$ is defined as the average of NOO of all the graphs in $I$: $NOO(I) = \frac{\Sigma_g{NOO_g(g)}}{n_I}$.

% \textbf{Number of Operation Types (NOT)}. 
% This metric shows the diversity of operations in a graph. The NOT of a graph $g$ is defined as the number of different types of operations in $g$. Similar to NOO, the NOT of $I$ is defined as the average of NOT of all the graphs in $I$: $NOT(I) = \frac{\Sigma_g{NOT_g(g)}}{n_I}$.
% %let $n_{op}(g)$ be the number of different types of operations, and $n_g$ be the number of all the operations in $g$, the NOT of $g$ is defined as the ratio of $n_{op}(g)$ and $n_g$: $NOT_g(g)=\frac{n_{op}(g)}{n_g}$. The NOT of $I$ is then defined as the average of NOT of all the graphs in $I$: $NOT(I) = \frac{\Sigma_g{NOT_g(g)}}{n_I}$.%

% \textbf{Number of Operation Pairs (NOP)}.
% This metric shows the diversity of edges in a graph. The NOP of a graph $g$ is defined as the number of different edges in $g$ that connects two operations together. The NOP of $I$ is defined as the average of NOP of all the graphs in $I$: $NOP(I) = \frac{\Sigma_g{NOP_g(g)}}{n_I}$.
% %Suppose that each operation could be directed to all types of operations appearing in the graph, the NOP of $g$ is defined as the ratio of $n_{e}(g)$ and $n_g^2$: $NOT_g(g)=\frac{n_{e}(g)}{n_g^2}$. As with the definition of NOT, the NOP of $I$ is defined as the average of NOP of all the graphs in $I$: $NOP(I) = \frac{\Sigma_g{NOP_g(g)}}{n_I}$.Note that if a node is connected to the output of the entire model, we% 

% \textbf{Number of Shapes and Parameters (NSP)}.
% This metric shows the diversity of shapes of tensors and parameters in a graph. The NSP of a graph $g$ is defined as the number of different shapes of input tensors and parameters for each operation in graph $g$. The NSP of $I$ is defined as the average of NSP of all the graphs in $I$: $NSP(I) = \frac{\Sigma_g{NSP_g(g)}}{n_I}$.

%\Luyao{I think we could remove this metric.}\Ziheng{I think so.} We also use the \textbf{Density (DST)} of graphs as one of our graph-level metrics. Given a graph $g$, the density of $g$ is defined as the ratio between the edges present in a graph and the maximum number of edges that the graph can contain. i.e., $DST_g(g)=\frac{E}{N(N-1)/2}$, where E is the number of edges and N is the number of nodes.
%\Ziheng{reference to the definition; directed graph shouldn't have 2 in the formula. Also, our generated graph has constraints of input and output, maximum num of edges possibly isn't n*(n-1)/2}

% Given a graph $g$ and an input tensor $t$ of the model, we call a route that $t$ goes along from the input to the output of the model a \textbf{Path} of tensor $t$ in $g$.
%Note that there may be more than one route from an input tensor $t$ to the output of the model  and we take them as different paths. 
% We define graph-level metric Max Length of Paths (MLP) based on the paths in the computation graph.
% The Max Length of Paths (MLP) of a graph $g$ is the length of the longest path in it.\Ziheng{can we explain why we don't define path metrics like avglen, numlens?}
% as \textbf{Number of Tensor Paths (NTP), , Average Length of Paths (ALP)}. The detailed definitions of these three metrics are shown in our project website~\cite{israproject}. \Luyao{refine: @ziheng}

% \textbf{Number of Tensor Paths (NTP)}.
% The NTP of a graph $g$ is  defined as the number of different paths in $g$. The NTP metric shows the number of different manipulations of an input tensor, which indicates the complexity of a model. The NTP of $I$ is defined as the average of NTP of all the graphs in $I$: $NTP(I) = \frac{\Sigma_g{NTP_g(g)}}{n_I}$.

% \textbf{Max Length of Paths (MLP)}.
% Given a path $p$ in a graph $g$, the length of $p$ is defined as the number of operations in this path. The MLP metric and the ALP metric below present the depth of the model. The MLP of graph $g$ is defined as the length of the longest path in $g$. The MLP of $I$ is defined as the average of MLP of all the graphs in $I$: $MLP(I) = \frac{\Sigma_g{MLP_g(g)}}{n_I}$.

% \textbf{Average Length of Paths (ALP)} of graph $g$ is defined as the average of the lengths of all the paths in $g$: $ALP_g(g) = \frac{\Sigma_p{len(p)}}{n_p}$, where $p$ is a path in $g$ and $n_p$ is the number of different paths in $g$. The ALP of $I$ is defined as the average of ALP of all the graphs in $I$: $ALP(I) = \frac{\Sigma_g{ALP_g(g)}}{n_I}$.


% \textbf{Graph-level Metric (GLM)}.
% For each graph $g$, the Graph-level Metric of $g$ is defined as the weighted mean of the metrics defined above for $g$:
% \begin{equation}\label{eq:GLM_g}
% {GLM}_{g}(g) = \frac{\Sigma_i{{w_{g}[i]}{M_{g}[i]}}}{\Sigma_i{w_{g}[i]}}, 
% \end{equation}
% where $w_{g}$ are non-negative weights,  $M_{g}=\{{{NOO}_{g}(g)},$ ${{NOT}_{g}(g)}, {{NOP}_{g}(g)}, {{NTP}_{g}(g)},
% {{MLP}_{g}(g)}, {{ALP}_{g}(g)}\}$.

% Similarly, the GLM of test set $I$ is defined as the weighted mean of the metrics defined above for $I$:
% \begin{equation}\label{eq:GLM}
% {GLM}(I) = \frac{\Sigma_i{{w_i}{M_i}}}{\Sigma_i{w_i}}, 
% \end{equation}
% where $w$ are non-negative weights,  $M=\{{{NOO}(I)},$
% $ {{NOT}(I)},{{NOP}(I)},{{NTP}(I)}, {{MLP}(I)}, {{ALP}(I)}\}$.

% --------------------------------------------------------
% --------------------------------------------------------
% --------------------------------------------------------
\subsubsection{Operation-level metrics}
\rev{Operation-level metrics are designed for measuring various aspects of operations among the whole test set.}
An \textbf{operation corpus} is a set of operations with their attributes including the operation name and the possible number of different input degrees. 
Given an operation corpus $C$ containing $n_C$ different operations and a test set $I$, 
we first calculate the metric on each type of operator $o$ in $I$, denoted as $XXC_{op}(o)$, then we have the operation-level metric of $I$ as the average of the operation-level metric on different operators, i.e., $XXC(I)=\frac{\Sigma_o{XXC_{op}(o)}}{n_C}$, where $XXC\in\{OTC,IDC,ODC,SEC,DEC,SAC\}$. We simply explain the meanings of these six metrics as below, and detailed definitions of these operation-level metrics are shown in our project website~\cite{israproject}.
  
\textbf{Operation Type Coverage (OTC)}, \textbf{Input Degree Coverage (IDC)}, \textbf{Output Degree Coverage (ODC)} show the diversity of operations types, and the diversity of the input and output degrees of them in the test set $I$ respectively. 
% Note that for operations that have infinite numbers of input degrees (e.g. \texttt{Max}), we set an upper bound as their max input degree.
% We also set an upper bound for the output degrees of an operation.
\textbf{Single Edge Coverage (SEC)} shows the diversity of edges between the operations in $I$.
\textbf{Double Edge Coverage (DEC)} shows the diversity of pairs of edges that are adjacent, which is actually the coverage of different triples of operations that are connected in a graph in the test set.
\textbf{Shapes and Attributes Coverage (SAC)} indicates the diversity of attributes of the operations (except for input degrees) and their input tensor shapes in the test set. 

% The results of our experiments on coverage measurement are shown in Table\ref{tab:1_200}.

% The operation-level metrics contains \textbf{Operation Type Coverage (OTC), Input Degree Coverage (IDC), Output Degree Coverage (ODC), Single Edge Coverage (SEC), Double Edge Coverage (DEC) and Shapes and Parameters Coverage (SPC).}
% An \textbf{operation corpus} is a set of operations with their attributes including the operation name and the possible number of different input degrees. Given an operation corpus $C$ containing $n_C$ different operations and a test set $I$, 
% we first give the definition of each metric on an operator $o$ in $I$, denoted as $XXC_{op}(o)$, and the operation-level metric of $I$ is defined as the average of the metric on different operators, i.e.,  $XXC(I) = \frac{\Sigma_o{XXC_{op}(o)}}{n_C}$, where $XXC \in \{OTC,IDC,ODC,SEC,DEC,SPC\}$.
% Detailed definitions of these operation-level metrics are also shown in our project website~\cite{israproject}.

% \textbf{Operation Type Coverage (OTC)} shows the diversity of operations in the test set $I$. Let ${OTC}_{op}(o)$ be 1 if operation $o$ appears in $I$, and 0 otherwise. %The OTC of test set $I$ is defined as ${OTC}(I)=\frac{\Sigma_o{OTC}_{op}(o)}{n_C}$.%


% \textbf{Input Degree Coverage (IDC)} shows the diversity of the input degrees of the operations in the test set. For each operation $o$ in $I$, let $n_{id}(o, I)$ and $n_{id}(o, C)$ be the number of different input degrees of $o$ in $I$ and in $C$ respectively, we have the IDC of the operation $o$ as the ratio of $n_{id}(o, I)$ and $n_{id}(o, C)$: ${IDC}_{op}(o) = \frac{n_{id}(o, I)}{n_{id}(o, C)}$. %The IDC of $I$ is defined as ${IDC}(I) = \frac{\Sigma_{o}{IDC}_{op}(o)}{n_C}$.%
% For operations that have infinite numbers of input degrees  (e.g. \CodeIn{Max}), we set an upper bound for their $n_{id}(o, C)$.

% \textbf{Output Degree Coverage (ODC)} shows the diversity of output degrees of operations in $I$. 
% %The output degree of an operation is often correlated with the number of times its output tensor is reused, and it helps to prove our method to be efficient in reusing generated tensors. %
% The ${ODC}_{op}(o)$ is defined as the number of different output degrees of $o$ in $I$. %The ODC of $I$ is defined as ${ODC}(I) = \frac{\Sigma_{o}{ODC}_{op}(o)}{n_C}$.%
% %The ODC of operation $o$ is defined asbe the number of different output degrees of $o$ in $I$ and in $C$ respectively, we have the ODC of the operation $o$ as ${ODC}_{op}(o) = \frac{n_{od}(o, I)}{n_{od}(o, C)}$. Similarly, the ODC of $I$ is defined as ${ODC}(I) = \frac{\Sigma_{o}{ODC}_{op}(o)}{n}$.Note that the reuse times of an output tensor could be infinite, we also define an upper bound for the number of different output degree in $C$.
% %

% \textbf{Single Edge Coverage (SEC)} shows the diversity of edges between the operations in $I$. Let $n_e(o, I)$ be the number of different edges directed from the operation $o$ in $I$. Supposing that each operation could be connected with all operations in $C$,  we define the SEC of $o$ as the ratio of $n_e(o, I)$ and $n_C$: ${SEC}_{op}(o) = \frac{n_e(o, I)}{n_C}$. %The SEC of $I$ is defined as $SEC(I) = \frac{\Sigma_{o}{SEC}_{op}(o)}{n_C}$.%

% \textbf{Shapes and Parameters Coverage (SPC)} indicates the diversity of input and output tensor shapes of the operations in the test set. The ${SPC}_{op}(o)$ is defined as the number of different input tensor shapes and parameters of  $o$ in $I$. %The SPC of $I$ is defined as $SPC(I) = \frac{\Sigma_{o}{SPC}_{op}(o)}{n_C}$.%
% %Let $N_{SP}$ be the upper bound for the total number of different tensor shapes and operation attributes, and let $n_{SP}(o, I)$ be the number of different input tensor shapes and attributes of operation $o$ in $I$. Then the SPC of $o$ is defined as the ratio of $n_{SP}(o, I)$ and $N_{SP}$: ${SPC}_{op}(o) = \frac{n_{SP}(o, I)}{N_{SA}}$, and the SPC of $I$ is defined as the average of SPC of all the operations in $I$: $SAC(I) = \frac{\Sigma_{o}{SPC}_{op}(o)}{n}$.%


% \textbf{Operation-level Coverage (OLC)}.
% For each operation $o$, the Operation-level coverage of $o$ is defined as the weighted mean of the metrics defined above for $o$:
% \begin{equation}\label{eq:OLC_op}
% {OLC}_{op}(o) = \frac{\Sigma_i{{w_{op}[i]}{M_{op}[i]}}}{\Sigma_i{w_{op}[i]}}, 
% \end{equation}
% where $w_{op}$ are non-negative weights,  $M_{op}=$ $\{{{OTC}_{op}(o)}, {{IDC}_{op}(o)},{{ODC}_{op}(o)},
% {{SEC}_{op}(o)}, {{SAC}_{op}(o)}\}$.

% Similarly, the OLC of test set $I$ is defined as the weighted mean of the metrics defined above for $I$:
% \begin{equation}\label{eq:OLC}
% {OLC}(I) = \frac{\Sigma_i{{w_i}{M_i}}}{\Sigma_i{w_i}}, 
% \end{equation}
% where $w$ are non-negative weights,  $M=\{{{OTC}(I)},$
% $ {{IDC}(I)},{{ODC}(I)}, {{SEC}(I)}, {{SAC}(I)}\}$.


%\input{tables/table4}
%\input{tables/table_bugs}
%\input{tables/table_pickrate}
% \input{tables/table_1_30_10000}


\input{tables/table_1_200_10000}

\subsection{RQ1: Evaluation Results of Generated Inputs}


% For the first experiment, we run each approach to generate a fixed number of valid deep learning model to test compilers and compare with the total time they used. In our experiment, we set the fixed number as 100. The less time the approach used means the higher performance of generating valid models. The result is shown as Table~\ref{tab:exper}. 

%We also measure the coverage information. The result of coverage for each approach is low and fairly closed. We suspect this is because the XXXXXXX.
\subsubsection{Operation-level metrics}
The result of experiment on coverage measurement is shown in Table~\ref{tab:1_200}. Firstly, with alignment on the number of generated inputs,
we can find that \toolname{} outperforms the baselines greatly with respect to the amount of time, showing the efficiency of our approach.

For operation-level metrics, we find that \toolname{} is able to cover all kinds of operations that we have chosen and all kinds of input degrees of each type of operation. Compared with the two baselines,  \toolname{} has higher coverage on all of operation-level metrics, especially for $SEC$, $DEC$, and $SAC$.

\subsubsection{Graph-level metrics}
We find that the $NOO$ (Number of Operations) of our approach and \btwoshort{} are closer to the average of the lower bound and upper bound of the operation numbers that we set (consistent with our uniform sampling for the number of operations), while
\boneshort{}'s $NOO$ remains at a significantly lower level. The reason is that \boneshort{} holds less probability to satisfy the semantic specifications, which leads to generating rather simple models and bad performance on the graph-level metrics. 
\btwoshort{}'s $NOP$ and $NTR$ are comparable with our approach, however, the operation types ($NOT$) of \toolname{} are more diverse, making it outperform \btwoshort{} at coverage of operation pairs ($SEC$) and triples ($DEC$). 
% \btwoshort{}'s incremental way of generation makes it hard to satisfy the tensor structural constraints when appending a new operation into the model, since the input shape of the new operation is generated randomly. This results in a lower 
The results of graph-level metrics indicate that \toolname{} are capable of generating diverse, large and complex models.
% while the models generated by \btwoshort{} are of smaller depth (see ALP). The reason is that the models generated by it are relatively wide, since incrementally expanding a model is easier to pass the check by adding a new input tensor into the model rather than matching with an existing one. As \toolname{} performs better in the metrics of NTP, MLP and ALP, the result indicates that \toolname{} is able to generate models of higher  complexity and deeper depths. \Ziheng{to refine,NTR?}




\subsubsection{\pre{Diversity} \rev{Distribution of Operation Frequency}}
As shown in Figure~\ref{fig:chart}, \rev{Figure~\ref{fig:withMuffin}, and Figure~\ref{fig:withNNSmith},}
% \rev{and Figure~\ref{fig:chart2},}
\toolname{} is able to generate different operations in a relatively uniform distribution, which is consistent with our uniform sampling for picking the type of operation. As a contrast, \pre{both of \boneshort{} and \btwoshort{}}\rev{all of baselines} fail to generate a sufficient number of operations with relatively complicated semantic specifications such as \CodeIn{Conv} and \CodeIn{Gemm}. It shows that \pre{\boneshort{} and \btwoshort{}} \rev{all of baselines} have a limitation that the diversity of models generated by them is weak. This is because the constraints of some operations are relatively
complicated and less possible to satisfy. Those complex operations are less possible to be chosen in the valid output by the filter of the \rev{iterative} checking process. \rev{Besides, among models generated by Muffin,
\CodeIn{reshape} operation appears most frequently because Muffin forces the insertions of \CodeIn{reshape} operation before many operations to ensure semantic specifications.}

\begin{figure}
    %\vspace{-18mm}
    \includegraphics[width=\linewidth]{imgs/1_200_097_10000.png}
    \caption{Distribution of Operation Frequency of \toolname{}  \pre{and the baselines} \rev{, \boneshort{}, and \btwoshort{}} (captioning only parts of operations in x-axis for a clear presentation, numbers at y-axis are normalized with the total number). \pre{Muffin is not included due to the difference on the supported operation set.}}
    \label{fig:chart}
    %\vspace{-4mm}
\end{figure}

\begin{figure*}
% \begin{figure}
\vspace{-4mm}
\begin{minipage}{\textwidth}
    %\centering
    \begin{minipage}[]{0.49\textwidth}
    \includegraphics[width=\linewidth]{imgs/distributionMuffin.png}
    % \includegraphics[width=\linewidth]{imgs/distributionMuffin.png}
    \vspace{-7mm}
    \caption{\rev{Distribution of Operation Frequency of Isra* and Muffin.}}
    \label{fig:withMuffin}
    \end{minipage}
    \hfill
    \begin{minipage}[]{0.49\textwidth}
    \includegraphics[width=\linewidth]{imgs/distributionNNSmith.png}
    % \includegraphics[width=\linewidth]{imgs/distributionNNSmith.png}
    \vspace{-7mm}
    \caption{\rev{Distribution of Operation Frequency of Isra** and NNSmith.}}
    \label{fig:withNNSmith}
    \end{minipage}

    % \vspace{-1cm}
\end{minipage}
% \end{figure}

% \label{fig:chart2}
% \caption{\rev{Distribution of Operation Frequency of Isra* and Muffin (left), Isra** and NNSmith (right).}}

\vspace{-5mm}
% \vspace{10mm}
\end{figure*}


%but NOO on Baseline \uppercase\expandafter{\romannumeral1}  is much smaller, indicating that Baseline I is weak for generating larger models. 

%Baseline\uppercase\expandafter{\romannumeral2}  is better than the Baseline\uppercase\expandafter{\romannumeral1}  on performance because of the incremental construction


% Note that although the models generated by Baseline \uppercase\expandafter{\romannumeral1}  are small in size, they can also cover all of the \opnumber{} operation types and have relatively deep paths in each model. We speculate the reason to be that Baseline \uppercase\expandafter{\romannumeral1}  tends to generate models with inputs that have small dimensions, making the manipulations performed on input tensors much simpler, since the shape of tensors is not changed. Thus it is easier to generate operation nodes that should have been more complex. The NSP metric helps us to confirm this speculation. 

% The reason that Baseline \uppercase\expandafter{\romannumeral2}  performs better than \toolname{} on NSP is that the models generated by Baseline \uppercase\expandafter{\romannumeral2} are relatively wide, leading to much more different input tensor shapes while our approach tends to reuse the shapes of tensors.

% Both of the two baselines face the problem of  lacking diversity for input generation. The result in Figure~\ref{fig:chart} shows that \toolname{} is able to generate different operations in a relatively uniform distribution. Both baselines fail to generate a sufficient number of operations with relatively complicated semantic specifications such as  \CodeIn{Conv} and \CodeIn{Gemm}. %Besides, Baseline\uppercase\expandafter{\romannumeral2}  also performs poorly in generating operations with multiple inputs like \textbf{Sum} and \textbf{Max}.

\begin{table}
      %\captionof{table}{Results of Sensitivity Experiment of $picking\ rate$.}
      %\vspace{-5mm}
      \centering 
      \input{tables/pickr}
\end{table} 

% \vspace{1cm}

\subsubsection{$picking\ rate$} To evaluate the effect of $picking\ rate$ parameter, we also compare the results of \toolname{} with the setting of different $picking\ rates$. The settings are the same as the experiment on coverage measurement, except that we set the operation number in the graphs as a fixed number 100.
The result is shown in Table~\ref{tab:pickrate}.
%We see that as the $picking\ rate$ increases, the number of connections of operations (NOP) increases as well but the number of different tensor shapes and parameter (NSP) goes down. The reasons are as follows.
If the $picking\ rate$ is relatively high, the operations are more likely to be matched with existing tensors, leading to $NOP$, $NTR$ going high. In the meanwhile, the shape of newly created tensors is more likely to be equal to the shape of previous tensors, leading to the result that $NSA$ goes down as the $picking\ rate$ increases. We finally choose its value as 0.97, as a trade-off.


%\Ziheng{Do we need to take generation time into consideration? i.e., acceptable extra overhead considering the higher metrics; time nearly the same when the pickrate is high enough}\Luyao{not necessary, the spend time is close, and much less comparing to test time.}

% Overall, the evaluation results show that our approach is both effective and efficient to generate valid, diverse, and relatively complex deep learning models.


% \begin{minipage}{\textwidth}
%     \begin{minipage}[b]{0.48\textwidth}
%       \centering
%       %\captionof{table}{Results of Sensitivity Experiment of $picking\ rate$.}
%       %\input{tables/pickr}
%       \includegraphics[width=\linewidth]{imgs/1_200_097_10000.png}
%     \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.48\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{imgs/1_200_097_10000.png}
%     %\captionof{figure}{\rev{The overlaps of bugs among different approaches on testing TVM.}}
%     % \captionof[figure]{Distribution of Operation Frequency of \toolname{} and the baselines (captioning only parts of operations in x-axis for a clear presentation, numbers at y-axis are normalized with the total number). Muffin \pre{is} \rev{and NNSmith are} not included due to the difference on the supported operation set.}
%     \label{fig:chart}
%   \end{minipage}
% \end{minipage}


% \begin{minipage}{\textwidth}

\begin{figure*}
\vspace{3mm}
    \begin{minipage}[]{0.53\textwidth}
      \captionof{table}{\# unique bugs detected on different compilers.}
      \input{tables/nofbugs}
    \end{minipage}
  \hfill
  % \noindent
  \begin{minipage}[]{0.4\textwidth}
    \centering
    \includegraphics[width=\linewidth]{imgs/overlap.drawio.png}
    \captionof{figure}{\rev{The overlaps of detected bugs among different approaches on testing three compilers (red for TVM, green for Glow, blue for SophGo).}}
    \label{fig:overlap}
  \end{minipage}
  % \vspace{-2mm}
\end{figure*}








% \begin{figure}[htbp]
% % \floatsetup{heightadjust=all, floatrowsep=columnsep}
% \newfloatcommand{figurebox}{figure}[\nocapbeside][\dimexpr(\textwidth-\columnsep)/2\relax]
% \newfloatcommand{tablebox}{table}[\nocapbeside][\dimexpr(\textwidth-\columnsep)/2\relax]

% \begin{floatrow}[2]
% \tablebox{\caption{Table}}{%
%   \begin{tabular}{|c|c|}
%     \hline
%     aa & bb \\ \hline
%     cc & dd \\ \hline
%   \end{tabular}}
% \figurebox{\caption{Image}}{%
%   \includegraphics[width=3cm]{example-image-1x1.pdf}}%

% \end{floatrow}
% \end{figure}



\subsection{RQ2: Evalution Results on Bug-Detection Capability}

We investigate the effectiveness of \toolname{} and baselines in terms of distinct bugs detected in the same version of compiler subjects. % We conduct the experiment for bug detection for comparing \toolname{} with baselines on the same benchmarks. 
%\toolname{} reports XX warnings in total, with YY as false positives, whose percent is fairly low.\Luyao{remove this maybe.}
After analysis of deduplication, \toolname{} detects \bugnumber{} unique bugs in total, \rev{as shown in Table~\ref{tab:bug_number}, } \pre{outperforming} \rev{performing better or as well than} baselines on all of three benchmarks.
The capability on bug detection shows the high effectiveness of \toolname{}.
\pre{The details of all of the detected bugs can be found on our project website~\cite{israproject}.}
\rev{To further evaluate bug-detection capability of \toolname{}, we conduct a study on the bugs \toolname{} detected.}
%Table~\ref{tab:bugs} presents the overall results.
% All reported bugs can be found on GitHub issues according to the provided issue IDs.\footnote{We eliminate the issue number in the Table~\ref{tab:bugs} according to the blind for anonymous review.}
%\footnote{\url{https://github.com/apache/tvm/issues}}
%\footnote{\url{https://github.com/microsoft/onnxruntime/issues}}


% \input{tables/table_merge}

% \begin{figure}[htbp]
%   \centering
%   \begin{minipage}[t]{0.6\linewidth}  % 这里图片位置设置为[t]竖直优先
%       \centering
%       \label{fig:chart1}\includegraphics[width=\linewidth]{imgs/1_200_097_10000.png}
%       % [width=2in] 图片宽度设置为2英寸，这里也可以用厘米
%   \end{minipage}
%     \begin{minipage}[t]{0.6\linewidth}  % 这里图片位置设置为[t]竖直优先
%       \centering
%       \label{fig:chart2}\includegraphics[width=\linewidth]{imgs/withMuffin.png}
%       % [width=2in] 图片宽度设置为2英寸，这里也可以用厘米
%   \end{minipage}
%   \begin{minipage}[t]{0.6\linewidth}  % 这里图片位置设置为[t]竖直优先
%       \centering
%       \label{fig:chart2}\includegraphics[width=\linewidth]{imgs/withMuffin.png}
%       % [width=2in] 图片宽度设置为2英寸，这里也可以用厘米
%   \end{minipage}
%   \caption{Distribution of Operation Frequency of \toolname{} and the baselines (captioning only parts of operations in x-axis for a clear presentation, numbers at y-axis are normalized with the total number). \pre{Muffin is not included due to the difference on the supported operation set.} \rev{Isra* and Muffin, Isra** and NNSmith are seperated due to different operation sets.}}
%   \label{fig1:subfig2}
% \end{figure}



\addtocounter{footnote}{0}
\footnotetext{The number of NNSmith's detected unique bugs on TVM is different from the results in the NNSmith's paper~\cite{NNSmith} due to the different settings on the compiler versions and testing amount.}

\rev{
\subsubsection{Bug Study}
}

\pre{In addition, we categorize the bugs found by \toolname{} as two types} \rev{Among all of unique bugs detected by ~\toolname{}, we categorize them into two types based on the test oracles detecting them}: (1) \emph{error bug} (29 of \bugnumber{}) : the given input triggers an \rev{error,} crash or unexpected exception during compilation; (2) \emph{inconsistency bug} (4 of \bugnumber{}): the compiler executes the given input and terminates normally but the compiled model produces different outputs according to differential testing.
% Our result shows that 29 of \bugnumber{} bugs belong to \emph{error} type and 4 of \bugnumber{} bugs belong to \emph{inconsistency} type.

After we report found bugs to the corresponding community, compiler developers give responses for most of them, all with positive feedback.
Among all of bugs found by \toolname{}, there are \unknownbug{} previously unknown bugs.
Until now, a majority of our detected bugs (27 of \bugnumber{}) have already been fixed by developers, with 16 bugs directly owing to our bug reporting/pull requests, benefiting all the compiler users and their applications. 
\rev{One of TVM core developers replies with the following message for bugs reported by us\footnote{\url{https://github.com/apache/tvm/pull/7208\#issuecomment-754406762}}: ``These two errors that you generated were excellent real bugs with the importer and were very easy to understand and replicate with your post. If they're being auto-generated they look excellent!''}
The feedback from real-world developers is also strong evidence showing that \toolname{} is practical for testing real-world deep learning compilers and able to detect critical bugs in practice. % Some of bugs are already been fixed in the lastest version.


% \begin{itemize}
% 	\item \textbf{Error Bug} A error bug means the bug produces internal error during compilation. The error could be raised in any stage in compilers including frontend (e.g. parsing) and backend (e.g. optimization, code generation). In our reported bugs, 8 of 10 belong to this type.
% 	\item \textbf{Wrong-Result Bug} A wrong-result bug means the compiler executes the input and terminates normally but produces the wrong result on the output. This is usually caused by the incorrect implementation or optimization. This type of bug could be detected by differential testing. We reported them after manually inspecting the output and checking with the excepted result. In our reported bugs, 2 of 10 belongs to this type.
% \end{itemize}

% Although we carefully analyzed the error message and root cause of our founded bugs, we still reported 2 duplicated bugs. All of duplicate bugs shares the same root causes with other bugs we have found.


\rev
{
%\textbf{Bug Study.}
We list 24 previously unknown bugs (as well as bug reports) detected by \toolname{} in Table~\ref{unknownbugs}, including the stage of root causes, the time it takes to have the bug confirmed and fixed, and the GitHub issue ID~\footnote{For reference, the URLs of TVM's and Glow's bug reports are https://github.com/apache/tvm/issues/\#IssueID, and https://github.com/pytorch/glow/issues/\#IssueID. The URLs for SophGo's bug reports are internal and not publicly accessible.} for reference. The details of confirmed/fixed bugs are as follows.


%After finding bugs on TVM, we reported them to the corresponding compiler developers. All of following bugs whose issues/pull requests could be tracked on GitHub.
\textbf{TVM-1} is a bug in the compiler backend, caused by a pass named \CodeIn{DynamicToStatic} which should not be defined at optimization level 3. It will lead the internal error when the deep learning model contains operations such as \CodeIn{MatMul}, \CodeIn{Dropout}. After our reporting, developers reordered passes in the backend and lowered \CodeIn{DynamicToStatic} optimization level to fix it~\footnote{\url{https://github.com/apache/tvm/pull/7213}}.


%\footnote{\url{https://github.com/apache/tvm/issues/7200}}
%It takes 1 day for confirming the bug, and takes 10 days for fixing the bug.
\textbf{TVM-2} is a bug in the compiler frontend. The TVM developer has explained the cause of the bug and fixed it\footnote{\url{https://github.com/apache/tvm/issues/7202\#issuecomment-754372403}}: ``It's due to a bad assumption made in \CodeIn{PRelu} conversion about the input layout......Our current PRelu converter assumes that incoming data is in NCHW format and that the slope will have C total elements. Neither of these are actual requirements for ONNX \CodeIn{PReLu}.''
%It takes 1 day for confirming the bug, and takes 1 day for fixing the bug.



\textbf{TVM-3} and \textbf{TVM-4} are bugs in the compiler frontend. Some of parameters in \CodeIn{LpPool} and \CodeIn{LeakyRelu} operation in ONNX standard allow default value but it was not supported in TVM.

\begin{table}
%\vspace{-3mm}
\centering
      \input{tables/bugs}
\vspace{-3mm}
\end{table} 


%\footnote{\url{https://github.com/apache/tvm/issues/7241}}
%It takes 1 day for confirming the bug, and takes 6 months for fixing the bug.

%\footnote{\url{https://github.com/apache/tvm/issues/7244}}
%It takes 1 day for confirming the bug, and takes 1 day for fixing the bug.


%\textbf{\#5} This is a frontend bug. It is because that the input format of ONNX allows attribute p in LpPool with a default value 2 while the TVM was not supported. This bug has fixed by paper's first author and developers. %~\footnote{https://github.com/apache/tvm/pull/8866}

%\textbf{\#6} This is a frontend bug. It is because that the input format of ONNX allows attribute alpha in LeakyRelu operation with a default value 0.01 while the TVM was not supported. This bug has fixed by developers. %~\footnote{https://github.com/apache/tvm/pull/7259}


\textbf{TVM-5} is a bug in the compiler backend, which catches an edge case of the compiler's type checker as explained by a TVM developer\footnote{\url{https://github.com/apache/tvm/issues/7262\#issuecomment-911968074}}.
% https://github.com/apache/tvm/issues/7262
%\footnote{\url{https://github.com/apache/tvm/issues/7262}}
%It takes 6 months for confirming the bug.
%The developer from TVM has explained the cause of the bug: `` This is just that our type checker is very tough and we have an edge case.''

\textbf{TVM-6} and \textbf{TVM-7} are bugs in the compiler frontend. The former is due to that one of input tensors in \CodeIn{Gemm} operation can be optional by the standard but the TVM doesn't allow that behavior. The latter is due to the fact that ``\CodeIn{Split} operation is not dynamic inputs'' as explained by the compiler developer.
%This bug has fixed by developers~\footnote{https://github.com/apache/tvm/pull/7489}.

%~\footnote{https://github.com/apache/tvm/issues/7263}.
%It takes 8 months for confirming and fixing the bug.

%\textbf{TVM-7} is an error bug on the frontend due to the fact that ``\CodeIn{Split} operation is not dynamic inputs'' as explained by the compiler developer.

\textbf{TVM-8} is a bug in the compiler backend due to inconsistent specifications between different versions on \CodeIn{Squeeze} operation, causing erroneous implementation in the compiler.

%Developer explains the reason: ``This is due to the fact that the onnx squeeze is not dynamic.''.

%~\footnote{https://github.com/apache/tvm/issues/8889}.
%~\footnote{https://github.com/apache/tvm/issues/8890}.
%It takes 2 days for confirming the bug, and takes XX day for fixing the bug.


\textbf{TVM-9} is a bug in the compiler backend. The erroneous backend implementation causes the inconsistent outputs on a model containing \CodeIn{Flatten} and \CodeIn{ReduceL1} operation. Developers have not confirmed this bug, but it has been fixed in the next released version of the compiler.

\textbf{Glow-1} is a bug in the compiler backend due to that \CodeIn{ReduceSum} operation in the input model contains multi axis inputs and attributes.

%\textbf{TVM-10} and \textbf{TVM-11} ...
%\textbf{Glow-1} and \textbf{Glow-2} ...

%\textbf{\#12 (patch reviewing)} This is a wrong-result bug on the backend. The calculation of \CodeIn{LpPool} operation in ONNX Runtime is inconsistent with many other deep learning engines like TVM, PyTorch.

%\subsubsection{Bugs on the compiler named SophGo}
%Besides two open-source deep learning compilers, we also conduct \toolname{} on a commercial deep learning compiler from the company SophGo. It turns out \extrabugnumber{} bugs.



\textbf{SophGo-1} is a bug in the compiler frontend. The compiler does not support that the weight tensor of \CodeIn{Conv} operation is an input tensor. Developers do not fix this bug due to the reason that they suppose users take this parameter as a constant because this parameter usually does not change after deployment.

\textbf{SophGo-2} is a bug in the compiler backend. If the inputs of \CodeIn{Mean} operation are the same tensor, then the calculation of mean operation will throw exception due to the naming error.

\textbf{SophGo-3} is a bug in the compiler backend. \CodeIn{ReduceProd} operation will register a buffer, but buffer size has not been assigned which leads to the incorrect parameters in calculation and further causes the final result wrong.

\textbf{SophGo-4} is a bug in the compiler frontend due to erroneous parsing for \CodeIn{Pooling} operation.

\textbf{SophGo-5} is a bug in the compiler backend due to incorrect implementation on \CodeIn{Split} operation.

\textbf{SophGo-6} is a bug in the compiler backend. The compiler assumes the second input of \CodeIn{PRelu} holds a specific shape which is not consistent with the specification.

\textbf{SophGo-7} is a bug in the compiler backend. The compiler backend incorrectly covers the input data for the calculation on \CodeIn{Cos} operation, causing the wrong results of model's output.

\textbf{SophGo-8}, \textbf{SophGo-9}, and \textbf{SophGo-10} are bugs in the compiler frontend due to erroneous parsing for 
\CodeIn{Unsqueeze} operation, \CodeIn{Split} operation and \CodeIn{Gemm} operation. ONNX standard of some operations has changed after version 13. The compiler only implements old version and is not compatible with latest standard. Developers do not fix \textbf{SophGo-10} due to the same reason as \textbf{SophGo-1}.

\textbf{SophGo-11} is a bug in the compiler backend due to incorrect implementation on \CodeIn{Resize} operation.
}

% It contains another false positive case with wrong-result situation. Compiler produces wrong result due to the slight error amplifies by $Ceil$ operation.



% \subsubsection{Compiler Developers' Feedback}
% After we report our found bugs to the corresponding community, compiler developers give responses for most of them, all with positive feedback. A majority of reported bugs (27 of \bugnumber{}) have already been fixed by developers, benefiting all the compiler users and their applications. One of TVM core developers replies with the following message for bugs reported by us\footnote{\url{https://github.com/apache/tvm/pull/7208\#issuecomment-754406762}}: ``These two errors that you generated were \textbf{excellent real bugs} with the importer and were \textbf{very easy to understand and replicate} with your post. If they're being auto-generated they look excellent!'' The feedback shows that our reported bugs are critical to the compiler. The feedback from real-world developers is also strong evidence that \toolname{} is practical for testing real-world deep learning compilers and able to detect critical bugs. 


% -------------------------------------
%There are 2 of our reported bugs are already confirmed by developers but still in the stage of patch review. Developers are discussing how to fix them. Overall, our reported bugs received positive feedback from deep learning compiler community that shows our tool is practical and could indeed benefit deep learning compilers in the real world.


% \section{Threats to Validity}

% Although we planned this work carefully, several threats still exist.

% First, We only implemented \opnumber{} common operations in ONNX, which is a subset of the whole operations in ONNX specification. There are some advanced features in ONNX specification that we have not implemented. Also, our settings on parameters limit the generated model size and tensor size. We may miss bugs triggered by larger model, larger tensor, or other unimplemented operations and features.

% Second, we only took three frequently-used deep learning compilers as our experimental objects. Our conclusion is only based on our testing results of these two compilers.

% \Luyao{remove this part if paper length is too long.}


\rev{
%\textbf{False positives.}
\subsubsection{False positives}
Though our test generation approach is sound (i.e., the models generated by our approach ensures the validity), false positives may be introduced by floating point errors~\cite{7194603, DBLP:journals/pomacs/XiaoLYPW22}.
For differential testing, one of test oracles we used,
when it comes to checking output equivalence,
false alarms may be produced due to floating point errors/inaccuracies.
To reduce false alarms, we use a high error tolerance in comparison of models' outputs (the relative error is set to 10\% as mentioned in Section~\ref{s4.2}), which is similar to a parallel work~\cite{NNSmith}.
In our evaluation, \toolname{} did not
find false positives caused by the floating-point errors.
%\TODO{bugs or features?}
}

\subsection{RQ3: Comparison with State-of-the-art Approaches}

We compare Isra with \pre{two} \rev{three} state-of-the-art approaches \rev{(i.e., Muffin~\cite{DBLP:conf/icse/GuLZ022}, TVMFuzz~\cite{DBLP:conf/sigsoft/ShenM0TCC21} and NNSmith~\cite{NNSmith})} in terms of coverage and bug detection capability.

For the comparison on coverage, as result shown in Table~\ref{tab:1_200}, \pre{under the same settings, compared with Muffin, \toolname{}* outperforms on most of metrics except for only $NTR$ and $NSA$.} \rev{(1) under the same settings, \toolname{}* outperforms Muffin on most of coverage metrics except for only $NTR$ and $NSA$,
and (2) under the same settings, \toolname{}** consistently outperforms NNSmith on all of coverage metrics. The reasons why Muffin achieves higher $NTR$ and $NSA$ than \toolname{}* are as follows.}
For $NTR$, this is mainly because Muffin contains a cells mode, which will favor generating dense graph structure which contains many triples, but its $DEC$ is still significantly low compared with Isra*, due to the fewer types of operations in per graph ($NOT$). Muffin's higher coverage on $NSA$ is
because Muffin inserts \CodeIn{Reshape} layers between adjacent layers for patching tensor structural constraints in a hardcode way, leads to change tensor shape frequently. However, Muffin is still significantly lower than \toolname{} on $SAC$, which is the coverage of $NSA$ among the whole test set. %The result shows that our approach outperforms Muffin in terms of generating models with higher coverage among the input space.


For the comparison on bug detection capability, 
\rev{as shown in Table~\ref{tab:bug_number}}, \toolname{} detects more bugs than Muffin on three compilers, with 1.5x, 2x, 1.22x respectively, in total 33 versus 23. Also, \toolname{} significantly outperforms TVMFuzz on detecting bugs on TVM with 18 versus 5.
\rev{\toolname{} achieves comparable results compared to NNSmith (33 versus 32) on three compilers.
In addition, we also investigate the overlaps of detected bugs among \toolname{}, Muffin, TVMFuzz, and NNSmith as shown in Figure~\ref{fig:overlap}.
There are overlapping bugs among them as well as distinct non-overlapping bugs, indicating that these approaches are complementary.
%feeding compilers with computation graphs.
%these test generation approaches all produce computation graphs 
There is no overlapping bug between TVMFuzz and other approaches, primarily because TVMFuzz fuzzes on low-level Relay IR instead of computational graphs.
}

% Note among all the detection bugs, there is no bug overlapping between \toolname{}'s and TVMFuzz's. The result indicates that \toolname{} could be complementary with TVMFuzz which is fuzzing on IR for detecting bugs on deep learning compilers.

\rev{
Overall, as shown in evaluation results, compared to state-of-the-art approaches under the same settings, \toolname{} outperforms those approaches on various coverage metrics, and also achieves comparable and complementary results on bug detection.
The results indicates that (1) \toolname{} is more effective and more efficient than existing approaches for test generation,
(2) \toolname{} is effective and complementary to existing approaches for detecting bugs in real-world compilers.

%There is XX bug overlapping between \toolname{}'s and Muffin's.

%The result indicates that these approaches could be complementary for detecting bugs on deep learning compilers.
}

% \input{tables/table_muffin_0.97_10000}

%\Luyao{remove this paragraph?} 


%\footnote{The paper of TVMFuzz~\cite{DBLP:conf/sigsoft/ShenM0TCC21} also conduct bug detection on TVM ``v0.8dev'', but the paper does not describe explicitly the specific version used for ``v0.8dev'', so we are unable to compare GenDice with TVMFuzz on ``v0.8dev''.},

%\toolname{} identifies 8 unique bugs during 1 hour, outperforming TVMFuzz, which identifies 5 unique bugs during 2 days~\cite{DBLP:conf/sigsoft/ShenM0TCC21}.


% TVMFuzz~\cite{DBLP:conf/sigsoft/ShenM0TCC21} conduct fuzzing on the Relay language (intermediate representation of TVM Compiler) for testing TVM compiler. Compared with it, \toolname{} has two difference:  For example, if new operations are added into compiler without testing coverage of existing test suite, \toolname{} could still conduct test to cover new operations' functionality but TVMFuzz is unable to test for them.




==> arXiv-2302.00842v2/sections/introduction.tex <==
\section{Introduction}
In recent years, deep learning has been widely used in software systems from various domains, such as autonomous driving, e-commerce, and smart cities.
%\Luyao{DL could run on XXX, but the performance is . In order to improve performance and energy, inference speed is slow.}
Given that deep learning models become increasingly large and complicated, there are emerging needs to deploy versatile deep learning models on different types of hardware such as GPU, FPGA, and TPU~\cite{DBLP:conf/isca/JouppiYPPABBBBB17}.
To reduce the burden of optimizing deep learning models and to address the difficulty of model deployment on hardware, deep learning compilers have been developed, such as TVM~\cite{DBLP:conf/osdi/ChenMJZYSCWHCGK18}, Glow~\cite{DBLP:journals/corr/abs-1805-00907},
%ONNX Runtime~\cite{onnxruntime},
and XLA~\cite{xla}.
%, and Tensor Comprehension~\cite{DBLP:journals/corr/abs-1802-04730}.
These deep learning compilers have been widely used for the optimization and deployment of deep learning models, especially those with critical performance requirements. 


%The orange part in Figure~\ref{fig:p1} shows an example deep learning model with two operations.
%The highly sophisticated two-part compilation process in deep learning compilers is bug prone, imposing high risk for all AI applications that use these compilers. 
%Deep learning compilers provide developers with end-to-end sophisticated two-part compilation to deploy pre-trained deep learning models on different backends.  
%Deep learning models could achieve better performance after the compilation of deep learning compilers. 
%Deep learning compilers mainly contain two parts of optimization:
%The first part of compilation is graph-level optimization, which contains processes such as rewriting the graph, fusing operators, and tuning parameters. The second part of compilation is operator-level optimization including synthesizing lower-level code that runs on different target hardware (e.g., GPU and  FPGA)~\cite{DBLP:journals/tpds/LiLLSYYLGYQ21}.


Testing a deep learning compiler is vital for two main reasons. First, if a deep learning compiler used by AI applications contains bugs, the deployed AI applications can exhibit serious failing behaviors. For example, a critical bug of TVM's SPIRV codegen led to incorrect results for a TVM-optimized model's output, which affected all users who use TVM for their model deployment on the Nvidia Vulkan backend\footnote{\url{https://github.com/apache/tvm/pull/8102}}. Second, the highly sophisticated compilation process in a deep learning compiler is error-prone. According to a very recent study~\cite{DBLP:conf/sigsoft/ShenM0TCC21}, during a time period of 15 months, there are 845 bug-fixing pull requests on the TVM project, including 318 bugs in total.

%
%Testing has been adopted in practice to find critical bugs and expose potential risk to improve the trustworthiness of compilers, and how to effectively construct test programs that are valid, diverse, and meet certain requirements is critical for testing compilers~\cite{DBLP:journals/csur/ChenPPXZHZ20}. 



% \yx{Why do we need this paragraph?} \Luyao{This paragraph is the background of deep learning model. We could remove it if it is not necessary.}


% To detect bugs in deep learning compilers, random testing, a practical way of automatic test generation, is a natural choice for three main reasons. First, random testing remains the most popular for compiler testing in practice ~\cite{DBLP:journals/csur/ChenPPXZHZ20}. Random testing has already shown great effectiveness in testing compilers of many languages ~\cite{DBLP:journals/pcs/KossatchevP05, DBLP:conf/icse/ChenHHXZ0X16}, such as Csmith and YARPGen~\cite{DBLP:conf/pldi/YangCER11, 10.1145/3428264} for C/C++, DeepSmith~\cite{DBLP:conf/issta/CumminsPML18} for OpenCL, Glade~\cite{DBLP:conf/pldi/Bastani0AL17} for Python, Ruby, and JavaScript. Second, it is a straightforward technique without bias, thus being able to test the system under test in unexpected ways ~\cite{DBLP:journals/jss/ChenKMT10}. 
% Previous work ~\cite{DBLP:conf/pldi/YangCER11, DBLP:conf/pldi/ZhangSS17, DBLP:conf/oopsla/SunLS16, DBLP:conf/oopsla/LeSS15} shows that bugs detected by random testing for compilers are often missed by existing human-written or well-designed test cases.
% Third, it may be the only practical choice when the source code under test or runtime information is unavailable or incomplete. For example, TVM is a fairly large project with about 400k+ lines of code, with language mixture (Python and C++), making techniques requiring code instrumentation hard to conduct.



%\Luyao{refine}

%Random testing is a black-box testing technique where the system under test is tested by generating random, independent inputs. Random testing is a straightforward technique, often easy to implement, without any bias, and has also been demonstrated to effectively detect bugs through testing the system under test in unexpected ways (which may not occur to a human tester)~\cite{DBLP:journals/jss/ChenKMT10}. It may also be the only practical choice when the source code or runtime information of the system under test is unavailable or incomplete. 

 %To reach core parts of a deep learning compiler, random testing needs to address the challenge of generating valid inputs,  
 % A compiler under test falls into the type of system system under test that is equipped with a well-defined input specification (e.g., the C99 grammar and defined-behavior input specification for a C compiler) and has also implemented pre-check (e.g., input-validation check to allow only valid inputs to pass through) for inputs. Testing such system poses challenges for random test generation, which holds high possibility of producing a large number of invalid inputs (inputs that do not satisfy the input specification), compromising the overall effectiveness and practicability of testing, because invalid inputs could not reach into core logic of the system under test and usually annoy developers with meaningless and duplicated exception information.
% Compiler testing contains several aspects including constructing test programs, choosing appropriate test oracles and how to execute compiler tests effectively. To construct test programs for compilers, there are various approaches including manually construction, grammar-based approaches, mutation-based approaches. Test oracles are to determine whether the behavior or output of a compiler is correct or not. The main approaches of test oracle are using differential-testing~\cite{DBLP:journals/dtj/McKeeman98} and metamorphic testing~\cite{chen2020metamorphic}. Besides, in order to optimize test-program execution time, some approaches have been proposed which mainly contain two directions: test-program prioritization and test-suite reduction.

%\Luyao{1. valid input? 2. test oracle. merge first two sentences.}
%\Luyao{intro the preconditions for mathematical operations.}
%\Luyao{computation graph -- move here.}
%\Luyao{error probabilty of precheck functionality is small.}


A deep learning model, as the input of a deep learning compiler, needs to satisfy semantic specifications in two aspects; otherwise, it will be rejected by the deep learning compilers at an early stage before invoking the actual core functionality of the compilers.
%The deep learning model also needs to satisfy certain constraints as we called semantic specification, pre-checked by the compilers. \Luyao{add acyclic specification here?}
First, a deep learning model is a neural network arranged as a directed and acyclic graph. Second, the model also needs to satisfy certain constraints, which are required by the operations in the model. For example, within a model, a \CodeIn{MatMul} operation (denoting matrix multiplication) with two input matrices (2-D tensors) requires that the number of columns in the first matrix is equal to the number of rows in the second matrix.



\iffalse
Existing work has already shown its great effectiveness in testing compilers of many languages ~\cite{DBLP:journals/pcs/KossatchevP05, DBLP:conf/icse/ChenHHXZ0X16}, such as Csmith~\cite{DBLP:conf/pldi/YangCER11} for C, YARPGen~\cite{10.1145/3428264} for C++, LangFuzz~\cite{DBLP:conf/uss/HollerHZ12} for JavaScript, and DeepSmith~\cite{DBLP:conf/issta/CumminsPML18} for OpenCL.
Also, previous work~\cite{DBLP:conf/pldi/YangCER11, DBLP:conf/pldi/ZhangSS17, DBLP:conf/oopsla/SunLS16, DBLP:conf/oopsla/LeSS15} shows that bugs detected by generator-based testing for compilers are often missed by existing human-written test cases.
\Luyao{add more data for generator-based testing.}
\fi
%It is scalable and may also be the only practical choice when the source code under test or runtime information is unavailable or incomplete. 

% For example, TVM is a fairly large project with about 400k+ lines of code, with language mixture (Python and C++), making techniques requiring code instrumentation hard to conduct.

%To generate highly-structured inputs for testing core compiler parts (achievable only by valid inputs),  
% To generate valid inputs for testing deep learning compiler,
%remains the most popular in practice~\cite{}.

%A deep learning model, as the input of deep learning compiler, can be regarded as a computation graph, essentially, a directed and acyclic graph with the model's operations or tensor placeholders as its nodes, and tensors as its edges. An example is shown in Figure~\ref{fig:p2}. The computation graph can be executed by feeding the specific data into tensor placeholders. In a computation graph, each operation denotes a mathematical function with tensor(s) as its input and output. The semantic specification of a computation graph (like the pre-condition of the function), specified from the definition of the operations, indicates which condition must be satisfied when executing the computation graph. 
%For example, a \CodeIn{MatMul} operation with two input matrices (2-D tensors) in a computation graph should ensure that the number of the columns in the first matrix is equal to the number of the rows in the second matrix\footnote{\url{https://docs.scipy.org/doc/numpy-1.13.0/reference/generated/numpy.matmul.html}}. The computation graph is valid only if it does not violate the semantic specifications, otherwise, the computation graph will not be accepted by deep learning compilers or fail to be compiled at a very early stage.


To test core compiler parts (achievable by only valid inputs),  
% To generate valid inputs for testing deep learning compiler,
one can indeed adopt random testing (the most popularly used technology for compiler testing practices~\cite{DBLP:journals/csur/ChenPPXZHZ20}) in a straightforward way: generating possible inputs and filtering them by checking against the semantic specifications\footnote{Checking against the semantic specifications can be in the form of a boolean checker such as \CodeIn{repOK}~\cite{boyapati02:korat}, etc.}, also called as declarative-style random test generation~\cite{boyapati02:korat, DBLP:conf/issta/ElkarabliehMK08, DBLP:conf/icst/GligoricGLMK09}; however, this style suffers from two main issues.
First, random testing in the declarative style has a fairly low probability of satisfying the semantic specifications, especially for complicated operations (as shown in our experimental results in Section~\ref{sec:evaluation}), wasting testing the budget on generating and checking many invalid inputs.
Second, valid inputs generated by this random testing strategy tend to be simple, as complex inputs have an even lower probability of satisfying the semantic specifications, whereas it is highly critical to also generate complicated models in order to achieve various testing goals.

%Third, the checking for validity still costs non-trivial extra running time.\tao{Please quote some stats from your experiments to support this point}

%, one can adopt two major straightforward test generation approaches based on random testing, which however waste testing budget on generating a large number of invalid models and checking them against the semantic specifications\footnote{Checking against the semantic specifications can be in the form of a grammar checker, a boolean function such as \CodeIn{repOK}~\cite{boyapati02:korat}, etc.}.  (1) Whole construction before checking in short as \textbf{whole checking}, where a whole deep learning model is randomly generated and then checked. This approach is ineffective because there is fairly low probability for a randomly generated model to  satisfy the semantic specifications. 
%(2) Incremental construction with checking in short as \textbf{incremental checking}, which, instead of constructing the whole model all at once, starts with an empty model and then incrementally and iteratively appends a new part (i.e., an operation) into the model. If the current work-in-progress model passes with checking against the  semantic specifications, the approach continues the appending process; otherwise, it discards the current work-in-progress model and restarts the same process starting with an empty model. 
% This approach is more effective than the whole checking approach but still suffers from two main issues: (1) valid models generated by this approach tend to be simple, and it is highly critical to also generate complicated models in order to achieve various testing goals, and (2) despite incremental, the checking for validity still costs non-trivial extra running time.



%Also, simply adopting other existing main categories of random testing faces limitation of generating valid inputs for testing DL compilers.
%The semantics of deep learning model cause existing test generation approach hard to generate valid deep learning model which further lose their efficacy of testing deep learning compilers.
%Grammar-based random testing~\cite{10.1145/1375581.1375607} is not adaquate here as semantic specifications of deep learning models cannot be easily captured by primitive grammars such as context free grammar. 
%Mution-based testing, as another category of random testing, has the limitation that it assumes existing various high-quality and representative testsuites which is not always true in practice, especially for latest produced compilers with new APIs that the number of its tests or users is relatively few.


%If we discard all of these semantic constraints and let all the operations and tensors produced by unguided random generation
%it will definitely produce a large number of invalid models, compromising the efficiency and practicability because purely randomly generated inputs have extremely low chance to reach core parts of compilers.

% Our experiments in evaluation part also proves it.\Luyao{add?}

% Our observation behind our work proposed in this paper is that  those constraints imposed on deep learning models could still probably be satisfied by subtle generation strategies. 


% \yx{Here you should follow the same storyline as Sect 2. First mention existing constraint sampling approach is those from Koushik Sen's group, but their approaches are limited by the constraints that could be easily solved by a constraint solver. However, the constraints have two characteristics (Scale and Complexity) that cannot be easily solved. We observe XXX, and then propose XXX. Then we observe XXX, then propose XXX.}

\iffalse
To effectively generate semantically valid inputs, in this paper, we propose to explicitly resolve constraints in the semantic specification during the test generation.\Luyao{the first sentence do not summary.}
However, to resolve constraints, existing techniques fail on account of
%With encoding the semantic specifications as logic constraints (as an example shown in Section~\ref{sec:s2}), test generation is equivalent to sampling solutions on the constraints.
two complex forms: (1) quantifiers such as $\forall x \in S, ...$ where $S$ is a set variable, and (2) unknown functions such as $f(x)=...$ where $f(x)$ is a function with an unknown domain (examples are shown in Section~\ref{sec:s2.2}). Such constraints are intractable to solve or sample because the first-order logic (with quantifiers in it) and the second-order logic (with unknown functions in it) is undecidable in general~\cite{turing1936computable}; also, in practice, existing solvers~\cite{DBLP:conf/tacas/MouraB08, DBLP:conf/iccad/DutraBS18} are limited when the constraints involve quantifiers and unknown functions.


To resolve issues of direct random test generation, an alternative perspective is to model the test generation as a constrained sampling problem. Taking the semantic specifications of computation graphs as logic constraints (as an example shown in Section~\ref{sec:s2}), test generation could be taken as sampling solutions on those constraints. In this way, our goal, i.e., effective test generation of computation graphs, is equivalent to efficiently sampling diverse solutions of constraints.
\fi
%To  generate both simple and complicated computation graphs without biased, an effective constrained sampler is critical.
%exclude the invalid computation graphs during the test generation,
%Because random test generation is not efficient, we take an alternative perspective to model the test generation as a constrained sampling problem, by explicitly specifying the semantic specifications of deep learning models. These specifications are expressed in first-order logic constraints, derived from conditions that valid computations must satisfy in deep learning. Each solution of the constraints corresponds to a valid deep learning model.
%Such explicit constraints make it possible for us to exclude the invalid deep learning models during the test generation by efficiently sampling solutions of the constraints. 

%Instead of random test generation with taking semantic specification as a blackbox, we could model the generation of valid deep learning models as a constrained sampling problem by taking the semantic specification as the constraints. Each solution of the constraints corresponds to a valid deep learning model. The constraints are expressed in the first-order logic instead of the propositional logic due to the existence of two forms: (1) quantifiers such as $\forall x \in S, ...$ where $S$ is a variable and (2) unknown functions such as $f(x)=...$ where $f(x)$ is a function with an unknown domain (shown in detail in Section~\ref{sec:s2.1}).
%For example, universal quantifier $i$ with an unknown domain (the domain of $i$ depends on $dim_A$) appears in Equation~\eqref{c5}, the unknown functions \yx{array or function?} appears as term $A[dim_A]$ and term $B[dim_B-1]$ in Equation~\eqref{c4} (functions of getting the length of last or last second dimension of a tensor).
%In general, it do not exist universal approaches to efficiently solve (or sample solutions of) the constraints that expressed in the first-order logic due to following reasons: (1) theoretically, first-order logic is undecidable in general~\cite{turing1936computable} \Luyao{add explanation of `undecidable' to `unable for sampling'?}; (2) practically, existing solvers ~\cite{DBLP:conf/tacas/MouraB08, DBLP:conf/iccad/DutraBS18} are limited when the constraints contain quantifiers and unknown functions.


To better conduct random testing on a deep learning compiler, we take the semantic specifications of a deep learning model as logic constraints; in this way, test generation is equivalent to finding solutions to the constraints. However, we face a challenge due to complex constraints, i.e., those related to both the graph structure of the model and operations within the model. Furthermore, within the constraints, the involved first-order/second-order logic (as shown in Section~\ref{sec:s2}) is  undecidable in general~\cite{turing1936computable} and causes existing solvers not to be able to encode, or perform efficiently ~\cite{DBLP:conf/iccad/DutraBS18, gradel2007finite}.

To address the preceding challenge, we propose a novel  approach named \toolname{} based on the following insight: 
%well properties of semantic specifications on deep learning models allow a proper instantiation order to resolve and simplify the constraints, towards effectively finding solutions.
the constraints on a deep learning model have certain properties, allowing us to iteratively resolve and simplify the constraints to effectively find solutions, by following a proper instantiation order.
We design two strategies in the core part of \toolname{}, a novel domain-specific constraint solver. Our solver conducts instantiation with an order for gradually resolving and simplifying constraints.
Based on the consistency among the constraints, \toolname{}, with our domain-specific constraint solver, is able to find semantically valid inputs without backtracking, while  ensuring both soundness (the generated inputs are semantically valid) and completeness (no loss for the probability of generating any valid model).

% by instantiation with the topological order of the graph
%Both of our two strategy conducts instantiation in a well-designed order to resolve constraints but in different levels.

%Specifically, first strategy, named \tone{}, is designed to resolve the whole constraints into separated parts; and second strategy is used as further resolving each separated part. 

%further simplifies the complex forms of constraints.
%\Luyao{mention eliminating quantifiers and unknown functions?}
% Generally, constraint solver may backtrack if the instantiation does not satisfy the constraints or apply some heuristic rules to reduce the search space without completeness guarantees (completeness means that it is able to generate any semantically valid model), both hurting the overall effectiveness for testing.

%For example, assume $S$ is a set variable, there is a constraint with a quantifier: $\forall x \in S, P(x)$. If we already instantiate the domain of $x$ (i.e., the value of $S$) such as $S=\{1,2,3\}$, then we could eliminate the universal quantifier by rewriting the constraints as follows: $\forall x \in S, P(x) \Longrightarrow P(1) \wedge P(2) \wedge P(3)$. 

%Based on this insight, we propose a layered instantiation technique with two stages to optimize the overall sampling process.
%For the first stage named graph-level instantiation, we gradually instantiate the structure of computation graph to eliminate the universal quantifier with the domain of the whole graph. In this way, first stage disassembles the whole sampling problem (for sampling a whole graph) into separated subproblems (for sampling an operation). 
%For the second stage named operation-level instantiation, our goal of this stage is to generate a specific operation. Our approach will further instantiate the parameters/input/output of operations in an iterative way with eliminating the quantifier and unknown functions in the meanwhile.
% For the second stage, we further conduct operation-level instantiation disassemble the sampling problem of an single operation to the several subproblems (for sampling an single tensor).
%Generally, to ensure the soundness (validity of generated results), constraint solver may backtrack if the instantiation does not satisfy the constraints, hurting the overall effectiveness. However, with two strategies we designed in \toolname{} (\tone{} and \ttwo{}), our instantiation-based solver is backtrack-free, guaranteed by the property of deep learning model's semantic specification. 
%In this way, \toolname{} effectively generates random and diverse deep learning models with both the soundness and completeness (no loss for the probability of generating any valid inputs). \Ziheng{What does the elimination and non-backtracking do with soundness and completeness?}

%With our analysis of the specification of deep learning models, we observe two key characteristics of the constraints we need to sample.
% distinguishes it from propositional logic, which does not use quantifiers
%and its domain depends on $dim_A$. In Equation~\eqref{c4}, the term  represents the length of last dimension of tensor $A$ and term  represents the length of last second dimension of tensor $B$, those terms contains unknown functions.
%Equation~\eqref{c5} (i.e. conducting quantifier elimination) due to the unknown of value $dim_A$. For the variable-length arrays such as $A$ and $B$ in Equation~\eqref{c4}, we could not explicate Equation~\eqref{c4} due to the unknown of value $dim_B$.

%existing constraint sampling approaches such as SMTSampler~\cite{DBLP:conf/iccad/DutraBS18} (based on SMT-Lib~\cite{barrett2010smt} and Z3 Solver~\cite{DBLP:conf/tacas/MouraB08}) face a major challenge when sampling solutions of the constraints (i.e., semantic specifications) on a deep learning model: the quantifiers with undetermined domains and the variable-length arrays in the constraints.


% The current SMT solver relies on some theories to solve quantified formulas and the array. However, when the domain of quantifier and the array is unknown, it causes difficulties to model them. We could of course enumerate all of possibilities in the domain, then transform the formula to quantifier-free on preliminary typed variables, however, this 


%
%taking the semantic specifications as the constraints on a deep learning model, the model construction can be formulated as a \textbf{constraint sampling problem}. To sample solutions of the constraints on the deep learning model,  are limited due to following two main reasons: 

%First, the scale of the constraints increases by the size of the generated deep learning models, leading to inefficient performance of sampling.

%\tao{Please add some supporting evidence or statement for the first point. Currently the argumentation is too thin}

%Second,  \textbf{quantifiers} such as $\forall i \in f(x)$ in Equation~\eqref{c5}, and \textbf{tensor structural constraints} (tensor structure refers to a variable-length array that denotes the structure of a tensor) such as the existence of the term $B[dim_B-1]$ in Equation~\eqref{c4} in the constraints cannot be directly modeled or efficiently solved by the  existing approaches.


%To address the challenge, we propose a new approach named \toolname{} to efficiently constructing diverse and valid deep learning models based on our observation that the constraints of models could be disassembled.

%Model-level acyclic trait means that the computation graph is acyclic, and the model's constraints could be decomposed to some separated sub-constraints.
%Consistency among tensors and Layered forms of variables are described as a running example in Section~\ref
%in Section~\ref{sec:approach}) is used for 
%is used for simplify the complicated constraints of deep learning models to a quantifier-free forms on 
%\tao{Luyao, please elaborate on explaining a bit these three characteristics. One characteristic one point.}%\Luyao{done.}
%that conducts constrained random test generation so that the generated deep learning models satisfy the semantic specifications by construction.




\iffalse
%\toolname{} includes our proposed generation strategy named  \textbf{incremental construction by satisfaction}. \toolname{} incrementally constructs a deep learning model by randomly picking an operation and appending it into the current work-in-progress  model (as the prefix of the final model), in a style similar to the preceding incremental checking approach.
The key idea for \toolname{}'s effectiveness comes from that we model the construction of a valid deep learning model as a \textbf{constraint sampling problem}. %, in contrast to a random generation problem (as done in the preceding incremental checking approach). 
To efficiently sample solutions of constraints, based on our insights of acyclic trait of deep learning models, we conduct \textbf{graph-level constraint reduction} to reduce the problem of constructing the whole model to the problem of constructing a new operation for the work-in-progress model.
However, even with graph-level constraint reduction, the constraints are still hard to handle by existing solver-based approach due to the existence of \textbf{tensor structural constraints} and \textbf{quantifiers} in the constraints such as Equation~\eqref{c4}, \eqref{c5}.
In order to address it, we propose two techniques named \textbf{\tone{}} and \textbf{\ttwo{}} based on our insights of layered constraints strong arc consistency on the constraints of tensors. Generally, \toolname{} constructs the input tensors of the new appended operation in a bottom-up way with the interaction of simplifying the original constraints to quantifier-free constraints on only elementary typed variables. In this way, \toolname{} effectively generates a random deep learning model with ensuring both of the soundness (resulting model's validity) and completeness (no loss for the probability of generating any valid model) for testing deep learning compilers. 
\fi

%\toolname{} is able to randomly sample a solution of the constraint under consideration without any retrying by using our ,
%(see Section~\ref{sec:approach} for details)

%\Luyao{add more details?}

% incrementally constructs and grows prefix parts of an eventually/finally constructed deep learning model so that an earlier constructed prefix part (along the way of construction) is guaranteed to satisfy the semantic specifications by construction.%\toolname{} includes two novel techniques: , which efficiently construct a random part into the existing generated model with ensuring the consistency of new model's validity. 
%In this way, \toolname{} constructs valid deep learning models without backtracking with soundness and completeness.

%In particular, based on our insight on `arc consistency' of node inputs and acyclic trait on the dependency of 

% In particular, we design \toolname{} based on our insight that semantic specifications in a deep learning model exhibit  the acyclic trait on three different levels. 
% The insight behind our work proposed in this paper is that the acyclic trait of semantic specifications in deep learning model provide us with opportunity to carefully design generation strategies for test generation.
%In fact, our insights on the acyclic trait reflects in three different levels. 
%Taking advantage of the  acyclic trait at each of these three levels, 



% For example, if we have three tensors named $A$, $B$, and $C$, and the operation is to calculate multiplication of 2-D tensor $A$ and $B$ and assign the result to tensor $C$: $$ C = MatMul(A, B) $$ If we first generate tensor $A$, we could know the length of the first dimension of tensor $B$ based on the semantic specification of matrix multiplication. Also, we could infer the shape of tensor $C$ if we have generated tensor $A$ and tensor $B$. Here, we name  values of the tensor's dimension and the length of each dimension as the attributes of the tensor. If we take the semantic specification as constraints on the tensor's attributes, we would get a series of constraints based on each operation in the deep learning model. As the case with high probability in purely random test generation, if tensors of the generated deep learning models could not satisfy those constraints, the compiler under test would stop at very early stages such as parsing or static checking that core parts of the compiler have no chance to be tested then the testing could not achieve the goal for detecting critical bugs in deeper compiler logic. How to efficiently generate a random deep learning models whose operations and tensors  satisfy the model's semantic specification? To construct valid deep learning models while taking their semantic specification into account becomes a crucial challenge of random testing for a deep learning compiler.

% To address the challenge of satisfying constraints in the semantic specification of deep learning model, in this paper, we propose a novel approach with following main insights: (1) A deep learning model is a directed acyclic graph\footnote{For structures such as recurrent neural network, we could still take the recurrent neural network as an acyclic graph after unrolling the loop.}, the semantic specification of model is introduced by the arithmetical operations, and it is only related with the attributes (e.g., the dimension size and length of each dimension) of a single operation's input and output tensors, it allows us to incrementally construct deep learning model with global validity; (2) semantic specification of deep learning model could mostly be represented as constraints with primitive mathematic operations that are able to safely propagate with validity; (3) higher order function\Luyao{refine} in the expression of constraints makes difficulties for generation, but the loop-free particularity gives us chance to carefully design the order of variable generation to simplify the situation.

% Based on our insights, we propose our approach to randomly generate valid deep learning models with satisfying semantic specifications by construction. First insight directs us to construct a random deep learning models by incrementally appending model's operations. Second insight provides us opportunity to use safe propagation for specification. Third insight guide us design a well order for the order of variable generation. our approach ensures validity of the constructed deep learning models during the whole generation process without losing the whole space of valid models. In other word, our approach preserve the properties on both soundness and completeness for generation.

To evaluate \toolname{},  we implement it and empirically compare it with \pre{four} \rev{five} baselines: (1) the aforementioned approach of random test generation, named as \bone, (2) test generation based on the idea of feedback-guided test generation~\cite{pacheco2007feedback}, named \btwo, (3)  a  state-of-the-art tool named  Muffin~\cite{DBLP:conf/icse/GuLZ022} implementing a generation-based approach for deep learning models, and (4) \rev{a mutation-based approach,} TVMFuzz~\cite{DBLP:conf/sigsoft/ShenM0TCC21}, \pre{the only existing tool} toward testing deep learning compilers \rev{, (5) a state-of-the-art generation-based approach named NNSmith~\cite{NNSmith} toward testing deep learning compilers}.
Our evaluation results show that our \toolname{} approach substantially outperforms the baselines on the metrics of generated valid test inputs under the same setting, for demonstrating our approach's effectiveness.
%when randomly constructing valid models to test deep learning compilers.
Furthermore, to investigate the bug detection capability, when used to test the same benchmark (TVM, Glow, and SophGo), \toolname{} detects \bugnumber{} unique bugs in total (with 18 on TVM, 4 on Glow, and 11 on SophGo), \pre{outperforming} \rev{performing better or as well than} the baselines.
%Muffin~\cite{}, which detects XX bugs; and TVMFuzz~\cite{DBLP:conf/sigsoft/ShenM0TCC21}, which detects only 5 bugs.
% Note that there is no bug overlapping between the preceding 8 bugs and 5 bugs.
%These results indicate that %even without requiring seed inputs,
%\toolname{} still outperforms TVMFuzz in terms of the number of detected bugs, and both approaches can be used in combination due to their complementary nature of detecting different bugs.
%has been deployed to test three popular real-world deep learning compilers (TVM~\cite{DBLP:conf/osdi/ChenMJZYSCWHCGK18} and ONNX Runtime~\cite{onnxruntime} as two popular open-source deep learning compilers along with a commercial compiler named SophGo).

In addition, among the bugs found by \toolname{}, there are \unknownbug{} previously unknown bugs. After these previously unknown bugs were reported to compiler developers, 19 were confirmed and 16 were already fixed upon our bug reporting so far. 
%Note that most of these detected bugs are found on the released versions of the compilers under test.
%\Luyao{add: \toolname{} also found \extrabugnumber{} bugs in a commercial deep learning compilers from company S and all of them are already fixed.}
The positive feedback from the developers also shows \toolname{}'s high value in practice. The source code, experimental results, and bug reports are publicly available at \url{https://github.com/israProj/isra}.

In summary, this paper makes the following contributions:
\begin{itemize}
%	\item The first to address the problem of testing deep learning compilers, to the best of our knowledge;
    %\item The first approach of testing deep learning compilers without requiring seed inputs.
	\item An effective test generation approach named \toolname{} for testing deep learning compilers, based on instantiation-based constraint solving, working in a backtrack-free way, with the guarantee of soundness and completeness.
	\item A domain-specific constraint solver toward  finding solutions to the constraints specified from the semantic specifications of a deep learning model, with two novel strategies for resolving complex constraints.
	\item Implementation and evaluation of our approach for showing its high effectiveness and high practical value, including
 \pre{outperforming state-of-the-art approaches (Muffin~\cite{DBLP:conf/icse/GuLZ022} and 
 TVMFuzz~\cite{DBLP:conf/sigsoft/ShenM0TCC21})}
 \rev{outperforming state-of-the-art approaches on coverage metrics, achieving comparable and complementary results on the bug detection}, and successfully finding \bugnumber{} unique bugs in three popular real-world deep learning compilers.
\end{itemize}

%The rest of the paper is organized as follows. Section 2 takes a concrete example to demonstrate the overview of our approach. Section 3 shares our observations on modeling semantic specification of deep learning model for test generation. Section 4 describes the technical details that how our approach effectively generate valid deep learning models by constraint propagation. Section 5 shows the evaluation results. The rest parts are threats to validity, discussion and future work, related work and conclusion.


==> arXiv-2302.00842v2/sections/overview.tex <==
\section{Background and Overview}\label{sec:s2}

%\yx{Suggested organization of this section (could use subtitles): 1. overall process (can be omitted if space constraint) 2. Challenge: fulfilling syntactic and semantic constraints with an example (please use a figure to only show the example, without our approach). 3. Why existing approaches fail 4. How our approach works (terms like arc consistency can only appear in this part).}


Figure~\ref{fig:pipeline} shows our overall pipeline of random testing for deep learning compilers. In the stage of test generation, we use our test program generator to generate random computation graphs that are semantically valid. For the test oracle, we use both differential testing and the crash status of the compiler under test~\cite{DBLP:journals/csur/ChenPPXZHZ20}.  
%As for the strategies of differential testing, we use a cross-compiler (i.e., comparing results produced by different compilers) and cross-optimization (i.e., comparing results produced by different optimization levels on the same compiler) .
Before formally describing our approach in detail (as shown in Section ~\ref{sec:approach}), we first take an overview of background with specific examples, then illustrate our approach in a nutshell.
% and finally present our approach in a nutshell with a concrete running example.


%--------------------------------------------------------------

%\subsection{Overall Process}


%Then, we only need to satisfy the semantic specification of our new generated operation such as the length of last dimension of first input tensor is equal to the length of penultimate dimension of second input tensor, and the \emph{model-level} acyclic trait will finally ensures the whole model's validity for the semantic specification.
% In our example, the attributes of a tensor $A$ are the number of its dimensions $a.len$, the length of the first dimension (denoted as $a[1]$), the length of the second dimension (denoted as $a[2]$), etc. In the meanwhile, we model the semantic specifications as constraints between those attributes. 


%Besides the preceding technique, in order to better construct connections between operations in the deep learning model (i.e., output tensor of one operation as the input of another operation), our approach includes another technique called on-demand tensor generation.

%Let us back to previous example of \CodeIn{MatMul} operation as $C = MatMul(A,B)$.

%For all of the various operations in the computation graph, corresponding semantic specifications should be satisfied, otherwise the generated model will be invalid for deep learning compilers. Our goal is to effectively generate random computation graph for testing deep learning compilers.



% For constructing tensors for inputs, we actually has two choices for a single tensor: (1) picking from existing tensors including $x_{out}$ and $y_{out}$, (2) generating a new one. If we directly conduct random generation (which is the way that most of black-box random testing uses), it holds low chance of satisfying the semantic specification.
%\Luyao{next, describe the limitation of existing approach}

% If we do not consider semantic specification in the generation process, as existing approaches do, 

% Back to the example, another situation is that we choose to pick both of inputs from existing tensors (i.e., tensor $x_{out}$, $y_{out}$ as shown in Figure~\ref{fig:p1}), it only holds 25\% probability of satisfying semantic specifications because only picking $x_{out}$ as the first tensor of inputs and $y_{out}$ as the second one is valid and all of other combinations are failed.

%only $\{A: x_{out}, B: y_{out}\}$ ($\{A: X, B: Y\}$ means that picking $X$ as the first tensor of inputs and $Y$ as the second one) is valid, while $\{A: x_{out}, B: x_{out}\}, \{A: y_{out}, B: y_{out}\}, \{A: y_{out}, B: x_{out}\}$ are all invalid. Without guidance from the semantic specifications, existing blackbox random testing approaches  are ineffective due to the low opportunity of generating valid tensor combinations.

% Taking the operations and their input/output tensors as variables, we could model this problem as a \textbf{constraint sampling problem}. However, existing solver-based approach ~\cite{DBLP:conf/tacas/MouraB08, DBLP:conf/iccad/DutraBS18} could not effectively handle this problem due to following reasons: (1) the scale of the constraints increase by the size of computation graph, leading to inefficient performance of sampling; (2) it contains complicate constraints that existing approach can not handle, including structural constraints\Luyao{add definition of structural constraints here}.


\begin{figure}[t]
    % \vspace{-0.2cm} 
    \centering
    % \setlength{\abovecaptionskip}{0cm}   
    % \setlength{\belowdisplayskip}{0pt} 
    \includegraphics[width=\linewidth]{imgs/ICSE23-luyao-flow(1).pdf}
    \caption{The Pipeline of Testing Deep Learning Compilers}
    \label{fig:pipeline}
    \vspace{-0.3cm}
\end{figure}

\subsection{Computational Graph for Deep Learning}\label{sec:s2.1}

A deep learning model, as the input of deep learning compiler, can be regarded as a computation graph, where an edge represents a tensor (an N-D array), denoting the flow of data between nodes, and a node represents (1) an operation (denotes a mathematical function) whose inputs are the incoming edge(s) and outputs are the outcoming edge(s), or (2) a tensor placeholder where we need to represent creation of a user-defined variable such as the input tensor of computational graph.
The computation graph can be executed by feeding the specific data into tensor placeholders. 
The formal definitions of the computation graph are shown in Section~\ref{sec:approach}. 

As an example, Figure~\ref{fig:p2} shows a deep learning model with two operations. The first operation is \CodeIn{Add}. It takes two tensors $p$ and $q$ as its input and outputs a tensor $r$ as their sum. The second operation is \CodeIn{Concat}. It accompanies an attribute $axis$ (denoting the dimension of the axis to concatenate on) and takes two tensors $r$ and $s$ as its input, and outputs a tensor $t$ as their concatenated results. The edge in the computation graph represents the dataflow that gets transferred between the nodes. For example, $r$, as the output of \CodeIn{Add} operation, could be transferred to the input of \CodeIn{Concat} operation.

% Both of input and output of operations is a set of tensors that we will assign the specific tensor value later in the computation of deep learning. A computation flow of data (i.e., an edge) is a tuple consisting of two tensors (written as $(x, y)$). Note, for edge $(x,y)$, $x$ should belong to the output of one operation and $y$ should belong to the input of another operation. In our example, $(Y_{out}, X_{in1})$ is an edge, denoting that during computation of deep learning the data of $Y_{out}$ will pass to tensor $X_{in1}$.


A computation graph is directed and acyclic, specifying the order of computation.
% The edges of the graph denote the data dependencies between two nodes.
In the example, you need to compute \CodeIn{Add} first in order to compute \CodeIn{Concat} because the output of \CodeIn{Add} (i.e., tensor $r$) flows to the input of \CodeIn{Concat}.
Except for the acyclicity of the graph, for each operation, the number of incoming edges should be aligned with the number of input arguments defined by corresponding mathematical function that operation denotes. For example, \CodeIn{Concat} requires two or more input arguments, so the number of incoming edges should be more than or equal to two. We called those semantic specification of computation graphs as \textbf{graph-level constraints}.

Besides graph-level constraints, each operations in the computation graph holds its internal semantic specification, specified from the definition of mathematical function that operation denotes, which we called \textbf{operation-level constraints}.
% Each operation in a computational graph is naturally accompanied by the semantic specification, which specify conditions that valid computations must satisfy.
In our example, as the input of \CodeIn{Add} operation, tensor $p$ and $q$ should have the same shape.
%i.e., $p$'s dimension size should be equal to $q$'s, and also, the length of each dimension of $p$ should also be equal to $q$'s.
Similarly, as for \CodeIn{Concat} operation, tensor $r$ and $s$ must have the same shape, except for the dimension of the axis to concatenate on (defined by an operation's attribute $axis$).
Particularly, by explicitly denoting the structure of tensors, operation-level constraints of the computation graph in Figure~\ref{fig:p2} could be specified as follows ($dim_a$ denotes the dimension size of tensor $a$, and $a[i]$ denotes the length of the i-th dimension of tensor $a$) :
\begin{eqnarray}
& dim_{p} = dim_{q} = dim_{r} \label{e3} \\
& \forall i \in [1, 2, ..., dim_p], p[i] = q[i] = r[i] \label{e4}  \\
& dim_{r} = dim_{s} = dim_{t} \label{e5} \\
& \forall i \in [1, 2, ..., dim_r] \wedge i \neq axis, r[i] = s[i] = t[i] \label{e6} \\
& t[axis] = r[axis] + s[axis] \label{e7}\\
& 1 \leq axis \leq dim_r \label{e8}
\end{eqnarray}

% We denote the semantic specification of an operation with type $t$ as $Spec_t$, which is a constraint on the operation's input, output and other attributes. For example, operation $x$ in Figure~\ref{fig:p1} contains two tensors $x_{in1}$, $x_{in2}$ as its input and a tensor $x_{out}$ as its output. The semantic specification of operation $x$ (denoted as $S_x$) could be represented as $S_x:= Spec_{Op_x}(para_x, x_{in1}, x_{in2}, x_{out})$ (here, $Op_x$ denotes the type of operation $x$, $para_x$ denotes the attributes of operation $x$ such as `strides' in \CodeIn{Conv} operation, it is similar to operation $y$). The semantic specification of each edge $e$ (denoted as $S_e$) is actually a equivalence relation of the structure of two tensors (we denoted $Str_x$ as the structure of a tensor $x$). For example, in Figure~\ref{fig:p1}, edge $(y_{out}, x_{in1})$ is accompanied by the semantic specification that the structure of tensor $y_{out}$ should be equal to tensor $x_{in1}$, i.e., $S_{(y_{out}, x_{in1})}:= Str_{y_{out}} = Str_{x_{in1}}$.

\iffalse
Formally, a valid deep learning model $G$ must satisfy following semantic specification (we use $V(G)$ as $G$'s nodes and $E(G)$ as $G$'s edges):\Ziheng{E(G) maybe too wide?}
%\Luyao{add the constraints that G is acyclic?}
\begin{equation}
\bigwedge_{v \in V(G)} Spec_{v}(E(G)) \label{e1} 
\end{equation}
\fi



\begin{figure}[t]
    \vspace{-0.2cm} 
    \centering
    \setlength{\abovecaptionskip}{0cm}   
    \setlength{\belowdisplayskip}{0pt} 
    \includegraphics[width=\linewidth]{imgs/p2.png}
    \caption{An Example of a Computation Graph.}
    \label{fig:p2}
    \vspace{-0.3cm}
\end{figure}


\subsection{Challenges}\label{sec:s2.2}

%A valid deep learning model corresponds to a solution for the Equation~\ref{e1}. In order to generate valid deep learning models for testing deep learning compilers, we need to effectively sample solutions for this constraint.

The complicated semantic specifications of the computation graph, which consist of both the graph-level constraints and operation-level constraints, result in the sparsity of semantically valid inputs (compared to syntactically valid inputs).
Thus, random test generation suffers the issues on effectiveness. Specifically, the approach that randomly generates possible computation graphs, and then filters invalid ones by checking against the semantic specification, holds fairly low possibility to satisfy the semantic specification.
As our previous example, for two tensors of the input of an \CodeIn{Add} operation, assume that the range of the tensor's dimension size is $O(D)$ and the length of each dimension is $O(L)$, the generation holds $O(L^{-D})$ possibility of producing valid ones due to Equation~\ref{e4}.
The possibility diminishes with larger deep learning model, wider range, or more complex specifications.

%To effectively generate semantically valid inputs, imperative-style test generation aims to generate test input by excluding semantically invalid space during the search process. 

In order to better conduct random testing on deep learning compilers, instead of taking semantic specification as a blackbox checker, we explicitly specify the semantic specifications of computation graph as constraints, i.e., take semantic specification as an whitebox, and test generation is equivalent to find solutions that satisfies those constraints.

However, existing practices of constraint solving are limited due to our complex constraints which are expressed in first-order/second-order logic instead of propositional logic due to following reasons: (1) the acyclicity of computation graph;
% According to the standard of deep learning operations such as ~\cite{onnx_standard},
% first, graph-level constraints (i.e., acyclicity of computation graph), are difficult to directly encode and solve as logic formulation such as satisfiability modulo theory (SMT);
% second, operation-level constraints, i.e., the constraints specified by each operation's specification, are expressed in first-order/second-order logic instead of propositional logic due to two special forms in the constraints:
(2) the existence of quantifiers such as $\forall i \in [1, 2, ..., dim_p]$ in Equation~\ref{e4}; (3) the existence of unknown functions such as $r[axis]$ in Equation~\ref{e7} (it is called unknown function because we actually need to construct a function that maps to the length of each dimension of a tensor that we may not know the dimension size).
Compared with propositional logic that is decidable, solving first-order/second-order logic (with quantifiers and unknown functions) is challenging because theoretically the first-order/second-order logic is undecidable in general~\cite{turing1936computable} and also, in practice, quantifiers and unknown functions cause existing solvers unable to encode, or perform inefficiently ~\cite{gradel2007finite, DBLP:conf/cade/ReynoldsTGKDB13, DBLP:conf/iccad/DutraBS18}.



%In our problem, this way holds fairly low possibility to satisfy the semantic specification. Even if we could produce solutions in this way, the solutions tend to be simple and biased because the operations with more complex specifications hold lower possibility to be produced compared to the operations with simpler specifications, as the evaluation result shown in Section~\ref{sec:evaluation}.
% For example, if the graph contains $K$ \CodeIn{MatMul} operation(s) in total, then the possibility of producing valid models by pure random sampling will be less than $O(L^{-K})$.


%Our key challenge of sampling lies in the existence of quantifiers and unknown functions with undetermined domains.
%Specifically, in our example, quantifiers $v$ and $e$ in Equation~\ref{e1} and quantifier $i$ in Equation~\ref{c5}. Also, the term $B[dim_B-1]$ in Equation~\ref{c4} represents the length of last second dimension of tensor $B$, it actually contains a function that is to get the length of i-th dimension of a tensor, where i is undetermined.


%For the first part, quantifier exists in the constraints such as Equation~\ref{c5}. In Equation~\ref{c5}, the existence of some relations is determined by the value of $dim_A$. For example, the relation $A[1]=B[1]$ exists only when $dim_A \geq 3$.

%This kind of constraints is not supported or directly modeled by existing approach~\cite{DBLP:conf/tacas/MouraB08, DBLP:conf/iccad/DutraBS18}.
%Also, the existing quantifier elimination technique~\cite{gradel2007finite} to simplify the formulas does not work due to the unknown domain of the quantifier. %Thus, the quantifier leads to our second challenge.

%For the second part, the tensor structural constraints exists in the constraints such as Equation~\ref{c4}.

\iffalse
Equation~\ref{c4} describes a relation between two tensors $A$ and $B$: the length of last dimension of $A$ is equal to the length of second last dimension of $B$. 
The Equation~\ref{c4} is equivalent to the following form on those variables: $$C_4': \bigvee_{\forall i \in \mathbb{N}^+, \forall j \in \mathbb{N}^+} (dim_A=i \wedge dim_A=j \wedge A[i]=B[j-1])$$
This form of constraints considerably increases the scale of constraints, causing the existing solver-based approaches inefficient.
\fi

% As the size of the model increases, the scale of model's constraints will be fairly large, causing the inefficient performance of sampling solutions of model's constraints. 

\iffalse

For both of the quantifiers and unknown functions, if we already determine the value of $dim_a$ and $dim_b$ as $\overline{dim_a}$ and $\overline{dim_b}$.
Equation~\ref{c4} (represented as constraints on variables of $a[i]$ and $b[i]$) could be simplified as $A[\overline{dim_A}] = b[\overline{dim_b}-1]$.
Equation~\ref{c5} could be simplified as $A[1]=b[1], A[2]=b[2], ..., A[\overline{dim_A}-2] = b[\overline{dim_b}-2]$.
It inspires us to design efficient strategies to address this challenge.

\fi

\subsection{Instantiation-based Constraint Solving} \label{sec:instantiation}
Instantiation ~\cite{apt2003principles, kumar1992algorithms, prosser1993hybrid, reynolds2014finding, reynolds2013quantifier} is a widely used technique for solving constraint satisfaction problem (CSP) such as satisfiability modulo theories (SMT).
%As the main idea for addressing the challenge of constrained sampling, instantiation is our key idea to eliminate the quantifiers and unknown functions in the constraints.
By assigning the values to the variables in the constraints, we could get an instantiation of the constraints.
% For example, for the constraint $S \subset T$, $\{T:\{1, 2\}\}$ ($\{x: v\}$ denotes that we assign a specific value $v$ to variable $x$) is an instantiation.

An instantiation-based solver starts from an empty instantiation and extends instantiation (mostly in an iterative way) to find solutions. 
An instantiation could be extended by assigning the values to the variables that are not assigned in the instantiation before.
In the meanwhile, by replacing the variables with their assigned specific values in the constraints, also, with the help of solver, it is possible to simplify constraints and reduce the domain of unassigned variables (it is called as constraint propagation~\cite{apt2003principles}). 
For example, for the constraint $S \subset T$ ($S$ and $T$ are set variables), if we first instantiate $T$ as $\{1,2\}$, then it is easy to simplify the constraints by solving constraints and simultaneously deducing the domain of $S$, i.e., $S \subset T \Rightarrow S \subset \{1,2\} \Rightarrow S \in \{\emptyset,\{1\},\{2\}\}$.

With instantiation, the elimination technique has a chance to be applied for the simplification on constraints which are originally encoded in first-order logic (or higher-order logic). Inspired by quantifier elimination~\cite{DBLP:conf/cade/MouraB07, gradel2007finite}, if we already determine the domains of quantifiers or unknown functions in constraints according to the instantiation, we could then simplify the constraint by rewriting the constraints to an quantifier-free and unknown-function-free form. 
For example, assume $S$ is a set variable, for the constraint $\forall x \in S, P(x)$, if we already instantiate the domain of the universal quantifier $x$ as $S: \{1,2,3\}$, then we could eliminate the quantifier by rewriting the constraints as follows: $\forall x \in S, P(x) \Longrightarrow P(1) \wedge P(2) \wedge P(3)$. 
% To satisfy the condition of elimination, i.e., the domain of quantifiers and unknown functions is determined, we could first instantiate the variables in the domain of quantifiers and unknown functions to simplify the constraints.


We call an instantiation consistent if it could be extended to a solution, otherwise it is inconsistent. For example, in the constraint $S \subset T$, if we first instantiate $T$ as $\emptyset$, then the instantiation is inconsistent.
% It is critical to determine if an instantiation is consistent for instantiation-based approaches.
%Generally, to ensure the consistency, instantiation-based solver will backtrack if assigned values of variables do not satisfy the constraints, hurting the overall performance of finding solutions.
Generally, instantiation-based solvers may backtrack to try other instantiations if it finds instantiations are inconsistent. Backtracking decreases the solver's efficiency on finding solutions.
%To improve that, existing practices apply heuristic rules to reduce the search space, however, usually without completeness guarantees ~\cite{}\Luyao{todo} (completeness means that any valid solution is able to be generated).
%For test generation, besides the soundness (generated inputs are valid), both efficiency and completeness are also critical, so a domain-specific solver with good instantiation strategies is necessarily required for improving overall testing effectiveness.


\subsection{\toolname{} in a Nutshell}\label{sec:nutshell}

%Taking our problem, i.e., sampling solutions of the constraints, as a constraint satisfaction problem (CSP),

To effectively generate semantically valid computation graphs, we propose an effective random test generation approach, named \toolname{}, including a domain-specific constraint solver with two strategies: \toneandtwo{}, based on our key idea that constraints are able to be simplified with a well-designed instantiation order. Next, we introduce a running example to briefly illustrate how \toolname{} works.


%In \tone{}, with the help of the topological ordering of the computation graph, \toolname{} resolves the constraints on the whole graph into constraints related to only a subpart of the graph (actually, a single operation with the incoming edges).

%In \ttwo{}, due to the strong n-consistency, .... \Luyao{todo}


% This section will cover instantiation and elimination, that are the key steps of \toolname{}. 



\begin{figure*}[htp]
    \centering
    \setlength{\abovecaptionskip}{0.2cm}   
    \setlength{\belowdisplayskip}{0pt} 
    \includegraphics[width=\linewidth]{imgs/p3.png}
    \vspace{-0.3cm} 
    \caption{A running example of \toolname{}}
    \label{fig:p3}
\end{figure*}


% \toolname{} is an instantiation-based approach that samples solutions of constraints without backtracking. The instantiation contains two stages: \tone{} and \ttwo{}, as we describe as follows.\Ziheng{Should we propose the subtitles 3,4 at the start of part C?} 

\subsubsection{Graph-level constraint resolving}

% In Equation~\ref{e1}, we define the semantic specification of a valid deep learning model. To eliminate the universe quantifiers $\forall v \in V(G)$ in Equation~\ref{e1}, we incrementally instantiate the operations in the computation graph in a top-down way.
Our generation follows a topological order of operations in computation graph. We say node a precedes node b, or b succeeds a, if there exists a path, where a appears earlier than b in the path. Each time we generate a node, this node does not precedes any existing node. 
%Due to the acyclic trait of the directed computation graph, we could find a topological order of operations.
For example, as the graph shown in Figure~\ref{fig:p2}, followed by a topological order, i.e., operation $Add$ then operation $Concat$, our approach instantiates operations one by one. For each operations, we first instantiate its type and the number of incoming edges.

%For the next operation we instantiate, we also instantiate the edge during our instantiation of operations.
%In other words, for each operation, we will consider the instantiation of all of edges that points to current operation (i.e., the second tensor of the edges belongs to the input of current operation). In our example, we would instantiate as following order: operation $Add$, operation $Concat$ ( during the instantiation of $Concat$, we would consider the existence of edge $(y_{out}, x_{in1})$).
%In this way, \tone{} eliminates the quantifiers in Equation~\ref{e1} by partitioning the generation into several subparts (each part corresponds to a single operation and its related edges):
In this way, our approach resolves the constraints by partitioning them into several subparts. Each subpart corresponds to a single operation and its related edges. Furthermore, because the output of operations could be determined only by the input and attributes, we rewrite the constraints by substituting the output as a function of the input and attributes. In our example, the constraints are as follows, where $Spec_{op}(V)$ is defined as a set of constraints on $V$ that specifies from the specification of an operation with type $op$, $f_{op}$ denotes the mathematical function of the operation with type $op$:
%In our example, it is as follows:
% $$Spec_{Add}(p,q,r) \wedge Spec_{Concat}(axis, r,s,t) $$
\iffalse
\begin{equation}
\label{ex}
\begin{split}
Spec_{Add}(p,q) \wedge Spec_{Concat}(axis,r,s)
\end{split}
\end{equation}
\fi

\begin{eqnarray}
& S_1: Spec_{Add}(p,q) \wedge (r = f_{Add}(p,q)) \label{eqs1} \\
& S_2: Spec_{Concat}(axis,r,s) \wedge (t = f_{Concat}(axis, r, s)) \label{eqs2}
\end{eqnarray}

%$$ Spec_{Add}(p,q,r) \wedge Spec_{Concat}(axis, r,s,t) \Leftrightarrow Spec_{Add}(p,q) \wedge (r = Add(p,q)) \wedge Spec_{Concat}(axis,r,s) \wedge (t = Concat(axis, r, s)) $$.

After resolving constraints with instantiating operations in the graph by their topological order, our goal turns to instantiate each single operation by solving constraints related to the operation (in our example, they are $Spec_{Add}(p,q)$ and $Spec_{Concat}(axis,r,s)$), as shown in the next part.
%after then the output could also be instantiated.
%, $$Spec_{op}(a, b, c) \Leftrightarrow S(a, b) \wedge (c = f(a,b))$$ (here, $f$ is a function depends on the operation's type), so our approach then only instantiate the attributes and input, and finally produces the structural information for output.
%To further simplify and resolve them, we conduct \ttwo{} as shown in next part.

\subsubsection{Operation-level constraint resolving}
The instantiation of a new operation includes assigning the value to its operation type, attributes, input (incoming edge(s)) (output of the operation is excluded as explained before).
As a concrete example, assume we already instantiate a computation graph with a single \CodeIn{Add} operation (with $p$ and $q$ as its input as shown in the red part of Figure~\ref{fig:p3}), now we extend the instantiation by appending a new operation into the computation graph.

%For example, the red part of Figure~\ref{fig:p1} shows a single operation with type as $MatMul$ and its two tensors as its input marked as $a$ and $b$ (to simplify, we ignore the output here). 

%Our approach first randomly decides the type of operation.
Assume we instantiate type of the new operation as \CodeIn{Concat}, and the number of incoming edges of the new operation as two in our example.
%Our approach then sets a special attribute of the operation named $indegree$ as the number of incoming edges of the operation, which depends on the operation type. Here we set it as two.
We now set symbol variables for the input and attributes of the operation.
In the example of \CodeIn{Concat}, we denote variable $ax$ for the attribute $axis$, and variable $x$ and $y$ as two incoming edges (note, $ax$, $x$ and $y$ are just symbol variables, which will be assigned with values later, such as assigning $r$ to $x$).

For each incoming edge, i.e., each tensor in the input, instead of instantiating the whole tensor, we focus on instantiating the structure of the tensor first due to that the semantic specifications are only related to tensor structure. For an edge $x$, we setup a set of symbol variables to substitute $x$ in the constraints, including $d_x$ (denoting the dimension size of $x$, i.e., $dim_x$) and $x_i$ (denoting each dimension's length of $x$, i.e., $x[i]$). In this way, the constraints could be further specified as follows: 
% $$Spec_{Concat}(axis, x, y) \Leftrightarrow Spec_{Concat}(axis, Str_x, Str_y)$$.
%Inspired by the theory of constraint programming~\cite{apt2003principles}, our approach
%By taking the operation's attributes and structure information of the tensors in the input as symbol variables, in our example, the constraints could be further specified as follows:
\begin{eqnarray}
& \bigwedge_{k \in \{1, 2, 3\}} C_k(ax, d_x, d_y, x_i, y_i)\\
& C_1: d_{x} = d_{y} \label{c1} \\
& C_2: \forall i \in [1, 2, ..., d_x] \wedge (i \neq ax), x_i = y_i \label{c2} \\
& C_3: 1 \leq ax \leq d_x \label{c3}
\end{eqnarray}



\iffalse
In our example, the semantic specification could be taken as following constraints\footnote{\Luyao{refine}\url{https://docs.scipy.org/doc/numpy-1.13.0/reference/generated/numpy.matmul.html}}:

$$ S(a, b) \Leftrightarrow \bigwedge_{k} C_k(d_a, d_b, a_i, b_i)$$
\begin{IEEEeqnarray}{CC}
\IEEEyesnumber \IEEEyessubnumber*
%&\forall MatMul(A, B) \in G,\\
&C_1: d_a \geq 2 \label{c1}\\
&C_2: d_b \geq 2 \label{c2}\\
&C_3: d_a = d_b       \label{c3}\\
&C_4: a_{d_a} = b_{d_b - 1}   \label{c4}\\
&C_5: \forall i \in [1, 2, ..., d_a-2], a_i = b_i \label{c5}
\end{IEEEeqnarray}
\fi

%A solution of those constraints (a specific value assignment on those symbol variables) 


% Equation~\ref{c1}-~\ref{c5} containing following preliminary-typed variables: $dim_a$, $dim_b$, $a_i$, $b_i$ ($a_i$ denotes the variable for the value of function $a[i]$, same as $b_i$).

%The strategy our approach conducts in following instantiation is named joint instantiation. 

To sample a random solution to the above constraints, our approach instantiates variables in a well-designed order:
%To satisfy the condition of elimination, we define a well order to instantiate variables:
first are variables related to $x$; then attribute $axis$; finally variables related to $y$. In our example, the order is as follows: $d_x$; $x_i$; $axis$; $d_y$; $y_i$.
Note, in the order, variables related to the same tensor are ordered together in a group, also, within the group, instantiation of the dimension size (e.g., $d_x$) is ahead of the length of each dimension (e.g., $x_i$). The detailed illustration and explanation of the order are shown in Section~\ref{sec:s3.3}.

Followed by this order, we are able to simplify the constraints to quantifier-free and unknown-function-free by the elimination technique mentioned in Section~\ref{sec:instantiation}; also controllably choose ways for instantiating unassigned tensors, i.e., instantiating the tensor as an instantiated one such as $r$ for $x$; or as the output from a tensor placeholder such as $s$ for $y$. Details are shown in Section~\ref{sec:approach}.

With above simplification, the constraints belong to propagation logic which is decidable. Thus, we are able to conduct constraint solving by constraint propagation~\cite{apt2003principles} to find solutions. In addition, the constraint propagation will not produce an empty domain (which causes the instantiation inconsistent) due to the good property as explained in next part, resulting in the overall process being backtrack-free. 


\subsubsection{Properties of \toolname{}}\label{sec:properties}
Based on the graph theory and the theory of constraint satisfaction problem (CSP)~\cite{apt2003principles}, our instantiation-based solver holds some good properties due to characteristics of constraints on deep learning models. We draw main conclusions here, formal definitions and detailed explanations are shown in Section~\ref{sec:approach}.

The first property is called \firstp{}. For any semantically valid computation graph with a topological order on operations as  $(O_1, O_2, ..., O_i)$, we can consistently extend the instantiation to include $O_{i+1}$ (with topological order as $(O_1, O_2, ..., O_i, O_{i+1})$) as long as ensuring satisfaction of constraints related to $O_{i+1}$.

The second property is called operation-level global consistency. For constraints related to each single operation, after determining operation's type and the number of tensors in the input, by taking attributes as a variable and each tensor in the input of the operation as a variable, this CSP, which consists of constraints on the operation level, is globally consistent: any consistent instantiation of a subset of the variables can be extended to a consistent instantiation of all of the variables without backtracking~\cite{dechter1992local}.


%To instantiate the variables in the order, 

% Note, we also need to consider the edge in the meantime. For example, $a$ could be passed from previous operations' output. So for the variables belong to the same tensor (such as $dim_a$ and $a_i$), we use an `on-demand' strategy for the instantiation of the edges (we will discuss in detail in our example).


%In our example, we skip the instantiation of attributes because \CodeIn{MatMul} does not have them. Then, it turns to tensor place holder $a$. Within $a$, we first instantiate $dim_a$. Assume 

% Assume we first instantiate $a$ then $b$ (another case is similar). To instantiate $a$, we sample solutions of $P_a(a)$ (i.e. the constraints related only to $dim_a$). Here $P_a(a)$ only contains Equation~\ref{c1} (i.e. $dim_a \geq 2$).

%With consideration of instantiating the edges, we have two choices for $a$: (1) reusing the structure of an existing tensor from the output tensor(s) of previous operations (i.e., $x_{out}$ and $y_{out}$), (2) generating a new tensor. The first choice actually corresponds to the instantiation of an edge in the generated computation graph. With a strategy named controlled edge construction, we could define the distribution of these two choices. In this way, we could control the `density' of edges in the graph (measured by a metric named NOP in our evaluation). We call it `on-demand' strategy for the instantiation of the edges. More details of this strategy are discussed in Section~\ref{sec:approach}.




% reducing the original constraints (that are related to the whole graph) to a more finer granularity (that are only related to single operations and its related edges). Specifically, instead of generating the whole model all at once, our generation will start with an empty model and incrementally construct a valid deep learning model following the topological order. It works as follows: given a valid model as a prefix model (e.g., orange part in Figure~\ref{fig:p1}), we generate a random operation and append it into the prefix model. For the new operation to append, we need to generate its type, attributes, input/output tensor(s), also, all of the edges that point to the new operation. In our example, we will first construct operation $Y$; then construct operation $X$ and also the edge ($y_{out}$, $x_{in1}$).

%Our second stage is operation-level instantiation. It could efficiently generate a random operation to append. In our example, assume new we already have a valid model with two operations: operation $X$ and operation $Y$ as the orange part in Figure~\ref{fig:p1}. We then generate a new operation as the red part in Figure~\ref{fig:p1}. 


% Inspired by the idea of instantiation for quantifier elimination~\cite{DBLP:conf/cade/MouraB07}, we propose a novel instantiation-based technique for effectively sampling solutions for the constraints from the deep learning model's semantic specification. With good properties of deep learning's semantic specification (that we will shown in Section~\ref{sec:properties}), our approach is sound (always produce valid models), complete (does not miss any chance of generating arbitrary valid deep learning models), and backtracking-free (and thus terminating).


% allows us to design an efficient approach for quantifier elimination. Followed a well order of instantiation to conduct quantifier elimination, with the propagation-based constraint satisfaction, the properties of constraints in deep learning models ensure the satisfaction of constraint all the time.










\iffalse
\subsection{A Running Example}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/p2.pdf}
    \caption{The Workflow of \toolname{} on the Example (it shows possible generated models) .}
    \label{fig:p2}
\end{figure*}

Our approach mainly contains two stages for efficiently sampling solutions of the constraints: (1) first stage dismantles the sampling of the constraints of a valid deep learning model into several separated subproblems by a technique called \tone{}; (2) second stage further dismantle the sampling process by a technique called operation-level instantiation.

The orange part in Figure~\ref{fig:p1} shows a deep learning model, with the form of a computation graph containing two operations $X$ and $Y$. The computation graph is a directed acycle graph, so we could find a topological order of the graph. For example, the model in orange part has a topological order: operation $Y$, operation $X$.

Our first stage is \tone{}, reducing the original constraints (that are related to the whole graph) to a more finer granularity (that are only related to single operations and its related edges). Specifically, instead of generating the whole model all at once, our generation will start with an empty model and incrementally construct a valid deep learning model following the topological order. It works as follows: given a valid model as a prefix model (e.g., orange part in Figure~\ref{fig:p1}), we generate a random operation and append it into the prefix model. For the new operation to append, we need to generate its type, attributes, input/output tensor(s), also, all of the edges that point to the new operation. In our example, we will first construct operation $Y$; then construct operation $X$ and also the edge ($y_{out}$, $x_{in1}$).

Our second stage is operation-level instantiation. It could efficiently generate a random operation to append. In our example, assume new we already have a valid model with two operations: operation $X$ and operation $Y$ as the orange part in Figure~\ref{fig:p1}. We then generate a new operation as the red part in Figure~\ref{fig:p1}. Our approach will first randomly choose the operation's type, assume we pick \CodeIn{MatMul} operation.

by randomly choosing its type and constructing a valid assignment for it. The assignment includes the attributes and input/output of the operation, and the edge(s) between this operation and existing operation(s).

Followed a well-designed order to sample and simplify the constraints, we first generate attributes of the operation such as `strides` in \CodeIn{Conv} operation. \CodeIn{MatMul} operation does not contain attributes so we skip this step, otherwise, our approach randomly construct the attributes of the operation. We then directly starts to construct the input (i.e., tensors $a$ and $b$) one by one. Assume we first construct $A$ then $b$ (another case is similar). To construct $A$, we need to generate a tensor satisfying $P_A(A)$ (i.e. the constraints related only to tensor $A$). Here $P_A(A)$ only contains Equation~\ref{c1} (i.e. $dim_A \geq 2$). We have two choices for $A$: (1) reusing an existing tensor from the output tensor(s) of previous operations (i.e., $x_{out}$ and $y_{out}$), (2) generating a new tensor. We illustrate both of the results of these two choices in the left of Figure~\ref{fig:p2}. After determining tensor $A$, we plug it into the constraints, then the left constraints are only related to $b$. As a specific example, assume we already construct $A$ as a tensor with shape of $3 * 5$. By plugging the value of $A$ into the constraints $P(A, b)$, then constraints becomes to $P'(b)$ (i.e. $P(A, b)[A:\overline{A}]$), which is the same as Equation~\ref{c6}-\ref{c10}. 



%\subsection{Our approach}
%To address the challenge, we propose our approach named ~\toolname{}. To generate a random valid deep learning model, ~\toolname{} conduct layered instantiations with two stages: \tone{} and operation-level instantiation. We will describe these two stages as follows.


\subsubsection{Properties}
The first characteristic is based on the acyclic trait of the deep learning model. 
A well-designed generation order of the operations holds the directional path consistency of the constraints, allowing us to eliminate quantifiers in the form of $\forall v \in V(G) ...$ ($V(G)$ denotes all of the operations in the model $G$) in a sound and complete way. The second characteristic is related to constraints within an operation. Tensor-level strong n-consistency allows us to generate tensors one-by-one in an arbitrary order, reducing the problem of constructing several tensors at once to problems of constructing only one tensor, in a sound and complete way. The third characteristic is about the dependencies of variables of a single operation. A well-designed order of sampling variables could eliminate quantifiers and unknown functions within operations. For example, eliminating the quantifier $i$ in the form of $\forall i \in f(dim_A) ...$. 
Based on our insights, we proposed a novel technique named layered instantiation with two main stages: (1) \tone{} first disassembles the whole sampling problem (for sampling a whole graph) into separated subproblems (for sampling an operation) with a bottom-up way;
%\tao{Luyao, please add one or two sentences to elaborate a bit the first technique.}
(2) operation-level instantiation further disassembles the sampling problem of an single operation to the several subproblems (for sampling an single tensor) with an iterative way.
With layered instantiation processes, \toolname{} simplifies the original constraints to quantifier-free formulas without unknown functions, easing the overall sampling process.
%Besides the disassembled characteristics of the constraints, the constraints hold graph-level directional path consistency in the first process, and the constraints hold tensor-level strong n-consistency in the second process. These consistencies of constraints ensure the overall sampling process without backtracking.

\iffalse

\subsubsection{\tone{}}
% If we follow existing approach, e.g., whole checking \yx{what is this?}\Luyao{named in Line 153}(first randomly generating the whole model and then checking against the semantic specifications), the generation would be fairly ineffective because the constraints in the specifications are hard to satisfy. For example, for the generation of a single \CodeIn{MatMul} operation, pure random generation on the two matrices holds only less than $O(L^{-1})$ possibility (assume that the range of tensor's dimension size is $O(L)$) of producing valid matrices due to Equation~\ref{c3}. %\yx{You may integrate the previous paragraph to explain the example, or if it is too complex, leave it to the second section.}
%The possibility diminishes with larger graph, wider range or more complex specifications. For example, if the graph contains $K$ \CodeIn{MatMul} operation(s) in total, then the possibility of producing valid models by whole checking will be less than $O(L^{-K})$.

Our strategy samples a valid model by constructing the model in a bottom-up way. Specifically, instead of constructing the whole model all at once, our construction will start with an empty model and incrementally construct a valid deep learning model following the topological order. It works as follows: given a valid model as a prefix model (e.g., orange part in Figure~\ref{fig:p1}), we generate a random operation and append it into the prefix model.

% Here, we only allow the input tensor(s) to be newly generated (as a user-input tensor or constant tensor) or be the existing tensors (e.g., rectangles with black box in Figure~\ref{fig:p1}) if their structures are matched. We do not allow the output of the new operation to be the input of operations in the prefix model, otherwise, the generated model will contain a loop. 

This bottom-up way successfully disassembles the constraints from the whole deep learning model (including all of its operations and edges) into separated parts (each part corresponds to construct a single operation with its related edges), reducing the problem of sampling of the whole graph to the multi problems of sampling single operations. Due to the directional path consistency, we could ensure the validity of the whole model if each subproblem (i.e. sampling single operations) satisfies their specifications.


As an example shown in Figure~\ref{fig:p1}, we incrementally construct the deep learning model with appending a new random operation. 
Assume we already have a valid work-in-progress model with two operations: Operation $X$ and Operation $Y$ as the orange part in Figure~\ref{fig:p1}. We then construct a new operation as the red part in Figure~\ref{fig:p1}, by randomly choosing its type and constructing a valid assignment for it. The assignment includes the attributes and input/output of the operation, and the edge(s) between this operation and existing operation(s).
\fi

%and a prefix of the topological order could be $Operation Y$. It corresponds to an induced subgraph with only $Operation Y$ as its operation, which is also valid.
%With the properties of computation graph, the validity of each operation (local consistency) will lead to guarantee of the whole computation graph's validity (global consistency).

%\yx{read this again. Assuming you know nothing of your approach. Will you be able to understand it?}



%With above properties of computation graph, if we ensure the validity of newly appended operation $MatMul$, then it will lead to the guarantee of the validity of the whole model (the graph with $Operation Y$, $Operation X$ and $MatMul$).




\subsubsection{Operation-Level Instantiation}

%To construct an operation, the challenge (the existence of quantifiers and unknown) causes the existing approaches of constraint sampling to be inefficient or unable to handle with the constraints of operations.

%To construct an operation, we could directly conduct random generation for constructing attributes and input tensors of the target operation. But this way suffers from ineffective problems because we will re-generate when the generated operation violate its semantic specification. For example, for the generation of the \CodeIn{MatMul} operation, pure random generation on the two matrices holds only less than $O(L^{-1})$ possibility (assume that the range of tensor's dimension size is $O(L)$) of producing valid matrices due to Equation~\ref{c3}.

%We denote the variables of an operation as the operation's type, attributes, input/output tensor(s), and the edges that point to the operation. Instead of generating all of variables of the current new operation together at once, we proposed an iterative way to construct those variables based on our two insights of the constraints. We illustrate them as follows.

\textbf{Layered form of variables within operations} means 
%Let us take all of the terms in the constraints (including operation's attributes and attributes of tensors) as variables. 
%Unlike traditional constraints, which can be expressed in the first-order logic without quantifier, there contains two special forms: (1) quantifier and (2) structural constraints.
we could categorize all of variables in several layers to simply the constraints. More specifically, after determining the values of the variables at previous layers, we could simplify the constraints that related to variables in the current layer into qualifier-free and unknown-function-free constraints on only elementary typed variables. The simplification is inspired by quantifier elimination technique~\cite{gradel2007finite}. We could simplify the original complicated constraints to quantifier-free and unknown-function-free forms if we already determine the domain of quantifiers and unknown functions. For example, we could simplify the terms in unknown functions such as $A[dim_A]$ if the dimension size of $A$ (i.e. $dim_A$) is known.
By following the layered order to generate variables, we could conduct quantifier elimination technique to simplify the constraints.

For example, we layer the variables of the \CodeIn{MatMul} operation as follows: first layer contains attributes in \CodeIn{MatMul} operation (it is actually empty in our example); second layer contains $dim_A, dim_B$; third layer contains $A[i], B[i], i \in \mathbb{N}^+$. After determining the value of $dim_A$ as $\overline{t}$, quantifier elimination could be conducted 
to simplify the Equation~\ref{c5} to several constraints without quantifiers: $ C_5[dim_A=\overline{t}] \Longrightarrow {C_5}_1: A[1]=B[1], {C_5}_2: A[2]=B[2],...,{C_5}_{\overline{t}-2}: A[\overline{t}-2]=B[\overline{t}-2] $, and simplify the Equation~\ref{c4} to $C_4[dim_A=\overline{t}]: A[\overline{t}] = B[dim_B - 1]$.

\textbf{Tensor-level strong n-consistency~\cite{apt2003principles}} implies a well property of the constraints among tensors.
% aiming to first construct one of input tensor(s) to satisfy only its local constraints, and then construct another tensor to satisfy the remaining constraints
For example, \CodeIn{MatMul} operation contains the semantic specification as Equation~\ref{c1}-\ref{c5}. We denote the constraints only related to tensor $A$ as $P_A(A)$, i.e, Equation~\ref{c1}, which is the same as Equation~\ref{c2} for $B$, and the rest of constraints related to both tensor $A$ and tensor $B$ as $P_{AB}(A, B)$. The constraints of \CodeIn{MatMul} operation hold n-strong consistency~\cite{apt2003principles} among tensors: for any tensor $A$ satisfying $P_A(A)$ there always exists a tensor $B$ that $P_B(B)$ and $P_{AB}(A, B)$ both holds, and vice versa (strong n-consistency here is arc consistency because it only contains 2 tensors. The general definition of strong n-consistency is shown in Section ~\ref{sec:approach}).
%Formally, $\forall A, \ P_{A}(A) \rightarrow	\exists B,\ P_{B}(B) \bigwedge P_{AB}(A, B)$,
%and also, $\forall B, \ P_{B}(B) \rightarrow	\exists A,\ P_{A}(A) \bigwedge P_{AB}(A, B)$.
%In our example, $\forall A, dim_A \geq 2 \rightarrow \exists B,\ dim_B \geq 2 \bigwedge (dim_A=dim_B \wedge A[dim_A]=B[dim_B-1] \wedge (\forall i \in [1, 2, ..., dim_A-2], A[i] = B[i])) $.
 
With this property, we could reduce the problem of constructing several tensors to problems of constructing only one tensor without sacrificing soundness and completeness. Our approach will generate the input tensors one by one (in arbitrary order). In our example, we could generate a tensor $A$ as long as it satisfies $P_A(A): dim_A \geq 2$, then plug the value of $A$ into the constraints and the property of consistency ensures that it exists a tensor $B$ that meets all of constraints. As a specific example, assume we already generate $A$ as a tensor with shape of $3 * 5$, by plugging the value of $A$ (denoted as $\overline{A}$ here) into the constraints, then constraints reduce to $P'(B)$, i.e. $P(A, B)[A:\overline{A}]$ (we denote $P[X:\overline{X}]$ as substituting $X$ with $\overline{X}$ in the constraints), as follows:
\begin{align} 
&C_1'(C_1[A]): true \label{c6}\\
&C_2'(C_2[A]): dim_B \geq 2 \label{c7}\\
&C_3'(C_3[A]): 2 = dim_B       \label{c8}\\
&C_4'(C_4[A]): 5 = B[dim_B - 1]   \label{c9}\\
&C_5'(C_5[A]): true \label{c10}
\end{align}

% \Luyao{todo: add the reason of strong arc consistency}

%More specifically, after determining the values of the variables at previous layers, we could simplify the constraints that related to variables in the current layer into a qualifier-free constraint on only elementary typed variables. With our analysis of deep learning's operations, we layer the variables as follows: first layer is the attributes of operations (such as `strides` in \CodeIn{Conv} operation); second layer is the dimension size of tensors; third layer is the length of each dimension of tensors; last layer is the specific assignments for tensors.


%With these two insights, we design an iterative way of tensor construction. Our approach will first generate the attributes of operations then . With the \cons{} among tensors, . With layered forms of variables, we could generate the variables of the tensors in a well order with only solving for qualifier-free constraint on only elementary typed variables. Actually a simple propagation-based solving approach is able to efficiently solve/sample the solution(s) of transformed constraints without backtracking.


%To address the challenge of complicated constraints (existence of structural constraints and qualifiers), we design two strategies to efficiently sample solution of those complicated constraints. Our strategies are mainly based on our insights on the constraints of operations: (1) layered constraint forms; (2) strong arc consistency among tensors in constraints.


%First strategy named layered constraint simplification is based on our insights on layered constraint forms. Second strategy named 

% with iterative simplification .

%After simplification on constraints, we could easily generate a random operation (with valid attributes and input tensors).

% Though the property ensures the existence, problem still leaves for designing an effective and also complete approach for generating a random solution. 

%(1) reduce the process of operation construction, (2) transform the complicated constraints into simplify 

%The operation contains the semantic specification for its input tensors. We omit output tensors here because they are determined by input tensors

% Inspired by quantifier elimination, we design our strategy named layered constraint simplification to simplify the complicated constraints of tensors to quantifier-free constraints of elementary typed variables.

% During operation construction, all of items in the constraints 

%there are two types of special dependencies here. First, the existences of some variables depend on some other variables. For example, the variable $a[2]$ (i.e., the length of tensor $A$'s second dimension) exists only when $dim(A) \geq 2$. Second, the constraints may use universal quantifiers whose range is determined by other variables, and thus the existence of some constraints is dependent on some other variable. For example, given a constraint: $\forall 1 \leq i \leq dim(A) - 2, a[i] = b[i]$, there exists an equality constraint between $a[1]$ and $b[1]$ only when $dim(A)$ is larger than 2.

%Those constraints cannot be directly modeled as standard SMT-lib ~\cite{barrett2010smt}.
%Solvers like Z3~\cite{DBLP:conf/tacas/MouraB08}, SMTSampler~\cite{DBLP:conf/iccad/DutraBS18} are not directly applicable. %The naive implementation would be randomly assigning values for all the variables and checking at last, which is ineffective.




% In this way, the models

%\Luyao{this paragraph is not ready, we should add reason why we can not generate tensor first then match --> lead to graph be simpler.}
% If we choose the former (i.e., reusing an existing tensor), we will randomly pick a tensor from existing tensors that satisfies local constraints\Luyao{more details here}. If we choose the latter (i.e., generating a new tensor), the tensor will be randomly sampled under current constraints. Note, the construction process interacts with layered constraint simplification,


% \subsection{A Running Example}

% Based on graph-level reduction , our approach incrementally add operations one by one into the work-in-progress computation graph.

%To append a new operation in the existing model, our approach starts with randomly deciding the type of the new operation. After then, our approach randomly construct the attributes of the operation including input tensor(s), attributes of the operation (such as ‘strides’ in \CodeIn{Conv} operation).

% The type of the new operation is randomly chosen. As for our example, we choose \CodeIn{MatMul} operation. We need to construct this operation's two input tensors, marked as $A$ and $B$, with satisfying the semantic specification as shown in Equation~\ref{c1}-~\ref{c5}.


\subsubsection{Overall Process}
Starting with an empty model, we conduct \tone{} in a bottom-up way, i.e., repeatedly constructing a new operation and append it into the model.

To append a new operation in the existing model, our approach starts with randomly deciding the type of the new operation.
%After then, our approach randomly construct the attributes of the operation including input tensor(s), attributes of the operation (such as ‘strides’ in \CodeIn{Conv} operation).

Assume we decide the type of new operation as \CodeIn{MatMul}, next we illustrate how our approach works for appending \CodeIn{MatMul} operation.
Followed the layered form of variables to simplify the constraints, we first generate attributes of the operation. \CodeIn{MatMul} operation does not contain attributes so we skip this step, otherwise, our approach randomly construct the attributes of the operation such as ‘strides’ in \CodeIn{Conv} operation. We then directly starts to construct the input tensor (i.e. $A$ and $B$) one by one. Assume we first construct $A$ then $B$ (another case is similar). To construct $A$, based on the property of \cons{}, we only need to generate a tensor satisfying $P_A(A)$ (i.e. the constraints related only to tensor $A$). Here $P_A(A)$ only contains Equation~\ref{c1} (i.e. $dim_A \geq 2$). We have two choices for $A$: (1) reusing an existing tensor from the output tensor(s) of previous operations (i.e. $x_{out}$ and $y_{out}$), (2) generating a new tensor. We illustrate both of the results of these two choices in the left of Figure~\ref{fig:p2}. After determining tensor $A$, we plug it into the constraints, then the left constraints are only related to $B$. As a specific example, assume we already construct $A$ as a tensor with shape of $3 * 5$. By plugging the value of $A$ into the constraints $P(A, B)$, then constraints becomes to $P'(B)$ (i.e. $P(A, B)[A:\overline{A}]$), which is the same as Equation~\ref{c6}-\ref{c10}. 

% To generate tensor $B$, we model $B$'s dimension size as a variable $dim_B$, and each dimension as a variable marked as $b_1$, $b_2$, $b_3$, ..., respectively.
Next is the generation for $B$. We first care about the dimension size of $B$ (i.e. constraints $C_2'$ and $C_3'$). It is obvious that the generation of $dim_B$ has only one result: $dim_B = 2$.
For the next layer, we care about each dimension of $B$ and related constraints ($C_4'$ and $C_5'$). Because the values of variable $dim_A$ and $dim_B$ are all determined, we could use quantifier elimination to simplify $C_5'$ by substituting $dim(B)$ as the value of $dim_B$. Finally, the constraints would be simplified as $5 = B[1]$. The constraints after simplification reduces the valid domain of tensor $B$. To finally generate the tensor $B$ within its valid domain (i.e. an 2-dimension tensor with first dimension as 5). The construction of tensor $B$ also has two choices: reusing an existing one or generating a new one. Two different choices correspond to the different models as shown in the right of Figure~\ref{fig:p2}. The first choice of construction actually corresponds to the creation of an edge in the generated computation graph. With a strategy named controlled edge construction, we could define the distribution of these two choices. In this way, we could control the `density' of edges in the graph (measured by a metric named NOP in our evaluation). More details of this strategy are discussed in Section~\ref{sec:approach}.

%$B$ could also reuse an existing tensor or be newly generated.
%Based on layered constraint simplification, we could 

%The difference here is that we need to carefully generate $B$. Specifically, our approach matches (as for first choice) or samples (as for the second choice) a valid tensor $B$ (i.e. valid tensor does not violate the operation's semantic specification) under the situation that the tensor $A$ have been generated ahead. 
%We illustrate both of the cases in the right of Figure~\ref{fig:p2}. Finally, the different choices for tensor $B$ lead to different models as shown in the rightmost of Figure~\ref{fig:p2}.




%the pool of valid tensors to construct our tensor. 
%build a pool of valid tensors by filtering the existing tensorsvia tensor matching (as is shown in detail in Section 3). Then weIn the case of no existing tensor satisfying the currentconstraints, we would generate a new tensor as the first choice does.



% Fortunately, those dependencies are layered and could be resolved through a well-designed layered order of generation.
% Specifically, our generation process is layered into three levels. The first level is to determine the value of tensors' dimension size. The second level is to determine the value of the length of tensors' each dimension. The last level is to generate the specific values for the elements in the tensors.
% At each level, because the items that variables or constraints depend on have already been determined at the previous level, constraints could be simplified as quantifier-free variables with quantifier-free constraints.
% To solve the constraints after simplification, we propose a propagation-based method that could randomly sample the solution of the constraints as shown in detail in Section~\ref{sec:s4}. The main idea of propagation is determining the value of the last undetermined variable in some constraints based on other variables' value in the constraints.

%a well generation order of variables could simplify the constraints 

% If the current work-in-progress model passes with checking against the  semantic specifications, the approach continues the appending process; otherwise, it discards the current work-in-progress model and restarts the same process starting with an empty model. 

%The order of generation is actually the topological order of the computation graph.

% We could incrementally construct graph with following insight: the 


%Besides the challenge of constructing single operation, another challenge is how to construct edges on the computation graph. For 


%\subsection{Constraint Simplification}

%To address these issues, we design our approach with following two insights: (1) the constraints between different tensors are loop-free and arc-consistent, allowing ; (2) a well generation order of variables could simplify the constraints to qualifier-free and without structural constraints.


%\subsection{Approach Overview}
%\label{sec:approach}
%To address the challenge of generating deep learning models without violating the semantic specification, we design our effective random generation approach, which could randomly generate a valid deep learning model with soundness and completeness. 

%Due to the acycle trait of the computation graph, our approach incrementally constructs a deep learning model by randomly picking an operation and appending it into the current work-in-progress model (as the prefix of the final model). The order of generation is actually the topological order of the computation graph.

% To satisfy the semantic specification of deep learning models, let us first define the specification as the constraints on tensors. For example,  if operation $MatMul$ take two tensors as its input (i.e. $MatMul(A,B)$), then it will have several constraints as Equation~\ref{c1}-\ref{c5}, first two constraints ($C_1$ and $C_2$) are only related with single tensor, rest of constraints  ($C_3$, $C_4$ and $C_5$) are related to both of $A$ and $B$. 


%Due to the properties of semantic specification of operations in deep learning models, we will find (1)  those constraints between tensors are arc-consistent~\cite{} and (2) they are loop-free. \Luyao{explanation}

%The reason of arc-consistence is because new user-input tensors are always allowed in deep learning models, .
%As for the example of $MatlMul$, it always have a valid tensor $B$ after we determined tensor $A$.

%The above properties implies we could generate the tensors in arbitrary order with the guarantee of the existence of valid solutions. A direct way is to generate tensor one by one.

%To address this problem, we propose a technique named \textbf{\ttwo{}} inspired by quantifier elimination ~\ref{} to effectively sample solutions of the constraints on tensors.
%Our technique is mainly based on our following insights: the dependencies 
% In order to simplify quantifiers and complicate structural constraints, we need to know 

\fi
% -------Ignore------------------------------------------------------------------------------------------

\iffalse
Because the domain of quantifiers (such as $i$ in $C_5$) and the `indexes' in complicate structural item (such as $dim_A$ of $A$ in $C_4$) is finite, we could \Luyao{simplify} the constraints when the value of quantifiers and `indexes' is known. \Luyao{do we need it be finite?}

%For example, we could eliminate quantifiers in Equation~\ref{c5} after having determined the value of $dim(A)$, also, we could eliminate complicate structural constraints in Equation~\ref{c4} after having determined the value of $dim(A)$ and $dim(B)$.

Based on our insights on the properties of semantic specification of operations in deep learning models, we design a technique that effectively samples the solution of tensor(s) with satisfying their constraints by layering the sampling process. 

]
For each layer, we care about different attributes of the tensor. We could simplify the constraints in each layer into a qualifier-free constraint based on quantifier elimination technique.


%As an example, assume we already pick $x_{out}$ for $A$ by As an example, assume we already pick $x_{out}$ for $A$ tensor generation. To generate tensor $B$, we model $B$'s dimension size as a variable $dim_B$, and each dimension as a variable marked as $b_1$, $b_2$, $b_3$, ..., respectively.
%For the generation of the first layer, we only care about the dimension size of $B$. So current constraints is as follows: $C_2: dim_B \geq 2, C_3: 2 = dim_B$. It is obvious that the generation of $dim_B$ has only one result: $dim_B = 2$.
%For the second layer, we care about each dimension of $B$ and related constraints ($C_4$ and $C_5$). Because the values of variable $dim_A$ and $dim_B$ are all determined, we could use quantifier elimination to simplify $C_5$ by substituting $dim(A)$ as the value of $dim_A$ and $dim(B)$ as the value of $dim_B$. Finally, current layer's constraints could be simplified as $5 = B[1]$, the rest sampling process would be randomly generate value for $B[2]$. 
%The third layer here is to generate the tensor, we only need to generate a 2-dimension tensor with the corresponding shape (i.e. generate a $B$'s shape as $(b_1, b_2)$). The source of tensor contains two ways: (1) reusing an existing tensor from work-in-progress model; (2) generating a new tensor as one of the input tensor(s) of the whole model.

%\subsection{A running example}




%First layer contains the dimension size of $B$. Second layer contains each dimension size of of $B$.


if we take the constraints as `tensor' level, we will find that the constraints between tensors is arc-consistent and loop-free.


In order to achieve this goal, we propose two techniques.
The first technique is called bottom-up tensor generation. It based 
This property allows us first generate the attributes of the operations and the dimension of the tensor.

Before formally describing this technique in detail (as shown in Section ~\ref{sec:s4}), let us first take a concrete example for illustrating how our approach works in a nutshell as shown in Figure~\ref{fig:p1} and Figure~\ref{fig:p2}.

Our approach incrementally add operations one by one into the work-in-progress computation graph with ensuring the validity of current computation graph. To append a new operation in the existing model, our approach starts with randomly deciding the type of the new operation. After then, our approach randomly construct the attributes of the operation including input tensor(s), attributes of the operation (such as ‘strides’ in \CodeIn{Conv} operation).

In order to effectively generate valid tensors (i.e. the tensors that satisfy operations' constraints), 



The second technique is called constrained tensor sampling. There exists a well order of variables that we could sample the value of variables 

For example, if we first determine the value of $dim(A)$ as $2$, then the Equation~\ref{1f} could be simplify to $a[1] = b[1], a[2] = a[2]$. We could further take $a[1], a[2], b[1], b[2]$ as four variables $a_1, a_2, b_1, b_2$ to transform this constraint into traditional quantifier-free first-order formula as $a_1 = b_1, a_2 = b_2$.

Back to the example, assume we choose \CodeIn{MatMul} as the type for the new operation to append into the existing model as shown in Figure~\ref{fig:p1}. We need to construct this operation's two input tensors, marked as $A$ and $B$. In this example, assume we first construct $A$ then $B$ (another way is similar).

To construct $A$, we first conduct on-demand tensor generation, here, we have two choices for $A$: (1) reusing an existing tensor (the output of existing operations like $x_{out}$ and $y_{out}$), (2) generating a new tensor. First choice leads to tensor matching process, which is to get tensor candidates from existing tensors that will not violate \CodeIn{MatMul}'s semantic specification. Second choices leads to another main techniques named constrained tensor sampling, which is to randomly generate a valid tensor without violating the semantic specification. We illustrate both of the results of these two choices in the left of Figure~\ref{fig:p2}, more details are shown in Section~\ref{sec:s4}.

Similar to $A$, our approach constructs $B$ with on-demand tensor generation. $B$ could reuse an existing tensor or be newly generated. The difference here is that we need to carefully generate $B$ with taking the generated tensor $A$ into account. Specifically, our approach matches (as for first choice) or samples (as for the second choice) a valid tensor $B$ (i.e. valid tensor does not violate the operation's semantic specification) under the situation that the tensor $A$ have been generated ahead. We illustrate both of the cases in the right of Figure~\ref{fig:p2}. Finally, the different choices for tensor $B$ lead to different models as shown in the rightmost of Figure~\ref{fig:p2}.

Because of the ensuring of validity during generation, our approach holds the soundness of random generation for deep learning models. Completeness holds because that our approach does not miss any chance of generating arbitrary valid deep learning models. The detailed explanation of the soundness and completeness will be described in Section~\ref{sec:s4}.






\subsection{Key Techniques of Our Approach}
Our approach contains our two proposed techniques named on-demand tensor generation and constrained tensor sampling, inspired by our insights on arc consistency of tensor generation and layered dependencies of tensor constraints, respectively.

\subsubsection{On-demand tensor generation}
To construct tensors without violating the semantic specifications, we propose a technique named on-demand tensor generation, which allows us to consistently generate valid tensors.

It is mainly based on our observation of the property of arc consistency~\cite{apt2003principles} among constraints\footnote{If the input of the operation contains more than two tensors, the property will actually be `hyper-arc consistency' as shown in Section~\ref{sec:s4}.}. As the example of the constraints on tensors $A$ and $B$, we denote the constraints  related only to tensor $A$ as $P_A(A)$, i.e, $P_A(A):=dim(A)\geq 2$, which is the same as $P_B(B):=dim(B)\geq 2$ for $B$, and the rest of constraints related to both tensor $A$ and tensor $B$ as $P_{AB}(A, B)$. The arc consistent means for any tensor $A$ satisfying $P_A(A)$ there always exists a tensor $B$ that $P_B(B)$ and $P_{AB}(A, B)$ both holds, and vice versa.
Formally, $\forall A, \ P_{A}(A) \rightarrow	\exists B,\ P_{B}(B) \bigwedge P_{AB}(A, B)$,
and also, $\forall B, \ P_{B}(B) \rightarrow	\exists A,\ P_{A}(A) \bigwedge P_{AB}(A, B)$.

Arc consistency allows us to first construct a tensor to satisfy only its local constraints, and then construct another tensor to satisfy the remaining constraints. In other words, the problem of constructing two tensors reduces to problems of constructing one tensor. Now we discuss how we construct one tensor. Generally, there are two ways to construct an input tensor: generating a new tensor as a user-input tensor/constant tensor; or reusing an existing tensor (the output of existing operations or the user-input tensors). 
%For the input tensors we need to construct, because we are always enabled to choose the first one (i.e., generating a new tensor) among two kinds of ways, the arc consistency always holds.
% Based on this property, it enables us to generate tensors one by one with the ensuring on validity (the existence of the valid solution).  
% For the generation of a single tensor, 
Our approach randomly chooses a kind of source.
% controlled by a hyperparameter $picking \ rate$. 
If we choose the former (i.e., generating a new tensor), our approach would conduct constrained tensor sampling solving as shown in the next paragraph.
If we choose the latter (i.e., reusing an existing tensor), we will build a pool of valid tensors by filtering the existing tensors via tensor matching (as is shown in detail in Section~\ref{sec:s4}). Then we randomly pick a tensor from the pool of valid tensors to construct our tensor. In the case of no existing tensor satisfying the current constraints, we would generate a new tensor as the first choice does.

% $Picking \ rate$ actually controls the connection status of deep learning model, in order to avoid generating many separated graph in the deep learning model, we set it relatively high (preference on the first choice). We call it on-demand tensor generation as the first novelty technique in our approach.

\subsubsection{Constrained tensor sampling}
To effectively construct a new tensor (i.e. assign the value of the tensor) without reusing an existing one, we propose a technique called constrained tensor sampling. Taking the generation as a constraint solving problem, our technique effectively samples a random solution (i.e. a tensor which satisfies the semantic specifications of the operation) for the constraints without any retrying.

Let us take all of the items in the constraints (i.e. Equation~\ref{1a} - ~\ref{1f}) as variables, which denote the attributes of the tensors. Unlike traditional constraints, which can be expressed in the first-order logic without quantifier,

there are two types of special dependencies here. First, the existences of some variables depend on some other variables. For example, the variable $a[2]$ (i.e., the length of tensor $A$'s second dimension) exists only when $dim(A) \geq 2$. Second, the constraints may use universal quantifiers whose range is determined by other variables, and thus the existence of some constraints is dependent on some other variable. For example, given a constraint: $\forall 1 \leq i \leq dim(A) - 2, a[i] = b[i]$, there exists an equivalent constraint between $a[1]$ and $b[1]$ only when $dim(A)$ is larger than 2.

Those constraints cannot be directly modeled as standard SMT-lib ~\cite{barrett2010smt}.
Solvers like Z3~\cite{DBLP:conf/tacas/MouraB08} are not directly applicable. The naive implementation would be randomly assigning values for all the variables and checking at last, which is ineffective.

Fortunately, due to the trait of deep learning specifications, those dependencies are layered and could be resolved through a well-designed layered order of generation.
Specifically, our generation process is layered into three levels. The first level is to determine the value of tensors' dimension size. The second level is to determine the value of the length of tensors' each dimension. The last level is to generate the specific values for the elements in the tensors.
At each level, because the items that variables or constraints depend on have already been determined at the previous level, constraints could be simplified as quantifier-free variables with quantifier-free constraints.
To solve the constraints after simplification, we propose a propagation-based method that could randomly sample the solution of the constraints as shown in detail in Section~\ref{sec:s4}. The main idea of propagation is determining the value of the last undetermined variable in some constraints based on other variables' value in the constraints.
%\Luyao{Do we need to describe our approach for solving linear constraints(propagation process) in detail here?} 


% We consider the variables or constraints whose existences are dependent on some other attributes as attribute-dependent. For an attribute-dependent $t$, if the values of attributes that $t$ is dependent on are all known, we consider $t$ as determined. In other words, at that moment, $t$'s existence is determined by the other known values of some attributes.
% If we treat the attributes and constraints as nodes in a graph, and treat the dependencies as edges, also, add edge between a node of constraint and a node of variable if the variable appears at the constraint
%Fortunately, the dependence graph formed by these two types is acyclic. \Luyao{describe the graph}

%Based on this observation, we can classify the attributes into a sequence of groups, such that none of the attribute in an earlier group depends on an attribute in a later group, and then we can assign the values of the variables following this order. \Luyao{remove group concepts?}


% none of them depends on an attribute that is after it in the sequence. The reason is that the constraints of operations have the acyclic trait on dependencies, ensuring the existence of such sequence, and we call it the  \emph{dependency-level} acyclic trait. With this insight, we can attempt to assign the values of the attributes followed by the order. The benefit of such ordering is that all the attribute-dependent attributes or constraints related to the current attribute will be determined.

As the example of \CodeIn{MatMul}, when it comes to the second level after determining the value of $dim(A)$ at the first level, the constraint $a[i]=b[i], \forall \in [1, 2, ..., dim(A)-2]$ could be simplified as quantifier-free because the value of $dim(A)$ is known. Actually, in each level, the constraints after simplification are composed of only preliminary linear expressions between variables, allowing us to easily sample the values for each variable via propagation. The soundness and completeness is guaranteed by the property of the acyclic trait on propagation (we will discuss in detail in Section~\ref{sec:s4}). Finally, at the third level, after the value of the tensor's dimension size and each dimension's length are determined, we generate random numerical values to fill in each element in the tensor. 

\fi

% As the example of \CodeIn{MatMul}, if we choose to generate a new tensor for $A$, we will start with first level which is to determine the value of $dim(A)$. Now, we only need to satisfy $dim(A) \geq 2$ here, assume we pick $dim(A)=2$. After that we could move to second level which is to determine the value of $a[i]$ ($i$ denotes an arbitrary integer). Because the value of $dim(A)$ is determined by previous level, we could simplify the constraint of $a[dim(A)]=b[dim(B)-1]$ as $a[2]=b[1]$. And the constraint of $a[i]=b[i], \forall \in [1, 2, ..., dim(A)-2]$ could be simplified as quantifier-free (actually it could be ignored because the range of $i$ is empty). Also, the constraints after simplification are composed by only preliminary linear expression between variables. This property allows us to easily determine the value of $a[i]$ which are globally valid. 


% A straightforward way is to first generate all input tensors, and then match with existing tensors. However, this way has a low chance on successfully matched cases.

%In our example, take the maximum length of each dimension as $L$, all tuples $(x, y, z)$ can be generated as $a[1] = x, a[2] = b[1] = y, a[3] = z$ for satisfying the constraint of $a[2] = b[1]$. However, considering the whole space for tuple's value space ($O(L^3)$), it is less possible that an existing 2-D tensor can be matched with $x * y$ or $y * z$ whose probability is $O(2/L^3)$. This factor causes one of the drawbacks of the straightforward way: a large number of isolated small parts in the computation will be generated.

% On-demand tensor generation overcomes it by directly copying the matched to the generated tensor after checking the validity. This process is like assigning values on variables in a batch. In order to avoid backtracking, we need to check whether those batch assignments satisfy the constraints. Fortunately, because of the characteristic of the operation's constraints, we have the opportunity to efficiently conduct those checks.


% A well order can simplify the attribute-dependent situation that causes attributes and constraints to become quantifier-free during the process of value assignment. However, directly applying a search algorithm to achieve the satisfactions of all constraints still needs backtracking when it faces the constraint violation, even with a well order. In order to assign the values of attributes for satisfying all the constraints without backtracking, we design a technique named propagation. The idea is to determine the values of unassigned attributes based on the constraints. For example, if there is a constraint of $a[2]=b[1]$, and $a[2]$ has already been assigned a value, but $b[1]$ has not, then we can get the value of $b[1]$ by propagation on the constraint. The insight behind this technique is the third acyclic trait that we call \emph{propagation-level} acyclic: if we treat both the variables and the quantifier-free constraints as nodes and add edge between a node of constraint and a node of variable if the variable appears in the constraint, the this graph is acyclic so we could safely conduct propagation as determining some attribute's value without backtracking.


% \Luyao{I move the concrete example with pictures to the approach section.}

% ------------------------------------------------------------------------------------------------------------
% ------------------------------------------------------------------------------------------------------------
% ------------------------------------------------------------------------------------------------------------
% ------------------------------------------------------------------------------------------------------------
% ------------------------------------------------------------------------------------------------------------


==> arXiv-2302.00842v2/sections/prop.tex <==

we design our delicate order for simplification on constraints.
, with constraint propagation, any order for instantiation is consistent. With this property, we design our delicate order for simplification on constraints.

\Luyao{or graph-level global consistency?}
The first property is called
\subsubsection{graph-level consistency}

%With taking each node as a variable (a set variable containing all of the elements related to a node), constraints of the computation graph form a binary CSP, consisting of two kinds of constraints: first are unary constraints on each node, and second are binary constraints between two nodes (i.e., the output of an node equals to the input of another node).

We call an operation $x$ is locally satisfied with the instantiation $Q$ if $eval(Q[\{Input_x, Attr_x\}], Spec_{OP_x}(Input_x, Attr_x)) = true$. 
An instantiation $Q$ on a computation graph holds global satisfaction, if all of operations in the graph are locally satisfied with $Q$.
A computation graph with global satisfaction, as well as no loop in the graph, corresponds to a semantically valid computation graph.

Because our instantiation follows the topological order of the computation graph, with only instantiating edges which are from previous nodes (nodes that are ahead of $x$ in the order) to current operation $x$, the instantiation on $x$ will not affect local satisfications of previous nodes (based on the property of topological order). Thus, as long as we are able to instantiate a new operation with its local satisfaction every time, the final instantiation will holds global satisfaction. Also, because we instantiates edges with the direction followed by the topological order, the overall graph is loop-free. Thus, following with the topological order, local satisfaction on each operation implies global satisfaction, also, leading to a semantically valid computation graph finally.


%for each operation $x$, only the output of operations that are ahead of $x$ in the order may affect the local satisfaction of $x$ (taking the output of an previous operation as the input of $x$). So when we instantiate operation $x$ in the order, its instantiation will not affect the local satisfication of operations ahead of $x$.



reduce the domain of $x$ by constraint propagation. Due to the acyclicity of topological order, the constraint propagation is loop-free. Also, we are able to generate


Because there is 

For a semantically valid computation graph, 

In Section~\ref{sec:approach}, we show that our instantiation for this CSP is consistent: by instantiating with the topological order, ensuring the constraints related to each single operation (local consistency) implies the satisfication of the overall constraints (global consistency).


\subsubsection{operation-level strong n-consistency}

The second property is called operation-level strong n-consistency. For the constraints related to each single operation, after determining the type and the number of tensors in the input, we could take attributes as a variable and each tensor in the input of the operation as a variable, then this CSP is strong n-consistency~\cite{apt2003principles}.

A strongly n-consistency CSP has the property that any consistent instantiation of a subset of the variables can be extended to a consistent instantiation of all of the variables~\cite{dechter1992local}.
Thus, any order for instantiation is consistent. With this property, we design our delicate order for simplification on constraints.

Above two good properties ensure the consistency of our instantiation during the whole process, thus our approach is sound, as well as, backtracking-free (no inconsistent instantiation will appear). Also, our approach samples solutions from the whole semantically valid space, so it is also complete.



\subsubsection{Properties of \tone{}}

%The first property is called graph-level consistency\Luyao{or graph-level global consistency?}. 
With taking each node as a variable (a set variable containing $Op_x$, $Input_x$, $Output_x$, $Attr_x$), then the constraints related to each operation (e.g. Equation~\ref{eqs1} and \ref{eqs2}) is an unary constraint, and each map in $\psi_G$ corresponds to a binary constraint on two variables (the output of an node equals to the input of another node), so it is a binary CSP. 
\Luyao{With the guarantee of some properties}
Thus, this CSP is always consistent, which means that ensuring the constraints related to each single operation (local consistency) implies the satisfication of the overall constraints (global consistency).

The second property is called operation-level strong n-consistency. For the constraints related to each single operation, after determining the type and the number of tensors in the input, we could take attributes as a variable and each tensor in the input of the operation as a variable, then this CSP is strong n-consistency~\cite{apt2003principles}. A strongly n-consistency CSP has the property that any consistent instantiation of a subset of the variables can be extended to a consistent instantiation of all of the variables~\cite{dechter1992local}.

For a computation graph $G$, taking each operation as a variable, it contains two types of constraints: unary constraint of each variable (operation's semantic specification on its attributes and input), and binary constraint of two nodes (the output of one operation is the input of another operation). The problem $P_G$ is a binary CSP.

A set of binary constraints that is arc consistent and has no empty domain can be inconsistent only if the network of constraints contains cycles ~\cite{}.
Because the graph $G$ is acyclic, so the 

\Luyao{todo}



\subsubsection{Properties of \ttwo{}}

% Not all of the computation graphs have a valid model. 

After determining $OP_x$ and $Indegree_x$, we could take $Attr_N$ as a set variable, and each tensor in $Input_x=\{in_1, in_2, in_3, ...\}$ as a variable.
Consider the problem $P:(Spec_{OP_N}, ..., \{Attr_{N}, in_1, in_2, in_3, ...\})$, it is strong n-consistent because that 

(1) the property of constraints. \Luyao{propagtion is a tree.}

(2) the allowance of the second way in our on-demand policy ensures that the domain is non-empty.

It indicates that the order of instantiation will not affect the consistency of instantiation.

%for every $i \in [1..k]$ and $a \in D(T_i)$, there exists a solution $Q \in sol(P)$ such that $a=Q[Str(T_i)]$.
% Back to the beginning of our construction, if we select reusing an existing tensor for $A$, then we will conduct the tensor matching process. The situation for tensor matching is trivial here because there is no instantiation yet. Thus all the existing tensors will be matched. Assume we choose the tensor $X_{out}$ which is the output of operation $X$. Then, we will assign value of attributes of $X_{out}$ to corresponding attributes of $A$: $a.len: 2, a[1]: 3, a[2]: 5$.


==> arXiv-2302.00842v2/sections/relatedwork.tex <==
\iffalse
\section{Discussion and Future Work}
Although our goal in this paper is to generate tests for deep learning compilers, the application scenarios of our approach may not be limited to deep learning compilers. It may also apply to other compilers which take graph-like structures as their inputs, such as the graph database engines. \Luyao{todo}

For test oracles in our testing, we can use other techniques like equivalence modulo inputs (EMI). For example, TASO~\cite{DBLP:conf/sosp/JiaPTWZA19} aims to generate graph substitutions to optimize the deep learning model. Similar to TASO, we can use equivalent variants of operators or the combination of operators as test oracles to check if the output is consistent after substitution.
\fi

%\section{Threats to Validity}
%The threat to internal validity mainly lies in the implementation of our approach whether our implementation correctly captures our approach. To alleviate the threat, we have manually checked all the bugs detected by our approach, and analyzed the reasons for the false positives, validating the implementation to some extent.

%Manual checking on the detected bugs may leads to XXXX.



\section{Related Work}

\textit{Random Testing and Test Generation}. 
Random testing~\cite{orso2014software} simply constructs test inputs in a random manner. For example, Randoop~\cite{pacheco2007feedback} and EvoSuite~\cite{fraser2011evosuite} aim to generate JUnit tests for classes by incrementally combining sequences of method calls. Besides many aspects of advantages, random testing still faces problems including inefficiency, imprecision, and lack of available information to guide test generation.
%As an effective alternative to random testing, adaptive random testing~\cite{DBLP:journals/jss/ChenKMT10} was proposed to enhance random testing’s failure-detection capability.
To test deep learning compilers, our work conducts random testing by enhancing the effectiveness of test generation.
Another test generation way is bounded-exhaustive testing. For example, UDITA~\cite{gligoric2010test} uses bounded-exhaustive testing to enumerate the paths through the generator with various optimizations. For deep learning models, the space of computation graph and the shape of tensors in it can be super large, and the valid space is very sparse; thus, it is intolerable to enumerate all kinds of the inputs by searching.

%Also, UDITA is still based on search, their strategies would be inefficient for deep learning model's specification.
% Torlak~\cite{DBLP:conf/sigsoft/Torlak12} proposes a framework of test generation for multidimensional models. It provided a domain-specific language for specifying multidimensional models, and a solver for generating sample data from them with the desired statistical properties.

\textit{Grammar-based Fuzzing}.
Fuzzing is a common approach for randomly generating inputs to test software.
%Blackbox fuzzing generates inputs for a target program without knowledge of its internal behavior or implementation.
It may generate inputs from scratch, or do mutation on a series of valid seed inputs. 
Without any knowledge of the input of the software under test, generating valid inputs randomly is ineffective, especially for the software such as compilers whose inputs are highly-structured.
% Coverage-guided fuzzing~\cite{afl} uses code instrumentation to trace the code coverage reached by each input fed to a fuzzing target.
%Fuzzing engines use coverage information to guide the mutation to maximize coverage.
To improve it, grammar-based fuzzing~\cite{godefroid2008grammar, DBLP:conf/uss/HollerHZ12} is proposed, which relies on a grammar specification to generate structured inputs, usually in context-free forms. Deep learning models with semantic specifications fail to be represented as a context-free grammar.
Recently Padhye et al.~\cite{padhye2019semantic} propose Zest, which is based on coverage-guided fuzzing, targeting at producing semantically valid inputs. 
However, Zest still requires developers to manually design a generator that can construct syntactically valid test programs. Different implementations for the generator could highly affect the effectiveness of test generation, especially for languages with complicated specifications such as deep learning models.
%Besides, Zest needs the coverage information to guide its fuzzing, while our approach is a blackbox one and does not need runtime information.

% \textit{Combinatorial Testing} Combinatorial testing is a test approach with the insight that many software faults will be triggered only by an unusual combinatorial interaction of more than two parameters and testing combinations of parameters can provide highly effective fault detection~\cite{DBLP:journals/ac/KuhnBDGLK15}.  

\pre{
\textit{Testing Deep Learning Engines}. 
CRADLE~\cite{DBLP:conf/icse/PhamLQT19} is proposed to detect and localize bugs in deep learning libraries by checking the inconsistency in multiple implementations of the same algorithms.
% LEMON~\cite{DBLP:conf/sigsoft/WangYCLZ20} is a mutation-based approach for testing deep learning libraries. It uses a series of mutation rules and some heuristic strategies to guide the model generation process.
%Luo et al.~\cite{DBLP:conf/icse/LuoCRWFC21} propose a graph-based fuzz testing technique with Monte Carlo Tree Search to drive the fuzzing process.
TVMFuzz~\cite{DBLP:conf/sigsoft/ShenM0TCC21} conducts fuzzing techniques to test deep learning compilers with some mutation operators to facilitate type-related bug detection.
LEMON~\cite{DBLP:conf/sigsoft/WangYCLZ20} and Muffin~\cite{DBLP:conf/icse/GuLZ022} are two recent work proposed to test deep learning libraries.
Both of these work generate deep learning models by applying some heuristic rules.
LEMON uses a series of mutation rules to guide the model generation process.
And Muffin ensures the semantic specification in a hardcode way: by inserting the reshape layers between adjacent layers in origin models.
Compared to LEMON and Muffin, our approach is able to generate more diverse deep learning models because we directly resolve semantic specification by constraint solving techniques. Besides, we generate deep learning models at the level of computation graph, by contrast, previous work either targets at a higher level (model expressed in encapsulated layers provided by deep learning library APIs) or targets at a lower level (such as TVMFuzz on the IR of compilers) which is usually compliler-dependent.
}

\rev{
\textit{Testing Deep Learning Toolkits}. 
Deep learning toolkits include deep learning libraries (frameworks) and deep learning compilers. The differences between them lie in their primary functions and interfaces provided to users, which result in divergent emphases in designing corresponding testing approaches.

Deep learning libraries, such as Keras and TensorFlow, are primarily used for simplifying the implementation of deep learning models, they provide high-level APIs and abstractions of pre-defined layers/models as well as optimizers, loss functions and other utilities that allow users to easily define and train deep learning models. To test deep learning libraries, LEMON~\cite{DBLP:conf/sigsoft/WangYCLZ20} and Muffin~\cite{DBLP:conf/icse/GuLZ022} focus on generating parameters and call sequences of high-level APIs.

%Though they are not specifically designed for testing deep learning compilers, we can translate the model constructed by high-level APIs into computation graphs.

%User defines DL model via APIs of deep learning framworks. Those APIs are high-level APIs, usually descibing a layer of DL model. 
%For example, existing work LEMON and Muffin generates Keras model
Deep learning compilers, such as TVM, are designed to transform deep learning models into efficient low-level code for deployment and execution on different hardware devices,
%DL compilers will compile DL model into hardware-specific low-level languages.
and they focus on optimizing the computational graph of the models to improve execution efficiency.
To test deep learning compilers, one direction is to directly generate inputs of deep learning compilers, i.e., computation graphs, including research work GraphFuzzer~\cite{DBLP:conf/icse/LuoCRWFC21} and MT-DLComp~\cite{DBLP:journals/pomacs/XiaoLYPW22}; another direction is to fuzz low-level intermediate representation of the compiler (e.g., TVM's compiler-specific intermediate representation), including research work TVMFuzz~\cite{DBLP:conf/sigsoft/ShenM0TCC21} and Tzer~\cite{DBLP:journals/pacmpl/LiuWYDZ22}.
%another direction is to directly construct deep learning compiler's input, i.e., computation graphs. 
Our approach, \toolname{}, as well as its two parallel works NNSmith~\cite{NNSmith} and HirGen~\cite{HirGen} belong to the former, i.e. test generation of computation graphs.

%generating computation graphs for testing deep learning compilers
%Our approach focuses on test generation for deep learning compilers, aims to effectively generate diverse test inputs, i.e., computation graphs.
}

\rev{
To generate test inputs for deep learning toolkits, the validity of test inputs is a critical challenge: invalid test inputs will largely diminish effectiveness and efficiency of testing.
To address it, different techniques are proposed by existing research work.
For example, Muffin~\cite{DBLP:conf/icse/GuLZ022}, GraphFuzzer~\cite{DBLP:conf/icse/LuoCRWFC21} and HirGen~\cite{HirGen} are all restricted to certain types of operations and connections for generating computation graphs, which will bias the generated graphs.
Specifically, Muffin~\cite{DBLP:conf/icse/GuLZ022} ensures the semantic specification by inserting the reshape layers between adjacent layers in origin models. Unfortunately, doing so biases the generated computation graphs to include many \CodeIn{Reshape} operations as shown in our evaluation.
GraphFuzzer~\cite{DBLP:conf/icse/LuoCRWFC21} and HirGen~\cite{HirGen} try to adjust mismatched tensor shapes through slicing and padding. They will also bias the generated computation graphs to include
many \CodeIn{Slice} and \CodeIn{Padding} operations.

%However, all of them will introduce biases on the generated models and extra overhead of test generation.

%Generation-based approaches, including two previous work Muffin~\cite{DBLP:conf/icse/GuLZ022} and GraphFuzzer~\cite{DBLP:conf/icse/LuoCRWFC21}, as well as two parallel work NNSmith~\cite{NNSmith} and HirGen~\cite{HirGen}, conducts different techniques for resolving the validity challenge.

%should conform the specifications of deep learning models, otherwise much testing budget is wasted on invalid test inputs.
% To address it, different techniques are proposed by previous work. We mainly categorize them as two types: mutation-based and generation-based.

%consistent with the traditional compiler testing ~\cite{DBLP:conf/pldi/YangCER11}

% Mutation-based approaches, including  TVMFuzz~\cite{DBLP:conf/sigsoft/ShenM0TCC21}, Tzer~\cite{DBLP:journals/pacmpl/LiuWYDZ22}, LEMON~\cite{DBLP:conf/sigsoft/WangYCLZ20}, and MT-DLComp~\cite{DBLP:journals/pomacs/XiaoLYPW22}, conduct a series of heuristic-based mutation rules on seed inputs (i.e., existing models). 
% %Seed inputs (i.e., existing test cases) are required by testing approaches such as mutation-based testing~\cite{DBLP:conf/sigsoft/ShenM0TCC21} whose
% To preserve validity to a large extent, mutation-based approaches often highly depend on the quality of mutation rules and seed inputs.
% As a result, they suffer following limitations: (1) mutations inherit the structures of seed inputs, limiting the exploration of diverse inputs; (2) seed inputs, especially high-quality seed inputs, may do not exist in various situations in practice, e.g., for testing new operations in the latest version of deep learning compilers. \TODO{refine...}

%mutation rules are usually carefully designed
%The effectiveness and efficiency of mutation-based approaches often highly depend on the mutation rules and the quality of seed inputs. Thus, these work suffer following limitations: (1) seed inputs, especially high-quality seed inputs, may do not exist in various situations in practice, e.g., for testing new operations in the latest version of deep learning compilers; (2) 


%however, seed inputs, especially high-quality seed inputs, do not exist in various situations in practice, e.g., for testing new operations/APIs of deep learning frameworks in the latest version of compilers with few test cases/users.


%Tzer~\cite{DBLP:journals/pacmpl/LiuWYDZ22} focuses on mutation-based fuzzing on the relay (i.e., TVM's low-level IR). It uses existing DL models' IR as seeds, and conducts mutations on IR to derive other test inputs.
%MT-DLComp~\cite{DBLP:journals/pomacs/XiaoLYPW22} is a mutation-based approach. It mutates seed deep learning models to generate equivalent models.
%Besides above mutation-based approaches on testing deep learning compilers, generation-based approaches are also recently proposed. There are two research work, which is parallel with our approach: HirGen~\cite{HirGen} and NNSmith~\cite{NNSmith}. 
%HirGen~\cite{HirGen} is a generation-based fuzzer for testing deep learning compiler. HirGen uses the high-level IR’s language features to generate diverse IRs of deep learning models, and uses the same test oracles as our approach: runtime failure and inconsistency from differential testing.
%NNSmith is also a generation-based approach.\TODO{...}

%To ensure validity,
%To resolve the validity challenge, 


%HirGen~\cite{HirGen} absorbs specifications of deep learning models as type checker and shape checker and uses checkers to avoid invalid models. The process of HirGen's test generation is similar to the settings of \emph{\btwoshort{}} in our compared work.

NNSmith~\cite{NNSmith}, as a parallel work with ~\toolname{}, addresses the validity challenge by leveraging the existing constraint solver Z3~\cite{DBLP:conf/tacas/MouraB08}. However, it leads to a further problem which is lack of diversity due to that existing constraint solvers tend to pick boundary values for constraints.
To relieve this problem, NNSmith tries to iteratively add extra constraints (named ``attribute binning''~\cite{NNSmith}). When extra constraints produce an unsatisfiable one, NNSmith will randomly drop some of the constraints and retry, until it succeeds.
It results in following disadvantages: (1) extra overhead for constraint solving due to the iteratively retrying; (2) a biased distribution of operations and parameters in the generated models, the models tend to contain more ``simple'' operations such as \CodeIn{Add} and \CodeIn{Sub}, and less ``complicated'' operations such as \CodeIn{Conv} and \CodeIn{Gemm} (as seen in both of the results in NNSmith's paper~\cite{NNSmith} and our evaluation).

Compared with related work, our test generation approach overcomes the validity challenge by the domain-specific constraint solver proposed in this paper. It offers several advantages as follows: %\TODO{refine and add more reasons.}
\begin{itemize}
    \item The computation graphs generated by our approach are more diverse because our domain-specific constraint solver can sample diverse operations/parameters without bias, as evidenced in our evaluation.
    \item
    Our approach is more efficient due to lower computational costs compared to other solutions such as repeatedly calling the external constraint solver (as NNSmith did), as evidenced in our evaluation.
    \item Our approach is more scalable because our domain-specific constraint solver is lightweight and backtrack-free,
    without inherent limitations on the type and the size of generated computation graphs, which is potentially beneficial for other scenarios such as generating extreme test cases for stress testing.
    % to generate computation graphs 
\end{itemize}

Besides test generation for valid computation graphs, existing research work also proposes other techniques to enhance the effectiveness of deep learning compiler testing, which are orthometric to our approach.
NNSmith~\cite{NNSmith} conducts value searching for improving numeric validity with gradients. HirGen~\cite{HirGen} proposes ``disruptive generation'' to generate computation graphs containing obvious breaks of specifications for detecting incorrect exception handling bugs.
In addition, mutation-based approaches such as  TVMFuzz~\cite{DBLP:conf/sigsoft/ShenM0TCC21} and Tzer~\cite{DBLP:journals/pacmpl/LiuWYDZ22}, %LEMON~\cite{DBLP:conf/sigsoft/WangYCLZ20}, and MT-DLComp~\cite{DBLP:journals/pomacs/XiaoLYPW22},
conduct a series of heuristic-based mutation rules on seed inputs (i.e., existing models) at the compiler's low-level intermediate representation.
Our approach is complementary to these techniques.
}
% Compared to TVMFuzz, \toolname{} has the following additional advantages: (1) \toolname{} could generate inputs without requiring seed inputs, but TVMFuzz requires the existing test suite as its seeds; (2) \toolname{} generates inputs for deep learning compiler at the model level, naturally supporting cross-compiler testing, whereas TVMFuzz generates inputs at the Relay level being compiler-dependent. \Luyao{refine}
%Compared to the preceding related work on testing deep learning libraries or % compilers, our approach has two major differences:
%(1) our approach generates deep learning models based on constraint solving techniques, while other approaches use heuristic rules to resolves constraints: LEMON~\cite{DBLP:conf/sigsoft/WangYCLZ20} design some mutation rules, and Muffin~\cite{DBLP:conf/icse/GuLZ022} ensure the semantic specification in a hardcode way: by inserting the reshape layers between adjacent layers in origin models; (2) 

%Computation graph expressed in a common set of operations such as ONNX Standard~\cite{onnx_standard} are powerful to express deep learning models among a variety of different frameworks, which is suitable for testing deep learning compilers.

%besides, our approach is a blackbox approach without requiring the internal runtime information of deep learning compilers or libraries.
%generates deep learning models without requiring seed inputs 

% \textit{Testing Deep Learning Models and Architectures} Pei~\cite{DBLP:conf/sosp/PeiCYJ17} first proposed neuron coverage to guide the testing of deep learning models. Odena~\cite{DBLP:conf/icml/OdenaOAG19} developed coverage-guided fuzzing methods on neural networks and applied the approximate nearest neighbors algorithm to guide their test generation. Zhang~\cite{zhang2020detecting} proposed DEBAR based on static analysis to detect numerical bugs in deep learning architectures. Those approaches focus on detecting bugs in a given deep learning models which is not within the scope of our work. They will analyze a given deep learning model (usually a commonly used model in some application scenarios), and generate input to trigger the erroneous behaviors of the deep learning model or point out the position of erroneously implemented deep learning model. By contrast, our work focus on generating valid deep learning model to detect bugs in deep learning compilers. Deep learning compilers take deep learning model as their inputs, but our work aims to validate the correctness of deep learning compiler, not its input.




==> arXiv-2302.00842v2/tables/bugs.tex <==
%\begin{table}[]
%\begin{minipage}[t]{0.4\textwidth}

\rev{
%\begin{threeparttable}

%\tiny
%\renewcommand\arraystretch{0.95}
\setlength{\tabcolsep}{2pt}

\caption{\rev{Previously unknown bugs detected by \toolname{}.}}
\label{unknownbugs}
\begin{tabular}{cccccc}
ID        & Type         & Location & Confirmed        & Fixed            & Issue ID \\
TVM-1     & error        & backend  & \textless 1 day  & 10 days          & 7200     \\
TVM-2     & error        & frontend & \textless 1 day  & \textless 1 day  & 7202     \\
TVM-3     & error        & frontend & \textless 1 day  & 6 months         & 7241     \\
TVM-4     & error        & frontend & \textless 1 day  & \textless 1 day  & 7244     \\
TVM-5     & error        & backend  & 7 months         & 7 months         & 7262     \\
TVM-6     & error        & frontend & 42 days          & 42 days          & 7263     \\
TVM-7     & error        & frontend & \textless 2 days & 10 months        & 8889     \\
TVM-8     & error        & backend  & \textless 2 days & 10 months        & 8890     \\
TVM-9     & inconsistency & backend  & N/A              & 10 months        & 7270     \\
TVM-10    & inconsistency & unknown  & N/A              & N/A              & 12734    \\
TVM-11    & error        & unknown  & N/A              & N/A              & 12735    \\
Glow-1    & error        & backend  & 13 days          & N/A              & 5995     \\
Glow-2    & error        & unknown  & N/A              & N/A              & 5991     \\
SophGo-1  & error        & frontend & \textless 3 days & N/A              & *        \\
SophGo-2  & error        & backend  & \textless 3 days & \textless 7 days & *        \\
SophGo-3  & error        & backend  & \textless 3 days & \textless 7 days & *        \\
SophGo-4  & error        & frontend & \textless 3 days & \textless 7 days & *        \\
SophGo-5  & error        & backend  & \textless 3 days & \textless 7 days & *        \\
SophGo-6  & error        & backend  & \textless 3 days & \textless 7 days & *        \\
SophGo-7  & inconsistency & backend  & \textless 3 days & \textless 7 days & *        \\
SophGo-8  & error        & frontend & \textless 3 days & \textless 7 days & *        \\
SophGo-9  & error        & frontend & \textless 3 days & \textless 7 days & *        \\
SophGo-10 & error        & frontend & \textless 3 days & N/A              & *        \\
SophGo-11 & error        & backend  & \textless 3 days & \textless 7 days & *       
\end{tabular}

}


% \begin{tablenotes}    %这行要添加， 从这开始
% \footnotesize               %这行要添加
% \item[1] For reference, the URLs of TVM and Glow's bug reports are https://github.com/apache/tvm/issues/\#IssueID, and https://github.com/pytorch/glow/issues/\#IssueID. The URLs of SophGo's bug reports are internal which are not public available.
% \end{tablenotes}            %这行要添加
% \end{threeparttable}       %这行要添加，到这里结束
% }

% \end{minipage}
% \end{table}




==> arXiv-2302.00842v2/tables/nofbugs.tex <==
		\centering
        \tabcolsep=0.4mm
		%\caption{\# unique bugs detected on different compilers.}
        \label{tab:bug_number}
        % \begin{tabular}{cccccc}
        %     & \toolname{} & \boneshort{} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Randoop-\\ Gen\end{tabular}} & Muffin & TVMFuzz \\
        %     TVM        & \textbf{18}      & 8                            & 14                      & 12     & 5       \\
        %     Glow       & \textbf{4}       & 2                            & 2                       & 2      & -       \\
        %     SophGo     & \textbf{11}      & 3                            & 3                       & 9      & -       \\
        %     Total      & \textbf{33}      & 13                           & 19                      & 23     & 5      
        % \end{tabular}
        % \boneshort{}
        \renewcommand\arraystretch{2}
        \begin{tabular}{ccccccc}
            & \toolname{} & \boneshort{} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Randoop-\\ Gen\end{tabular}} & Muffin & TVMFuzz & \rev{NNSmith\footnotemark}  
            \\
            TVM        & \textbf{18}      & 8                            & 14                      & 12     & 5  & \rev{\textbf{21}}     \\
            Glow       & \textbf{4}       & 2                            & 2                       & 2      & -  & \rev{\textbf{4}}     \\
            SophGo     & \textbf{11}      & 3                            & 3                       & 9      & -  & \rev{7}     \\
            Total      & \textbf{33}      & 13                           & 19                      & 23     & 5  & \rev{\textbf{32}}    
        \end{tabular}

        % \footnote{The number of NNSmith's detected unique bugs is different to the results in the NNSmith's paper~\cite{NNSmith} due to the different settings on the compiler versions and testing amount.}

==> arXiv-2302.00842v2/tables/pickr.tex <==
% \begin{table}[]

%     \begin{minipage}[]{0.5\textwidth}
% 		\centering
%         \tabcolsep=0.5mm
		\caption{Results of Sensitivity Experiment of $picking\ rate$}
        \label{tab:pickrate}
        \begin{tabular}{crrrr}
                %\textbf{Picking Rate}
                \multicolumn{1}{c}{\textbf {\begin{tabular}[c]{@{}c@{}}Picking-\\ Rate\end{tabular}}}
                & \multicolumn{1}{c}{\textbf{time/s}} & \multicolumn{1}{c}{\textbf{NOP}} & \multicolumn{1}{c}{\textbf{NTR}} & \multicolumn{1}{c}{\textbf{NSA}} \\
                \textbf{0.5}          & \textbf{215.29}                 & 51.07                         & 23.73                          & \textbf{62.86}                \\
                \textbf{0.8}          & 260.47                          & 82.91                          & 63.99                         & 42.05                         \\
                \textbf{0.9}          & 269.98                          & 94.34                         & 83.30                         & 33.84                         \\
                \textbf{0.95}         & 270.01                          & 100.17                         & 94.19                         & 29.54                         \\
                \textbf{0.97}         & \textbf{267.24}                 & \textbf{102.56}               & \textbf{98.77}                & \textbf{27.77}                \\
                \textbf{0.99}         & 266.36                          & \textbf{104.94}               & \textbf{103.57}               & 25.93                        
        \end{tabular}

% 	\end{minipage}
	
% \end{table}


==> arXiv-2302.00842v2/tables/table1.tex <==
\begin{table*}[htbp]

    \caption{List of reported bugs.}
    \label{tab:bugs}
    %\setlength{\tabcolsep}{5pt}
    
    \centering
    %\large
    \begin{tabular}{ccclcccc}
    \hline
        ID & Compiler & Issue ID & Component        & Type & Status & Confirmed & In the Released Version\\ 
        1  &   TVM    & \multirow{10}{*}{Blind for anonymous review}     &  Backend  & Error     &  Fixed &  \Checkmark & \XSolid   \\ 
        2  &   TVM    &      &    Backend       & Error     &  Dup. with \#1  &  \Checkmark & \XSolid   \\ 
        3  &   TVM    &      &    Frontend      & Error     &  Fixed    &   \Checkmark &  \Checkmark  \\ 
        4  &   TVM    &      &    Frontend      & Error &  Dup.  with \#3   &  \Checkmark &  \Checkmark   \\ 
        5  &   TVM    &      &    Frontend      & Error  &  Fixed    &  \Checkmark &  \Checkmark   \\ 
        6  &   TVM    &      &    Frontend      & Error     &  Fixed    &  \Checkmark &  \Checkmark   \\ 
        7  &   TVM    &      &    Backend       & Error  &  Open    &  \Checkmark &  \Checkmark \\ 
        8  &   TVM    &      &    Frontend      & Error &  Open     &  \Checkmark  &  \Checkmark  \\  
        9  &   TVM    &      &    Frontend      & Error &  Open     &  \Checkmark  &  \Checkmark  \\  
        10  &   TVM    &      &    Frontend      & Error &  Fixed     & \Checkmark   &  \Checkmark  \\  
        11  &   TVM    &      &    Backend(Suspected)     & Wrong-Result   &  Open    &  -  &  \Checkmark \\ 
        12 & ONNX Runtime &  &    Backend       & Wrong-Result     &  Patch Review & \Checkmark &  \Checkmark    \\ 
    \hline
    \end{tabular}
\end{table*}




==> arXiv-2302.00842v2/tables/table2.tex <==
\begin{table}[htbp]
    \caption{List of Operations}
    \label{tab:ops}
    %\setlength{\tabcolsep}{1pt}
%\small
    %\hspace{1pt} 
    \centering
    
\begin{tabular}{cccc}
Number & Operation Name  & Type            & Parameters                                   \\
1      & Identity        & Identity        & None                                         \\
2      & Abs             & Identity        & None                                         \\
3      & Neg             & Identity        & None                                         \\
4      & Reciprocal      & Identity        & None                                         \\
5      & Floor           & Identity        & None                                         \\
6      & Ceil            & Identity        & None                                         \\
7      & Round           & Identity        & None                                         \\
8      & Erf             & Identity        & None                                         \\
9      & Sign            & Identity        & None                                         \\
10     & Exp             & Identity        & None                                         \\
11     & Softsign        & Identity        & None                                         \\
12     & Softmax         & Identity        & axis                                         \\
13     & Sigmoid         & Identity        & None                                         \\
14     & HardSigmoid     & Identity        & alpha, beta                                  \\
15     & Relu            & Identity        & None                                         \\
16     & LeakyRelu       & Identity        & alpha                                        \\
17     & Selu            & Identity        & alpha, gamma                                 \\
18     & Sin             & Identity        & None                                         \\
19     & Cos             & Identity        & None                                         \\
20     & Sqrt            & Identity        & None                                         \\
% 21     & \textbf{LpNormalization} & Identity        & axis, p                                      \\
21     & PRelu           & Multi           & None                                         \\
22     & Flatten         & Multi           & axis                                         \\
23     & Add             & Multi           & None                                         \\
24     & Sub             & Multi           & None                                         \\
25     & Mul             & Multi           & None                                         \\
26     & Div             & Multi           & None                                         \\
27     & Sum             & Multi           & None                                         \\
28     & Max             & Multi           & None                                         \\
29     & Min             & Multi           & None                                         \\
30     & Mean            & Multi           & None                                         \\
\multirow{4}{*}{31}     & \multirow{4}{*}{MaxPool}         & \multirow{4}{*}{Multi}           & auto\_pad, ceil\_mode,              \\
       &                 &                 & dilations, kernel\_shape,  \\
       &                 &                 & pads, storage\_order \\
       &                 &                 & strides \\
\multirow{4}{*}{32}     & \multirow{4}{*}{AveragePool}     & \multirow{4}{*}{Multi}           & auto\_pad, ceil\_mode,    \\
       &                 &                 & count\_include\_pad,      \\
       &                 &                 & dilations, kernel\_shape, \\
       &                 &                 & pads, strides \\
\multirow{2}{*}{33}     & \multirow{2}{*}{LpPool}          & \multirow{2}{*}{Multi}           & auto\_pad, kernel\_shape,    \\
       &                 &                 & p, pads, strides \\
\multirow{3}{*}{34}     & \multirow{3}{*}{Conv}            & \multirow{3}{*}{Multi}           & auto\_pad, dilations,                   \\
       &                 &                 & group, kernel\_shape,                \\
       &                 &                 & pads, strides                \\
\multirow{2}{*}{35}     & MatMul          & Multi           & None                                         \\
\multirow{2}{*}{36}     & \multirow{2}{*}{Gemm}            & \multirow{2}{*}{Multi}           & alpha, beta,                   \\
       &                 &                 & transA, transB \\
\multirow{2}{*}{37}     & \multirow{2}{*}{Concat}          & Multi           & \multirow{2}{*}{axis}                                         \\
       &                 & ReShape         &                                          \\
% \multirow{2}{*}{39}     & \multirow{2}{*}{\textbf{ReduceSum}}       & Multi           & keepdims,noop\_wi-            \\
       &                 & ReShape         & th\_empty\_axes                     \\
38     & SpaceToDepth    & ReShape         & blocksize, mode                              \\
39     & ReduceMax       & ReShape         & axes, keepdims                               \\
40     & ReduceMean      & ReShape         & axes, keepdims                               \\
41     & ReduceMin       & ReShape         & axes, keepdims                               \\
42     & ReduceProd      & ReShape         & axes, keepdims                               \\
43     & ReduceSumSquare & ReShape         & axes, keepdims                               \\
44     & ReduceL1        & ReShape         & axes, keepdims                               \\
45     & ReduceL2        & ReShape         & axes, keepdims                               \\
%48     & ReduceLogSum    & ReShape         & axes, keepdims                               \\
46     & ReduceLogSumExp & ReShape         & axes, keepdims                              
\end{tabular}
\end{table}

==> arXiv-2302.00842v2/tables/table3.tex <==
\begin{table}[]
\begin{tabular}{lcrrr}
                                    & \multicolumn{1}{l}{} & \multicolumn{1}{c}{GenDice} & \multicolumn{1}{c}{Baseline1} & \multicolumn{1}{c}{Baseline2} \\
\multicolumn{1}{c}{}                & valid models         & \textbf{38993.8}            & 525.6                         & 6593.4                        \\
                                    & \multicolumn{1}{l}{} &                             &                               &                               \\
                                    & OTC                  & \textbf{100\%}              & 98.70\%                       & 96.09\%                       \\
\multicolumn{1}{c}{opreation-level} & IDC                  & \textbf{100\%}              & 97.52\%                       & 94.61\%                       \\
\multicolumn{1}{c}{metrics}         & ODC                  & \textbf{11.1739}            & 2.5739                        & 3.1956                        \\
\multicolumn{1}{c}{}                & SEC                  & \textbf{0.9929}             & 0.2142                        & 0.5738                        \\
                                    & SPC                  & \textbf{2767.5040}          & 22.7739                       & 81.1870                       \\
                                    &                      &                             &                               &                               \\
                                    & NOO                  & 15.5119                     & 2.1626                        & 15.5018                       \\
                                    & NOT                  & \textbf{12.6943}            & 2.0856                        & 11.3909                       \\
\multicolumn{1}{c}{graph-level}     & NOP                  & \textbf{13.3066}            & 1.0141                        & 2.5397                        \\
\multicolumn{1}{c}{metrics}         & NSP                  & 5.4229                      & 1.2147                        & \textbf{6.2904}               \\
\multicolumn{1}{c}{}                & NTP                  & \textbf{25.7387}            & 2.5457                        & 14.3949                       \\
                                    & MLP                  & \textbf{4.276}              & 1.7097                        & 2.0959                        \\
                                    & ALP                  & \textbf{2.7056}             & 1.5170                        & 1.0964                       
\end{tabular}
\end{table}

==> arXiv-2302.00842v2/tables/table4.tex <==
\begin{table}[t]
    \caption{Result of second Experiment}
    \label{tab:exper2}
    %\setlength{\tabcolsep}{5pt}
    \centering
    %\large
\begin{tabular}{ccccc}
 Approach &   Time & \# Valid Inputs & Avg. of \#Unique Ops & Avg. of Ops  \\ 
Baseline1 & \multirow{3}{*}{300s}  & 24 & 7.375 & 10.542 \\ 
Baseline2 &                        & 33 & 12.455 & 44.061  \\
GenDice   &                        & 109 & 17.211 & 34.862 \\ 
\end{tabular}

\end{table}

==> arXiv-2302.00842v2/tables/table5.tex <==
\begin{table}%[]
    \caption{Results of Sensitivity Experiment of $picking\ rate$}
    \label{tab:exper5}
    %\setlength{\tabcolsep}{1pt}
%\small
    %\hspace{1pt} 
    \centering
    
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

% \begin{tabular}{crrrrrr}
% \multicolumn{1}{l}{}                                                & \multicolumn{1}{l}{}                    & \multicolumn{1}{l}{Pick}         & \multicolumn{1}{l}{Thres.}       & \multicolumn{1}{l}{value}              & \multicolumn{1}{l}{}              & \multicolumn{1}{l}{}              \\
%                                                                     & \multicolumn{1}{l}{\textbf{0.5}}        & \multicolumn{1}{l}{\textbf{0.8}} & \multicolumn{1}{l}{\textbf{0.9}} & \multicolumn{1}{l}{\textbf{0.95}}      & \multicolumn{1}{l}{\textbf{0.98}} & \multicolumn{1}{l}{\textbf{0.99}} \\
% \textbf{\begin{tabular}[c]{@{}c@{}}\# valid \\ models\end{tabular}} & \textbf{37115.0}                        & 39281.0                          & 39529.6                          & \textbf{40819.0}                       & 40098.2                           & 40067.6                           \\
% \textbf{NOP}                                                        & \textbf{6.4690}                         & \textbf{10.8292}                 & \textbf{12.4428}                 & \textbf{13.2941}                       & 13.7868                           & \textbf{13.9863}                  \\
% { \textbf{NSP}}                                 & {\textbf{11.0360}} & {7.3798}    & { 6.0827}    & { \textbf{5.4114}} & { 5.0267}     & { 4.8915}    
% \end{tabular}

\begin{tabular}{cccc}

\textbf{Picking Rate} & \textbf{\# valid models} & \textbf{NOP}      & \textbf{NSP}      \\
\textbf{0.5}          & 111297.6                 & 6.47186           & \textbf{11.04458} \\
\textbf{0.8}          & 125572.4                 & 10.8291           & 7.37808           \\
\textbf{0.9}          & 127330.2                 & 12.45178          & 6.08246           \\
\textbf{0.95}         & \textbf{130537.2}        & \textbf{13.30472} & \textbf{5.41996}  \\
\textbf{0.98}         & 127104.8                 & 13.81482          & 5.02604           \\
\textbf{0.99}         & 126897                   & \textbf{14.00344} & 4.89982  

\end{tabular}


%\begin{tabular}{p{1cm}<{\centering}p{1cm}<{\centering}p{1cm}<{\raggedright}p{1cm}<{\flushright}p{1cm}<{\flushleft{}}}

\end{table}

% data of ICSE-2022 version
% \textbf{Picking Rate} & \textbf{\# valid models} & \textbf{NOP}     & \textbf{NSP}     \\
% \textbf{0.5}         & 37115.0                  & 6.4690           & \textbf{11.0360} \\
% \textbf{0.8}         & 39281.0                  & 10.8292          & 7.3798  \\
% \textbf{0.9}         & 39529.6         & 12.4428          & 6.0827           \\
% \textbf{0.95}        & \textbf{40819.0}         & \textbf{13.2941} & \textbf{5.4114}  \\
% \textbf{0.98}        & 40098.2                  & 13.7868          & 5.0267           \\
% \textbf{0.99}        & 40067.6                  & \textbf{13.9863} & 4.8915          

==> arXiv-2302.00842v2/tables/table_1_200_10000.tex <==
\begin{table*}[]

    % \vspace{-0.2cm} 
    \caption{Results on Graph-level and Operation-level Metrics}
    \label{tab:1_200}
    %\setlength{\tabcolsep}{1pt}
%\small
    % \hspace{1pt} 
    
    \centering


\begin{tabular}{c|rrr|rr|rr}
\textbf{}       & \multicolumn{1}{c}{\textbf{Isra}} & \multicolumn{1}{c}{\textbf{DeclGen}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Randoop-\\ Gen\end{tabular}}} & \multicolumn{1}{c}{\textbf{Isra*}} & \multicolumn{1}{c|}{\textbf{Muffin}} & \multicolumn{1}{c}{\rev{\textbf{Isra**}}} & \multicolumn{1}{c}{\rev{\textbf{NNSmith}}} \\ \hline
\textbf{time/s} & \textbf{320.1713}                 & 9011.9172                            & 4721.8233                                                                            & \textbf{20.1031}                   & 25847.6804                           & \rev{\textbf{111.8615}}                   & \rev{880.7737}                             \\
\textbf{}       &                                   &                                      &                                                                                      &                                    &                                      &                                     &                                      \\
\textbf{OTC}    & \textbf{100\%}                    & 97.536\%                             & 98.46\%                                                                              & \textbf{100\%}                     & \textbf{100\%}                       & \rev{\textbf{100\%}}                      & \rev{\textbf{100\%}}                       \\
\textbf{IDC}    & \textbf{92.95\%}                  & 90.178\%                             & 89.966\%                                                                             & \textbf{91.85\%}                   & 88.52\%                              & \rev{\textbf{89.54\%}}                    & \rev{88.71\%}                              \\
\textbf{ODC}    & \textbf{11.848}                   & 4.928                                & 10.616                                                                               & \textbf{8.75}                      & 4.22                                 & \rev{\textbf{6.925}}                      & \rev{6.225}                               \\
\textbf{SEC}    & \textbf{98.27\%}                  & 67.804\%                             & 88.08\%                                                                              & \textbf{98.15\%}                   & 35.49\%                              & \rev{\textbf{99.38\%}}                    & \rev{78.50\%}                              \\
\textbf{DEC}    & \textbf{90.208\%}                 & 2.126\%                              & 45.324\%                                                                             & \textbf{57.7\%}                    & 4.95\%                               & \rev{\textbf{84.30\%}}                    & \rev{28.70\%}                              \\
\textbf{SPC}    & \textbf{3001.938}                 & 227.018                              & 1509.356                                                                             & \textbf{1192.22}                   & 556.44                               & \rev{\textbf{2822.9}}                     & \rev{1641.725}                             \\
\textbf{}       &                                   &                                      &                                                                                      &                                    &                                      & \multicolumn{1}{l}{}                & \multicolumn{1}{l}{}                 \\
\textbf{NOO}    & \textbf{100.8766}                 & 2.8783                               & 100.1231                                                                             & \textbf{10.4236}                   & \textbf{10.4236}                     & \rev{\textbf{16.3999}}                    & \rev{\textbf{16.3999}}                     \\
\textbf{NOT}    & \textbf{45.237}                   & 2.76                                 & 33.0021                                                                              & \textbf{8.6589}                    & 5.3289                               & \rev{\textbf{13.1333}}                    & \rev{10.5113}                              \\
\textbf{NOP}    & \textbf{103.7621}                 & 1.4856                               & 98.6460                                                                              & \textbf{7.8243}                    & 6.399                                & \rev{\textbf{14.5851}}                    & \rev{10.4880}                              \\
\textbf{NTR}    & 102.9130                          & 0.6042                               & \textbf{105.5774}                                                                    & 4.6481                             & \textbf{6.0766}                      & \rev{\textbf{13.065}}                     & \rev{7.6740}                               \\
\textbf{NSA}    & \textbf{26.6252}                  & 1.5533                               & 10.0211                                                                              & 5.9253                             & \textbf{11.3604}                     & \rev{\textbf{10.8192}}                    & \rev{10.1459}                             
\end{tabular}

%\vspace{-3cm}

\end{table*}


% \begin{tabular}{crrrrr}
% \multicolumn{1}{l}{} & \multicolumn{1}{c}{\textbf{Isra}} & \multicolumn{1}{c}{\textbf{DeclGen}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Randoop-\\ Gen\end{tabular}}} & \multicolumn{1}{c}{\textbf{Isra*}} & \multicolumn{1}{c}{\textbf{Muffin}} \\
% %\hline
% \textbf{time/s}      & \textbf{320.17}                 & 9011.92                            & 4721.82                                                                           & \textbf{20.10}                   & 25847.68                          \\

% %\textbf{}            &                                   &                                      &                                                                                     &                                    &                                     \\
% \textbf{OTC}         & \textbf{100\%}                    & 97.536\%                             & 98.46\%                                                                             & \textbf{100\%}                     & \textbf{100\%}                      \\
% \textbf{IDC}         & \textbf{92.95\%}                  & 90.178\%                             & 89.966\%                                                                            & \textbf{91.85\%}                   & 88.52\%                             \\
% \textbf{ODC}         & \textbf{11.848}                   & 4.928                                & 10.616                                                                              & \textbf{8.75}                      & 4.22                                \\
% \textbf{SEC}         & \textbf{98.27\%}                  & 67.804\%                             & 88.08\%                                                                             & \textbf{98.15\%}                   & 35.49\%                             \\
% \textbf{DEC}         & \textbf{90.208\%}                 & 2.126\%                              & 45.324\%                                                                            & \textbf{57.7\%}                    & 4.95\%                              \\
% \textbf{SAC}         & \textbf{3001.938}                 & 227.018                              & 1509.356                                                                            & \textbf{1192.22}                   & 556.44                              \\
% %\textbf{}            &                                   &                                      &                                                                                     &                                    &                                     \\
% \textbf{NOO}         & \textbf{100.8766}                 & 2.8783                               & 100.1231                                                                            & \textbf{10.4236}                   & \textbf{10.4236}                    \\
% \textbf{NOT}         & \textbf{45.237}                   & 2.76                                 & 33.0021                                                                             & \textbf{8.6589}                    & 5.3289                              \\
% \textbf{NOP}         & \textbf{103.7621}                 & 1.4856                               & 98.6460                                                                             & \textbf{7.8243}                    & 6.399                               \\
% \textbf{NTR}         & 102.9130                          & 0.6042                               & \textbf{105.5774}                                                                   & 4.6481                             & \textbf{6.0766}                     \\
% \textbf{NSA}         & \textbf{26.6252}                  & 1.5533                               & 10.0211                                                                             & 5.9253                             & \textbf{11.3604}                             
% \end{tabular}

% %\vspace{-0.3cm}
% \end{table}



% \begin{table}[]\begin{tabular}{ccrrr}
% \multicolumn{1}{l}{}     & \multicolumn{1}{l}{} & \textbf{\toolname{}}     & \textbf{\boneshort{}}     & \textbf{\btwoshort{}} \\
% \textbf{}                & \textbf{time/s}      & \textbf{320.1713}    & 9011.9172            & 4721.8233            \\
% \textbf{}                & \textbf{}            & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
% \textbf{}                & \textbf{OTC}         & \textbf{100\%}       & 97.536\%             & 98.46\%              \\
% \textbf{}                & \textbf{IDC}         & \textbf{92.95\%}     & 90.178\%             & 89.966\%             \\
% \textbf{operation-level} & \textbf{ODC}         & \textbf{11.848\%}    & 4.928                & 10.616\%             \\
% \textbf{metrics}         & \textbf{SEC}         & \textbf{98.27\%}     & 67.804\%             & 88.08\%              \\
% \textbf{}                & \textbf{DEC}         & \textbf{90.208\%}    & 2.126\%              & 45.324\%             \\
% \textbf{}                & \textbf{SPC}         & \textbf{3001.938}    & 227.018              & 1509.356             \\
% \textbf{}                & \textbf{}            & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
% \textbf{}                & \textbf{NOO}         & \textbf{100.8766}    & 2.8783               & 100.1231             \\
% \textbf{}                & \textbf{NOT}         & \textbf{45.237}      & 2.76                 & 33.0021              \\
% \textbf{graph-level}     & \textbf{NOP}         & \textbf{103.7621}    & 1.486                & 98.6460              \\
% \textbf{metrics}         & \textbf{NTR}         & 102.9130             & 0.6042               & \textbf{105.5774}    \\
%                          & \textbf{NSP}         & \textbf{26.6252}     & 1.5533               & 10.0211              \\
%                          & \textbf{DST}         & 0.041                & \textbf{0.2756}      & 0.0445               \\
%                          & \textbf{MLP}         & 8.0667               & 1.8507               & \textbf{8.3899}     
% \end{tabular}
% \end{table}

==> arXiv-2302.00842v2/tables/table_1_30_10000.tex <==
\begin{table}[]

    \caption{Results of 1-30\Ziheng{to refine}\Luyao{remove operation-level metrics at left is okay.}\Ziheng{fix rand and inc order.}}
    \label{tab:1_30}
    %\setlength{\tabcolsep}{1pt}
%\small
    %\hspace{1pt} 
    \centering
\begin{tabular}{ccrrr}
\multicolumn{1}{l}{}     & \multicolumn{1}{l}{} & \textbf{\toolname{}}  & \textbf{\boneshort{}} & \textbf{\btwoshort{}} \\
\textbf{}                & \textbf{time/s}      & \textbf{19.38}    & 330.2655         & 194.5023             \\
\textbf{}                & \textbf{}            &                   &                  &                      \\
\textbf{}                & \textbf{OTC}         & \textbf{100\%}    & 97.844\%         & 97.536\%             \\
\textbf{}                & \textbf{IDC}         & \textbf{92.95\%}  & 90.332\%         & 89.472\%             \\
\textbf{operation-level} & \textbf{ODC}         & \textbf{8.79}     & 4.91             & 7.568                \\
\textbf{metrics}         & \textbf{SEC}         & \textbf{98.262\%} & 68.246\%         & 80.54\%              \\
\textbf{}                & \textbf{DEC}         & \textbf{25.276\%} & 2.102\%          & 18.86\%              \\
\textbf{}                & \textbf{SPC}         & \textbf{974.144}  & 226.856          & 691.566              \\
\textbf{}                & \textbf{}            &                   &                  &                      \\
\textbf{}                & \textbf{NOO}         & 15.4321           & 2.8783           & 15.4505              \\
\textbf{}                & \textbf{NOT}         & \textbf{13.3626}  & 2.7612           & 12.2484              \\
\textbf{graph-level}     & \textbf{NOP}         & 12.6837           & 1.4873           & \textbf{13.6511}     \\
\textbf{metrics}         & \textbf{NTR}         & 8.4232            & 0.5979           & \textbf{10.3643}     \\
                         & \textbf{NSP}         & \textbf{7.6405}   & 1.5468           & 3.2252               \\
                         & \textbf{DST}         & 0.1428            & \textbf{0.1599}  & 0.2774               \\
                         & \textbf{MLP}         & 4.1944            & 4.4294           & \textbf{1.8555}     
\end{tabular}
\end{table}

==> arXiv-2302.00842v2/tables/table_bugs.tex <==
\begin{table}[]
\caption{\# unique bugs detected on different compilers.}
\label{tab:bug_number}
\centering

\begin{tabular}{cccccc}

           & \toolname{} & \boneshort{} & \btwoshort{} & Muffin & TVMFuzz \\
TVM        & \textbf{18}      & 8                            & 14                      & 12     & 5       \\
Glow       & \textbf{4}       & 2                            & 2                       & 2      & -       \\
SophGo     & \textbf{11}      & 3                            & 3                       & 9      & -       \\
Total      & \textbf{33}      & 13                           & 19                      & 23     & 5      

\end{tabular}


\end{table}

==> arXiv-2302.00842v2/tables/table_muffin_0.97_10000.tex <==

   \caption{Results of muffin 0.97 10000\Ziheng{to refine}}
    \label{tab:muffin}
    %\setlength{\tabcolsep}{1pt}
%\small
    %\hspace{1pt} 
    \centering
  \begin{table}[]  
\begin{tabular}{crr}
             & \multicolumn{1}{c}{\textbf{Isra}} & \multicolumn{1}{c}{\textbf{Muffin}} \\
\textbf{OTC} & \textbf{100\%}                    & 100\%                               \\
\textbf{IDC} & \textbf{91.85\%}                  & 88.52\%                             \\
\textbf{ODC} & \textbf{8.69}                     & 4.17                                \\
\textbf{SEC} & \textbf{98.15\%}                  & 35.49\%                             \\
\textbf{SPC} & \textbf{1192.22}                  & 556.44                              \\
\textbf{}    &                                   &                                     \\
\textbf{NOO} & 10.4236                           & 10.4236                             \\
\textbf{NOT} & \textbf{8.6589}                   & 5.3289                              \\
\textbf{NOP} & \textbf{7.8243}                   & 6.399                               \\
\textbf{NTR} & 4.6481                            & \textbf{6.0766}                     \\
\textbf{NSP} & 5.9253                            & \textbf{11.3604}                    \\
\textbf{MLP} & 3.5833                            & \textbf{7.0792}                    
\end{tabular}
\end{table}

==> arXiv-2302.00842v2/tables/table_pickrate.tex <==
\begin{table}[t]
    \caption{Results of Sensitivity Experiment of $picking\ rate$}
    \label{tab:pickrate}
    %\setlength{\tabcolsep}{1pt}
%\small
    %\hspace{1pt} 
    \centering

\begin{tabular}{crrrr}
\textbf{Picking Rate} & \multicolumn{1}{c}{\textbf{time/s}} & \multicolumn{1}{c}{\textbf{NOP}} & \multicolumn{1}{c}{\textbf{NTR}} & \multicolumn{1}{c}{\textbf{NSA}} \\
\textbf{0.5}          & \textbf{215.2858}                 & 51.06744                         & 23.7335                          & \textbf{62.86254}                \\
\textbf{0.8}          & 260.4653                          & 82.9076                          & 63.98712                         & 42.04568                         \\
\textbf{0.9}          & 269.9829                          & 94.33816                         & 83.30116                         & 33.84228                         \\
\textbf{0.95}         & 270.0106                          & 100.1718                         & 94.19208                         & 29.54448                         \\
\textbf{0.97}         & \textbf{267.2378}                 & \textbf{102.55626}               & \textbf{98.77044}                & \textbf{27.76688}                \\
\textbf{0.99}         & 266.3605                          & \textbf{104.94422}               & \textbf{103.56684}               & 25.93236                        
\end{tabular}
\end{table}

\vspace{-0.2cm}
    % \begin{table}[]
% \begin{tabular}{crlllrlrrlrrrrrrr}
% \textbf{Picking Rate} & \multicolumn{1}{c}{\textbf{time}} & \multicolumn{1}{c}{\textbf{}} & \multicolumn{1}{c}{\textbf{OTC}} & \multicolumn{1}{c}{\textbf{IDC}} & \multicolumn{1}{c}{\textbf{ODC}} & \multicolumn{1}{c}{\textbf{SEC}} & \multicolumn{1}{c}{\textbf{DEC}} & \multicolumn{1}{c}{\textbf{SPC}} & \multicolumn{1}{c}{\textbf{}} & \multicolumn{1}{c}{\textbf{NOO}} & \multicolumn{1}{c}{\textbf{NOT}} & \multicolumn{1}{c}{\textbf{NOP}} & \multicolumn{1}{c}{\textbf{NTR}} & \multicolumn{1}{c}{\textbf{NSP}} & \multicolumn{1}{c}{\textbf{DST}} & \multicolumn{1}{c}{\textbf{MLP}} \\
% \textbf{0.5}          & \textbf{215.2858}                 &                               & 100\%                            & 92.95\%                          & 8.46                             & 98.27\%                          & 54.566\%                         & 3152.53                          &                               & \multicolumn{1}{l}{100}          & 51.2                             & 51.06744                         & 23.7335                          & \textbf{62.86254}                & 0.0105                           & 5.2638                           \\
% \textbf{0.8}          & 260.4653                          &                               & 100\%                            & 92.95\%                          & 11.018                           & 98.27\%                          & 83.44\%                          & \textbf{3168.516}                & \multicolumn{1}{r}{}          & 100                              & 51.21002                         & 82.9076                          & 63.98712                         & 42.04568                         & 0.0173                           & 7.31192                          \\
% \textbf{0.9}          & 269.9829                          &                               & 100\%                            & 92.95\%                          & 11.608                           & 98.27\%                          & 87.806\%                         & 3099.232                         &                               & 100                              & \textbf{51.23842}                & 94.33816                         & 83.30116                         & 33.84228                         & 0.01982                          & 8.07182                          \\
% \textbf{0.95}         & 270.0106                          &                               & 100\%                            & 92.95\%                          & 11.75                            & 98.27\%                          & 89.24\%                          & 3031.676                         &                               & 100                              & 51.2124                          & 100.1718                         & 94.19208                         & 29.54448                         & 0.0211                           & 8.453                            \\
% \textbf{0.96}         & 268.0957                          &                               & 100\%                            & 92.95\%                          & 11.766                           & 98.27\%                          & 89.456\%                         & 3020.32                          &                               & 100                              & 51.2048                          & 101.33792                        & 96.40912                         & 28.61842                         & 0.0214                           & 8.53216                          \\
% \textbf{0.97}         & 267.2378                          &                               & 100\%                            & 92.95\%                          & 11.786                           & 98.27\%                          & 89.668\%                         & 3011.63                          & \multicolumn{1}{r}{}          & 100                              & 51.21956                         & 102.55626                        & 98.77044                         & 27.76688                         & 0.02168                          & 8.62132                          \\
% \textbf{0.98}         & 266.047                           &                               & 100\%                            & 92.95\%                          & 11.784                           & 98.27\%                          & 89.84\%                          & 2973.578                         & \multicolumn{1}{r}{}          & 100                              & 51.21226                         & 103.76544                        & 101.15406                        & 26.81846                         & 0.0219                           & 8.69834                          \\
% \textbf{0.99}         & 266.3605                          &                               & 100\%                            & 92.95\%                          & \textbf{11.836}                  & 98.27\%                          & \textbf{90.042\%}                & 2968.824                         &                               & 100                              & 51.2081                          & \textbf{104.94422}               & \textbf{103.56684}               & 25.93236                         & \textbf{0.0222}                  & \textbf{8.77982}                 \\
% \multicolumn{1}{l}{}  & \multicolumn{1}{l}{}              &                               & \multicolumn{1}{r}{}             & \multicolumn{1}{r}{}             &                                  & \multicolumn{1}{r}{}             &                                  &                                  & \multicolumn{1}{r}{}          &                                  & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}            
% \end{tabular}
% \end{table}

==> sections/prop.tex <==

we design our delicate order for simplification on constraints.
, with constraint propagation, any order for instantiation is consistent. With this property, we design our delicate order for simplification on constraints.

\Luyao{or graph-level global consistency?}
The first property is called
\subsubsection{graph-level consistency}

%With taking each node as a variable (a set variable containing all of the elements related to a node), constraints of the computation graph form a binary CSP, consisting of two kinds of constraints: first are unary constraints on each node, and second are binary constraints between two nodes (i.e., the output of an node equals to the input of another node).

We call an operation $x$ is locally satisfied with the instantiation $Q$ if $eval(Q[\{Input_x, Attr_x\}], Spec_{OP_x}(Input_x, Attr_x)) = true$. 
An instantiation $Q$ on a computation graph holds global satisfaction, if all of operations in the graph are locally satisfied with $Q$.
A computation graph with global satisfaction, as well as no loop in the graph, corresponds to a semantically valid computation graph.

Because our instantiation follows the topological order of the computation graph, with only instantiating edges which are from previous nodes (nodes that are ahead of $x$ in the order) to current operation $x$, the instantiation on $x$ will not affect local satisfications of previous nodes (based on the property of topological order). Thus, as long as we are able to instantiate a new operation with its local satisfaction every time, the final instantiation will holds global satisfaction. Also, because we instantiates edges with the direction followed by the topological order, the overall graph is loop-free. Thus, following with the topological order, local satisfaction on each operation implies global satisfaction, also, leading to a semantically valid computation graph finally.


%for each operation $x$, only the output of operations that are ahead of $x$ in the order may affect the local satisfaction of $x$ (taking the output of an previous operation as the input of $x$). So when we instantiate operation $x$ in the order, its instantiation will not affect the local satisfication of operations ahead of $x$.



reduce the domain of $x$ by constraint propagation. Due to the acyclicity of topological order, the constraint propagation is loop-free. Also, we are able to generate


Because there is 

For a semantically valid computation graph, 

In Section~\ref{sec:approach}, we show that our instantiation for this CSP is consistent: by instantiating with the topological order, ensuring the constraints related to each single operation (local consistency) implies the satisfication of the overall constraints (global consistency).


\subsubsection{operation-level strong n-consistency}

The second property is called operation-level strong n-consistency. For the constraints related to each single operation, after determining the type and the number of tensors in the input, we could take attributes as a variable and each tensor in the input of the operation as a variable, then this CSP is strong n-consistency~\cite{apt2003principles}.

A strongly n-consistency CSP has the property that any consistent instantiation of a subset of the variables can be extended to a consistent instantiation of all of the variables~\cite{dechter1992local}.
Thus, any order for instantiation is consistent. With this property, we design our delicate order for simplification on constraints.

Above two good properties ensure the consistency of our instantiation during the whole process, thus our approach is sound, as well as, backtracking-free (no inconsistent instantiation will appear). Also, our approach samples solutions from the whole semantically valid space, so it is also complete.



\subsubsection{Properties of \tone{}}

%The first property is called graph-level consistency\Luyao{or graph-level global consistency?}. 
With taking each node as a variable (a set variable containing $Op_x$, $Input_x$, $Output_x$, $Attr_x$), then the constraints related to each operation (e.g. Equation~\ref{eqs1} and \ref{eqs2}) is an unary constraint, and each map in $\psi_G$ corresponds to a binary constraint on two variables (the output of an node equals to the input of another node), so it is a binary CSP. 
\Luyao{With the guarantee of some properties}
Thus, this CSP is always consistent, which means that ensuring the constraints related to each single operation (local consistency) implies the satisfication of the overall constraints (global consistency).

The second property is called operation-level strong n-consistency. For the constraints related to each single operation, after determining the type and the number of tensors in the input, we could take attributes as a variable and each tensor in the input of the operation as a variable, then this CSP is strong n-consistency~\cite{apt2003principles}. A strongly n-consistency CSP has the property that any consistent instantiation of a subset of the variables can be extended to a consistent instantiation of all of the variables~\cite{dechter1992local}.

For a computation graph $G$, taking each operation as a variable, it contains two types of constraints: unary constraint of each variable (operation's semantic specification on its attributes and input), and binary constraint of two nodes (the output of one operation is the input of another operation). The problem $P_G$ is a binary CSP.

A set of binary constraints that is arc consistent and has no empty domain can be inconsistent only if the network of constraints contains cycles ~\cite{}.
Because the graph $G$ is acyclic, so the 

\Luyao{todo}



\subsubsection{Properties of \ttwo{}}

% Not all of the computation graphs have a valid model. 

After determining $OP_x$ and $Indegree_x$, we could take $Attr_N$ as a set variable, and each tensor in $Input_x=\{in_1, in_2, in_3, ...\}$ as a variable.
Consider the problem $P:(Spec_{OP_N}, ..., \{Attr_{N}, in_1, in_2, in_3, ...\})$, it is strong n-consistent because that 

(1) the property of constraints. \Luyao{propagtion is a tree.}

(2) the allowance of the second way in our on-demand policy ensures that the domain is non-empty.

It indicates that the order of instantiation will not affect the consistency of instantiation.

%for every $i \in [1..k]$ and $a \in D(T_i)$, there exists a solution $Q \in sol(P)$ such that $a=Q[Str(T_i)]$.
% Back to the beginning of our construction, if we select reusing an existing tensor for $A$, then we will conduct the tensor matching process. The situation for tensor matching is trivial here because there is no instantiation yet. Thus all the existing tensors will be matched. Assume we choose the tensor $X_{out}$ which is the output of operation $X$. Then, we will assign value of attributes of $X_{out}$ to corresponding attributes of $A$: $a.len: 2, a[1]: 3, a[2]: 5$.


==> tables/table1.tex <==
\begin{table*}[htbp]

    \caption{List of reported bugs.}
    \label{tab:bugs}
    %\setlength{\tabcolsep}{5pt}
    
    \centering
    %\large
    \begin{tabular}{ccclcccc}
    \hline
        ID & Compiler & Issue ID & Component        & Type & Status & Confirmed & In the Released Version\\ 
        1  &   TVM    & \multirow{10}{*}{Blind for anonymous review}     &  Backend  & Error     &  Fixed &  \Checkmark & \XSolid   \\ 
        2  &   TVM    &      &    Backend       & Error     &  Dup. with \#1  &  \Checkmark & \XSolid   \\ 
        3  &   TVM    &      &    Frontend      & Error     &  Fixed    &   \Checkmark &  \Checkmark  \\ 
        4  &   TVM    &      &    Frontend      & Error &  Dup.  with \#3   &  \Checkmark &  \Checkmark   \\ 
        5  &   TVM    &      &    Frontend      & Error  &  Fixed    &  \Checkmark &  \Checkmark   \\ 
        6  &   TVM    &      &    Frontend      & Error     &  Fixed    &  \Checkmark &  \Checkmark   \\ 
        7  &   TVM    &      &    Backend       & Error  &  Open    &  \Checkmark &  \Checkmark \\ 
        8  &   TVM    &      &    Frontend      & Error &  Open     &  \Checkmark  &  \Checkmark  \\  
        9  &   TVM    &      &    Frontend      & Error &  Open     &  \Checkmark  &  \Checkmark  \\  
        10  &   TVM    &      &    Frontend      & Error &  Fixed     & \Checkmark   &  \Checkmark  \\  
        11  &   TVM    &      &    Backend(Suspected)     & Wrong-Result   &  Open    &  -  &  \Checkmark \\ 
        12 & ONNX Runtime &  &    Backend       & Wrong-Result     &  Patch Review & \Checkmark &  \Checkmark    \\ 
    \hline
    \end{tabular}
\end{table*}




==> tables/table2.tex <==
\begin{table}[htbp]
    \caption{List of Operations}
    \label{tab:ops}
    %\setlength{\tabcolsep}{1pt}
%\small
    %\hspace{1pt} 
    \centering
    
\begin{tabular}{cccc}
Number & Operation Name  & Type            & Parameters                                   \\
1      & Identity        & Identity        & None                                         \\
2      & Abs             & Identity        & None                                         \\
3      & Neg             & Identity        & None                                         \\
4      & Reciprocal      & Identity        & None                                         \\
5      & Floor           & Identity        & None                                         \\
6      & Ceil            & Identity        & None                                         \\
7      & Round           & Identity        & None                                         \\
8      & Erf             & Identity        & None                                         \\
9      & Sign            & Identity        & None                                         \\
10     & Exp             & Identity        & None                                         \\
11     & Softsign        & Identity        & None                                         \\
12     & Softmax         & Identity        & axis                                         \\
13     & Sigmoid         & Identity        & None                                         \\
14     & HardSigmoid     & Identity        & alpha, beta                                  \\
15     & Relu            & Identity        & None                                         \\
16     & LeakyRelu       & Identity        & alpha                                        \\
17     & Selu            & Identity        & alpha, gamma                                 \\
18     & Sin             & Identity        & None                                         \\
19     & Cos             & Identity        & None                                         \\
20     & Sqrt            & Identity        & None                                         \\
% 21     & \textbf{LpNormalization} & Identity        & axis, p                                      \\
21     & PRelu           & Multi           & None                                         \\
22     & Flatten         & Multi           & axis                                         \\
23     & Add             & Multi           & None                                         \\
24     & Sub             & Multi           & None                                         \\
25     & Mul             & Multi           & None                                         \\
26     & Div             & Multi           & None                                         \\
27     & Sum             & Multi           & None                                         \\
28     & Max             & Multi           & None                                         \\
29     & Min             & Multi           & None                                         \\
30     & Mean            & Multi           & None                                         \\
\multirow{4}{*}{31}     & \multirow{4}{*}{MaxPool}         & \multirow{4}{*}{Multi}           & auto\_pad, ceil\_mode,              \\
       &                 &                 & dilations, kernel\_shape,  \\
       &                 &                 & pads, storage\_order \\
       &                 &                 & strides \\
\multirow{4}{*}{32}     & \multirow{4}{*}{AveragePool}     & \multirow{4}{*}{Multi}           & auto\_pad, ceil\_mode,    \\
       &                 &                 & count\_include\_pad,      \\
       &                 &                 & dilations, kernel\_shape, \\
       &                 &                 & pads, strides \\
\multirow{2}{*}{33}     & \multirow{2}{*}{LpPool}          & \multirow{2}{*}{Multi}           & auto\_pad, kernel\_shape,    \\
       &                 &                 & p, pads, strides \\
\multirow{3}{*}{34}     & \multirow{3}{*}{Conv}            & \multirow{3}{*}{Multi}           & auto\_pad, dilations,                   \\
       &                 &                 & group, kernel\_shape,                \\
       &                 &                 & pads, strides                \\
\multirow{2}{*}{35}     & MatMul          & Multi           & None                                         \\
\multirow{2}{*}{36}     & \multirow{2}{*}{Gemm}            & \multirow{2}{*}{Multi}           & alpha, beta,                   \\
       &                 &                 & transA, transB \\
\multirow{2}{*}{37}     & \multirow{2}{*}{Concat}          & Multi           & \multirow{2}{*}{axis}                                         \\
       &                 & ReShape         &                                          \\
% \multirow{2}{*}{39}     & \multirow{2}{*}{\textbf{ReduceSum}}       & Multi           & keepdims,noop\_wi-            \\
       &                 & ReShape         & th\_empty\_axes                     \\
38     & SpaceToDepth    & ReShape         & blocksize, mode                              \\
39     & ReduceMax       & ReShape         & axes, keepdims                               \\
40     & ReduceMean      & ReShape         & axes, keepdims                               \\
41     & ReduceMin       & ReShape         & axes, keepdims                               \\
42     & ReduceProd      & ReShape         & axes, keepdims                               \\
43     & ReduceSumSquare & ReShape         & axes, keepdims                               \\
44     & ReduceL1        & ReShape         & axes, keepdims                               \\
45     & ReduceL2        & ReShape         & axes, keepdims                               \\
%48     & ReduceLogSum    & ReShape         & axes, keepdims                               \\
46     & ReduceLogSumExp & ReShape         & axes, keepdims                              
\end{tabular}
\end{table}

==> tables/table3.tex <==
\begin{table}[]
\begin{tabular}{lcrrr}
                                    & \multicolumn{1}{l}{} & \multicolumn{1}{c}{GenDice} & \multicolumn{1}{c}{Baseline1} & \multicolumn{1}{c}{Baseline2} \\
\multicolumn{1}{c}{}                & valid models         & \textbf{38993.8}            & 525.6                         & 6593.4                        \\
                                    & \multicolumn{1}{l}{} &                             &                               &                               \\
                                    & OTC                  & \textbf{100\%}              & 98.70\%                       & 96.09\%                       \\
\multicolumn{1}{c}{opreation-level} & IDC                  & \textbf{100\%}              & 97.52\%                       & 94.61\%                       \\
\multicolumn{1}{c}{metrics}         & ODC                  & \textbf{11.1739}            & 2.5739                        & 3.1956                        \\
\multicolumn{1}{c}{}                & SEC                  & \textbf{0.9929}             & 0.2142                        & 0.5738                        \\
                                    & SPC                  & \textbf{2767.5040}          & 22.7739                       & 81.1870                       \\
                                    &                      &                             &                               &                               \\
                                    & NOO                  & 15.5119                     & 2.1626                        & 15.5018                       \\
                                    & NOT                  & \textbf{12.6943}            & 2.0856                        & 11.3909                       \\
\multicolumn{1}{c}{graph-level}     & NOP                  & \textbf{13.3066}            & 1.0141                        & 2.5397                        \\
\multicolumn{1}{c}{metrics}         & NSP                  & 5.4229                      & 1.2147                        & \textbf{6.2904}               \\
\multicolumn{1}{c}{}                & NTP                  & \textbf{25.7387}            & 2.5457                        & 14.3949                       \\
                                    & MLP                  & \textbf{4.276}              & 1.7097                        & 2.0959                        \\
                                    & ALP                  & \textbf{2.7056}             & 1.5170                        & 1.0964                       
\end{tabular}
\end{table}

==> tables/table4.tex <==
\begin{table}[t]
    \caption{Result of second Experiment}
    \label{tab:exper2}
    %\setlength{\tabcolsep}{5pt}
    \centering
    %\large
\begin{tabular}{ccccc}
 Approach &   Time & \# Valid Inputs & Avg. of \#Unique Ops & Avg. of Ops  \\ 
Baseline1 & \multirow{3}{*}{300s}  & 24 & 7.375 & 10.542 \\ 
Baseline2 &                        & 33 & 12.455 & 44.061  \\
GenDice   &                        & 109 & 17.211 & 34.862 \\ 
\end{tabular}

\end{table}

==> tables/table5.tex <==
\begin{table}%[]
    \caption{Results of Sensitivity Experiment of $picking\ rate$}
    \label{tab:exper5}
    %\setlength{\tabcolsep}{1pt}
%\small
    %\hspace{1pt} 
    \centering
    
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

% \begin{tabular}{crrrrrr}
% \multicolumn{1}{l}{}                                                & \multicolumn{1}{l}{}                    & \multicolumn{1}{l}{Pick}         & \multicolumn{1}{l}{Thres.}       & \multicolumn{1}{l}{value}              & \multicolumn{1}{l}{}              & \multicolumn{1}{l}{}              \\
%                                                                     & \multicolumn{1}{l}{\textbf{0.5}}        & \multicolumn{1}{l}{\textbf{0.8}} & \multicolumn{1}{l}{\textbf{0.9}} & \multicolumn{1}{l}{\textbf{0.95}}      & \multicolumn{1}{l}{\textbf{0.98}} & \multicolumn{1}{l}{\textbf{0.99}} \\
% \textbf{\begin{tabular}[c]{@{}c@{}}\# valid \\ models\end{tabular}} & \textbf{37115.0}                        & 39281.0                          & 39529.6                          & \textbf{40819.0}                       & 40098.2                           & 40067.6                           \\
% \textbf{NOP}                                                        & \textbf{6.4690}                         & \textbf{10.8292}                 & \textbf{12.4428}                 & \textbf{13.2941}                       & 13.7868                           & \textbf{13.9863}                  \\
% { \textbf{NSP}}                                 & {\textbf{11.0360}} & {7.3798}    & { 6.0827}    & { \textbf{5.4114}} & { 5.0267}     & { 4.8915}    
% \end{tabular}

\begin{tabular}{cccc}

\textbf{Picking Rate} & \textbf{\# valid models} & \textbf{NOP}      & \textbf{NSP}      \\
\textbf{0.5}          & 111297.6                 & 6.47186           & \textbf{11.04458} \\
\textbf{0.8}          & 125572.4                 & 10.8291           & 7.37808           \\
\textbf{0.9}          & 127330.2                 & 12.45178          & 6.08246           \\
\textbf{0.95}         & \textbf{130537.2}        & \textbf{13.30472} & \textbf{5.41996}  \\
\textbf{0.98}         & 127104.8                 & 13.81482          & 5.02604           \\
\textbf{0.99}         & 126897                   & \textbf{14.00344} & 4.89982  

\end{tabular}


%\begin{tabular}{p{1cm}<{\centering}p{1cm}<{\centering}p{1cm}<{\raggedright}p{1cm}<{\flushright}p{1cm}<{\flushleft{}}}

\end{table}

% data of ICSE-2022 version
% \textbf{Picking Rate} & \textbf{\# valid models} & \textbf{NOP}     & \textbf{NSP}     \\
% \textbf{0.5}         & 37115.0                  & 6.4690           & \textbf{11.0360} \\
% \textbf{0.8}         & 39281.0                  & 10.8292          & 7.3798  \\
% \textbf{0.9}         & 39529.6         & 12.4428          & 6.0827           \\
% \textbf{0.95}        & \textbf{40819.0}         & \textbf{13.2941} & \textbf{5.4114}  \\
% \textbf{0.98}        & 40098.2                  & 13.7868          & 5.0267           \\
% \textbf{0.99}        & 40067.6                  & \textbf{13.9863} & 4.8915          

==> tables/table_1_30_10000.tex <==
\begin{table}[]

    \caption{Results of 1-30\Ziheng{to refine}\Luyao{remove operation-level metrics at left is okay.}\Ziheng{fix rand and inc order.}}
    \label{tab:1_30}
    %\setlength{\tabcolsep}{1pt}
%\small
    %\hspace{1pt} 
    \centering
\begin{tabular}{ccrrr}
\multicolumn{1}{l}{}     & \multicolumn{1}{l}{} & \textbf{\toolname{}}  & \textbf{\boneshort{}} & \textbf{\btwoshort{}} \\
\textbf{}                & \textbf{time/s}      & \textbf{19.38}    & 330.2655         & 194.5023             \\
\textbf{}                & \textbf{}            &                   &                  &                      \\
\textbf{}                & \textbf{OTC}         & \textbf{100\%}    & 97.844\%         & 97.536\%             \\
\textbf{}                & \textbf{IDC}         & \textbf{92.95\%}  & 90.332\%         & 89.472\%             \\
\textbf{operation-level} & \textbf{ODC}         & \textbf{8.79}     & 4.91             & 7.568                \\
\textbf{metrics}         & \textbf{SEC}         & \textbf{98.262\%} & 68.246\%         & 80.54\%              \\
\textbf{}                & \textbf{DEC}         & \textbf{25.276\%} & 2.102\%          & 18.86\%              \\
\textbf{}                & \textbf{SPC}         & \textbf{974.144}  & 226.856          & 691.566              \\
\textbf{}                & \textbf{}            &                   &                  &                      \\
\textbf{}                & \textbf{NOO}         & 15.4321           & 2.8783           & 15.4505              \\
\textbf{}                & \textbf{NOT}         & \textbf{13.3626}  & 2.7612           & 12.2484              \\
\textbf{graph-level}     & \textbf{NOP}         & 12.6837           & 1.4873           & \textbf{13.6511}     \\
\textbf{metrics}         & \textbf{NTR}         & 8.4232            & 0.5979           & \textbf{10.3643}     \\
                         & \textbf{NSP}         & \textbf{7.6405}   & 1.5468           & 3.2252               \\
                         & \textbf{DST}         & 0.1428            & \textbf{0.1599}  & 0.2774               \\
                         & \textbf{MLP}         & 4.1944            & 4.4294           & \textbf{1.8555}     
\end{tabular}
\end{table}

==> tables/table_bugs.tex <==
\begin{table}[]
\caption{\# unique bugs detected on different compilers.}
\label{tab:bug_number}
\centering

\begin{tabular}{cccccc}

           & \toolname{} & \boneshort{} & \btwoshort{} & Muffin & TVMFuzz \\
TVM        & \textbf{18}      & 8                            & 14                      & 12     & 5       \\
Glow       & \textbf{4}       & 2                            & 2                       & 2      & -       \\
SophGo     & \textbf{11}      & 3                            & 3                       & 9      & -       \\
Total      & \textbf{33}      & 13                           & 19                      & 23     & 5      

\end{tabular}


\end{table}

==> tables/table_muffin_0.97_10000.tex <==

   \caption{Results of muffin 0.97 10000\Ziheng{to refine}}
    \label{tab:muffin}
    %\setlength{\tabcolsep}{1pt}
%\small
    %\hspace{1pt} 
    \centering
  \begin{table}[]  
\begin{tabular}{crr}
             & \multicolumn{1}{c}{\textbf{Isra}} & \multicolumn{1}{c}{\textbf{Muffin}} \\
\textbf{OTC} & \textbf{100\%}                    & 100\%                               \\
\textbf{IDC} & \textbf{91.85\%}                  & 88.52\%                             \\
\textbf{ODC} & \textbf{8.69}                     & 4.17                                \\
\textbf{SEC} & \textbf{98.15\%}                  & 35.49\%                             \\
\textbf{SPC} & \textbf{1192.22}                  & 556.44                              \\
\textbf{}    &                                   &                                     \\
\textbf{NOO} & 10.4236                           & 10.4236                             \\
\textbf{NOT} & \textbf{8.6589}                   & 5.3289                              \\
\textbf{NOP} & \textbf{7.8243}                   & 6.399                               \\
\textbf{NTR} & 4.6481                            & \textbf{6.0766}                     \\
\textbf{NSP} & 5.9253                            & \textbf{11.3604}                    \\
\textbf{MLP} & 3.5833                            & \textbf{7.0792}                    
\end{tabular}
\end{table}

==> tables/table_pickrate.tex <==
\begin{table}[t]
    \caption{Results of Sensitivity Experiment of $picking\ rate$}
    \label{tab:pickrate}
    %\setlength{\tabcolsep}{1pt}
%\small
    %\hspace{1pt} 
    \centering

\begin{tabular}{crrrr}
\textbf{Picking Rate} & \multicolumn{1}{c}{\textbf{time/s}} & \multicolumn{1}{c}{\textbf{NOP}} & \multicolumn{1}{c}{\textbf{NTR}} & \multicolumn{1}{c}{\textbf{NSA}} \\
\textbf{0.5}          & \textbf{215.2858}                 & 51.06744                         & 23.7335                          & \textbf{62.86254}                \\
\textbf{0.8}          & 260.4653                          & 82.9076                          & 63.98712                         & 42.04568                         \\
\textbf{0.9}          & 269.9829                          & 94.33816                         & 83.30116                         & 33.84228                         \\
\textbf{0.95}         & 270.0106                          & 100.1718                         & 94.19208                         & 29.54448                         \\
\textbf{0.97}         & \textbf{267.2378}                 & \textbf{102.55626}               & \textbf{98.77044}                & \textbf{27.76688}                \\
\textbf{0.99}         & 266.3605                          & \textbf{104.94422}               & \textbf{103.56684}               & 25.93236                        
\end{tabular}
\end{table}

\vspace{-0.2cm}
    % \begin{table}[]
% \begin{tabular}{crlllrlrrlrrrrrrr}
% \textbf{Picking Rate} & \multicolumn{1}{c}{\textbf{time}} & \multicolumn{1}{c}{\textbf{}} & \multicolumn{1}{c}{\textbf{OTC}} & \multicolumn{1}{c}{\textbf{IDC}} & \multicolumn{1}{c}{\textbf{ODC}} & \multicolumn{1}{c}{\textbf{SEC}} & \multicolumn{1}{c}{\textbf{DEC}} & \multicolumn{1}{c}{\textbf{SPC}} & \multicolumn{1}{c}{\textbf{}} & \multicolumn{1}{c}{\textbf{NOO}} & \multicolumn{1}{c}{\textbf{NOT}} & \multicolumn{1}{c}{\textbf{NOP}} & \multicolumn{1}{c}{\textbf{NTR}} & \multicolumn{1}{c}{\textbf{NSP}} & \multicolumn{1}{c}{\textbf{DST}} & \multicolumn{1}{c}{\textbf{MLP}} \\
% \textbf{0.5}          & \textbf{215.2858}                 &                               & 100\%                            & 92.95\%                          & 8.46                             & 98.27\%                          & 54.566\%                         & 3152.53                          &                               & \multicolumn{1}{l}{100}          & 51.2                             & 51.06744                         & 23.7335                          & \textbf{62.86254}                & 0.0105                           & 5.2638                           \\
% \textbf{0.8}          & 260.4653                          &                               & 100\%                            & 92.95\%                          & 11.018                           & 98.27\%                          & 83.44\%                          & \textbf{3168.516}                & \multicolumn{1}{r}{}          & 100                              & 51.21002                         & 82.9076                          & 63.98712                         & 42.04568                         & 0.0173                           & 7.31192                          \\
% \textbf{0.9}          & 269.9829                          &                               & 100\%                            & 92.95\%                          & 11.608                           & 98.27\%                          & 87.806\%                         & 3099.232                         &                               & 100                              & \textbf{51.23842}                & 94.33816                         & 83.30116                         & 33.84228                         & 0.01982                          & 8.07182                          \\
% \textbf{0.95}         & 270.0106                          &                               & 100\%                            & 92.95\%                          & 11.75                            & 98.27\%                          & 89.24\%                          & 3031.676                         &                               & 100                              & 51.2124                          & 100.1718                         & 94.19208                         & 29.54448                         & 0.0211                           & 8.453                            \\
% \textbf{0.96}         & 268.0957                          &                               & 100\%                            & 92.95\%                          & 11.766                           & 98.27\%                          & 89.456\%                         & 3020.32                          &                               & 100                              & 51.2048                          & 101.33792                        & 96.40912                         & 28.61842                         & 0.0214                           & 8.53216                          \\
% \textbf{0.97}         & 267.2378                          &                               & 100\%                            & 92.95\%                          & 11.786                           & 98.27\%                          & 89.668\%                         & 3011.63                          & \multicolumn{1}{r}{}          & 100                              & 51.21956                         & 102.55626                        & 98.77044                         & 27.76688                         & 0.02168                          & 8.62132                          \\
% \textbf{0.98}         & 266.047                           &                               & 100\%                            & 92.95\%                          & 11.784                           & 98.27\%                          & 89.84\%                          & 2973.578                         & \multicolumn{1}{r}{}          & 100                              & 51.21226                         & 103.76544                        & 101.15406                        & 26.81846                         & 0.0219                           & 8.69834                          \\
% \textbf{0.99}         & 266.3605                          &                               & 100\%                            & 92.95\%                          & \textbf{11.836}                  & 98.27\%                          & \textbf{90.042\%}                & 2968.824                         &                               & 100                              & 51.2081                          & \textbf{104.94422}               & \textbf{103.56684}               & 25.93236                         & \textbf{0.0222}                  & \textbf{8.77982}                 \\
% \multicolumn{1}{l}{}  & \multicolumn{1}{l}{}              &                               & \multicolumn{1}{r}{}             & \multicolumn{1}{r}{}             &                                  & \multicolumn{1}{r}{}             &                                  &                                  & \multicolumn{1}{r}{}          &                                  & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}            
% \end{tabular}
% \end{table}
